How Do Data Analysts Respond to AI Assistance? A Wizard-of-Oz Study

Data analysis is challenging as analysts must navigate nuanced decisions that may yield divergent conclusions. AI assistants have the potential to support analysts in planning their analyses, enabling more robust decision making. Though AI-based assistants that target code execution (e.g., Github Copilot) have received significant attention, limited research addresses assistance for both analysis execution and planning. In this work, we characterize helpful planning suggestions and their impacts on analysts' workflows. We first review the analysis planning literature and crowd-sourced analysis studies to categorize suggestion content. We then conduct a Wizard-of-Oz study (n=13) to observe analysts' preferences and reactions to planning assistance in a realistic scenario. Our findings highlight subtleties in contextual factors that impact suggestion helpfulness, emphasizing design implications for supporting different abstractions of assistance, forms of initiative, increased engagement, and alignment of goals between analysts and assistants.

==> 0-figures-and-tables.tex <==
\newcommand{\wozFig}{
\begin{figure*}[t!]
  \centering
  \includegraphics[width=0.89\linewidth]{final_figures/woz.pdf}
  \caption{In our \woz study, analysts work with a JupyterLab notebook containing the assistant interface (left). They are unaware of the existence of a human wizard, located in a separate room, operating the assistant backend (right). The wizard uses a general purpose LLM and integrates information prepared before the study. The wizard observes the analyst's notebook for opportunities for assistance and obtains the relevant notebook context (A). Next, the wizard either retrieves a prewritten suggestion developed prior to the study (B) or prompts the LLM (C) to generate a relevant suggestion (D). The wizard may further refine the suggestion (e.g., shorten its length) with additional prompting of the LLM (C-D Loop). Finally, after creating the suggestion, the wizard presents the suggestion back to the analyst (E). In this process, the wizard acts as the interface between the analyst and the LLM, deciding on the content and timing of the suggestion. 
  % \tim{love the aesthetics! the dashed line has shading and nothing else does. I suggest to remove the shading for visual consistency}
  }
  \Description{The figure shows the analyst perception of the assistant on the left. This is an analyst icon with a JupyterLab notebook. The right side shows the assistant backend on the right consisting of a wizard icon, a monitor icon with ChatGPT and a spreadsheet icon. The figure also consists of the following arrows:
  1. The JupyterLab notebook to the wizard (labeled A)
  2. The spreadsheet to the wizard (labeled B)
  3. The wizard to the ChatGPT icon (labeled C)
  4. The ChatGPT icon to the wizard (labeled D)
  5. The wizard to the JupyterLab notebook (labeled E)
  }
  \label{fig:woz}
\end{figure*}
}




\newcommand{\quadrantFig}{
\begin{figure}[t]
  \centering
  \includegraphics[width=0.92\linewidth]{final_figures/quadrant.pdf}
  \caption{\textbf{Planning assistance has limited support and is unexplored}. Existing assistants, such as Github Copilot,  are well-suited for execution assistance, such as suggesting data wrangling or modeling code. 
  % Suggestions can be initiated by the analyst, such as through an explicit query (A), or by the assistant, based on the current context (B). While tools like ChatGPT may provide basic planning assistance (C), analysts can struggle to write effective prompts. Thus, there may be easier ways to initiate planning assistance or opportunities to rely on assistant initiation (D). However, it is unclear how to provide assistant-initiated planning assistance. Naive applications of LLMs alone cannot support this since they do not know the timing and relevant context for an assistant. Thus, they require selective context, higher-level scaffolding, targeted prompts, and triggers. 
  % In practice, planning assistance may be offered in conjunction with execution assistance to be easily adapted by the analyst.
  }
  \Description{The figure shows four quadrants. From left to right and top to bottom, the quadrants are labeled A, B, C, and D. The x-axis is labeled analyst-initiated and assistant-initiated. The y-axis is labeled execution assistance and planning assistance. The top row indicating execution assistance shows existing systems such as Github Copilot and ChatGPT. The bottom left quadrant shows analyst-initiated planning assistance which needs LLMs and LLM/domain expertise. The bottom right quadrant for assistant-initiated planning assistance show N/A for no current systems.}
  \label{fig:quadrant}
\end{figure}
}

\newcommand{\tableDefinitions}{
\begin{table}
  \caption{Relevant Multiverse Analysis Definitions}
  \label{tab:definitions}
  \begin{tabular}{cl}
    \toprule
    Term & Definition\\
    \midrule
     Decision & \makecell{Any reasonable and defensible decision that an analyst may consider in an analysis. \\ &(e.g., Statistical Model, Data Filtering etc.)} \\
     Decision Option & The alternatives an analyst considers in a decision. (e.g., bayesian model, frequentist model, etc.) \\
     Universe & A single end-to-end analysis representing one combination of decision options \\
     Multiverse & A collection of all universes as specified by a set of decisions and their decision options\\
  \bottomrule
\end{tabular}
\end{table}
}


\newcommand{\interfaceFig}{
\begin{figure*}[t!]
  \centering
  \includegraphics[width=0.95\linewidth]{final_figures/interface.pdf}
  \caption{\textbf{Assistant User Interface}. Our assistant is integrated into JupyterLab as a side panel. Analysts can open the side panel in the right sidebar (A) and turn the assistant on/off with a toggle (B). Suggestions are raised as cards in this side panel. When first turned on, the assistant welcomes the analyst with a startup message (C). When a new suggestion occurs, the side panel shows a loading animation of variable duration to call attention to it; variability in duration aims to indicate that the system is working and simulate a real system computing and generating a suggestion~\cite{Fraser1991SimulatingSS, Riek2012WizardOO}. New suggestions also have a yellow highlight around them for greater visibility (D). Likewise, each suggestion has a corresponding context (D1) in the notebook, which is automatically scrolled into view when the suggestion is clicked (D2). Analysts can provide feedback for each suggestion via the thumbs-up and thumbs-down buttons (E). Finally, analysts can copy recommended code using the copy button (F). Note that the width of the side panel can be adjusted and is typically smaller than is pictured here for illustration.
  % \jeff{Figure has F and G, not E and F!}
  % \tim{Minor: match letters across figures. fig 1 uses colorful rectangles with rounded corners :)}
  }
  \Description{The figure shows a screenshot of the JupyterLab notebook interface with the notebook on the left side and the suggestion panel on the right side.}
  \label{fig:interface}
\end{figure*}
}
\newcommand{\tableResults}{
\begin{table*}[t]
% \small
  \centering
  \renewcommand{\arraystretch}{1.23} % Adjust the vertical spacing of rows
  % \large
  \begin{tabular}{| p{1.8 cm} | p{11.5cm} p{1.4cm}|}
    \hline
    & \textbf{Assistants should ...} & \\
    \hline
    \multirow{3}{*}{\parbox{2.0cm}{\raggedright \textbf{Alignment}}} & 1. Communicate with analysts to align on analysis goals.&  (Sec.~\ref{sec:discussion_design_implications_match_goals}) \\
    % \cline{2-2}
    & 2. Provide suggestion content suited to the analysts' background.& (Sec.~\ref{sec:discussion_design_implications_match_bg}) \\
    % \cline{2-2}
    & 3. Match analysts' preferred level of planning assistance abstraction.& (Sec.~\ref{sec:discussion_design_implications_match_abstraction})\\
    \hline
    \multirow{2}{*}{\parbox{2.0cm}{\raggedright \textbf{Timing and Initiative}}} & 4. Time suggestions based on analysts' openness to considering alternative approaches.& (Sec.~\ref{sec:discussion_design_implications_timing})\\
     & 5. Provide multiple ways to request content for different levels of abstraction. & (Sec.~\ref{sec:discussion_design_implications_initiative}) \\
    \hline
    \multirow{2}{*}{\parbox{2.0cm}{\raggedright \textbf{Engagement and Trust}}} & 6. Mitigate suggestion overreliance by promoting engagement and critical thinking. & (Sec. ~\ref{sec:discussion_design_implications_trust})\\
     & 7. Adopt multiple explanation methods for increased understanding and trust.
     % Mitigate suggestion overreliance by promoting engagement and critical thinking.
     % Encourage critical thinking and engagement to counterbalance suggestion automation.
     & (Sec. ~\ref{sec:discussion_design_implications_explanation})\\
    \hline
  \end{tabular}
  \caption{Design implications and takeaways for building analysis assistants. }
  \label{tab:design_implications}
\end{table*}
}
\newcommand{\tableParticipants}{
\begin{table*}
    \small
 
  \begin{tabular}{lllllcc}
    \toprule
    \textbf{ID} & \textbf{Gender} & \textbf{Occupation/Background} & \rr{\textbf{AI Code Assistant Usage}} & \textbf{Prog Lang} & \textbf{Lang Exp} & \textbf{Stats Exp} \\
    \midrule
    A01 & Male & Professor in Public Policy  & None & R & 4 & 5 \\
    A02 & Male & PhD Student in Public Policy & None & R & 5 & 4 \\
    A03 & Male & PhD Student in Civil Engineering & None & Python & 5 & 4 \\
    A04 & Male & Research Scientist in Public Policy & Minimal & R & 5 & 4 \\
    A05 & Female & Masters Student in Data Science & Regular & Python & 4 & 4 \\
    A06 & Female & Masters Student in Data Science & None & Python & 4 & 4 \\
    A07 & Male & Masters Student in Data Science & Minimal & Python & 4 & 5 \\
    A08 & Female & PhD Student in Atmospheric Sciences & Minimal & Python & 5 & 5 \\
    A09 & Female & PhD Student in Political Science & None & R & 4 & 4 \\
    A10 & Male & Data Scientist & Regular & Python & 5 & 5 \\
    A11 & Female & Masters Student in Data Science & Regular & Python & 4 & 4 \\
    A12 & Male & PostDoc in Materials Science & None & R & 4 & 4 \\
    A13 & Female & PhD Student in Computational Finance & None & Python & 4 & 4 \\
    \bottomrule

  \end{tabular}
  \caption{\textbf{Participant Information.} \rr{Prior AI code assistant experience was gathered from our study interviews.}}
   \label{tab:participants}
\end{table*}
}

% \newcommand{\tableParticipants}{
% \begin{table*}
%     \small
 
%   \begin{tabular}{llllcc}
%     \toprule
%     ID & Gender & Occupation/Background & Lang. & Lang. Proficiency & Stats. Proficiency \\
%     \midrule
%     A01 & Male & Professor in Public Policy  & R & 4 & 4 \\
%     A02 & Male & PhD Student in Public Policy & R & 5 & 4\\
%     A03 & Male & PhD Student in Civil Engineering & Python & 5 & 4\\
%     A04 & Male & Research Scientist in Public Policy & R & 5 & 4 \\
%     A05 & Female & Masters Student in Data Science & Python &4 & 4\\
%     A06 & Female & Masters Student in Data Science & Python &4 & 4\\
%     A07 & Male & Masters Student in Data Science & Python & 4 & 5 \\
%     A08 & Female & PhD Student in Atmospheric Sciences & Python & 5 & 5\\
%     A09 & Female & PhD Student in Political Science & R & 4 & 4\\
%     A10 & Male & Data Scientist & Python & 5 & 5 \\
%     A11 & Female & Masters Student in Data Science & Python & 4 & 4\\
%     A12 & Male & PostDoc in Materials Science & R & 4 & 4 \\
%     A13 & Female & PhD Student in Computational Finance & Python & 4 & 4 \\
%     \bottomrule
%   \end{tabular}
%   \caption{\textbf{Participant Information.} Proficiency was self-rated on a 5-point scale, with 5 being the highest.}
%    \label{tab:participants}
% \end{table*}
% }

\newcommand{\tableSuggestions}{
\begin{table*}
  \small
  
  \begin{tabular}{p{2.6cm}p{14.0cm}p{0.0cm}}
    \toprule
    \raggedright \textbf{Suggestion Category} & \textbf{Example} &   \\
    \toprule
    \raggedright Domain Background & \textbf{Similar Analyses Done in the Past}

    The question of whether skin tone influences the way referees make decisions in soccer games has been a topic of research. 
    "Racial Bias in the Allocation of Fouls in Soccer" by Price and Wolfers (2010) is a representative study...
    % One of the most well-known studies in this area is "Racial Bias in the Allocation of Fouls in Soccer" by Price and Wolfers (2010).  
    & \\
    \midrule
    \raggedright Data Wrangling Assistance & \textbf{Reminder - Check for Missing Data}

    Always check for missing data values in your DataFrame before performing any data analysis or machine learning tasks. Missing data can cause unexpected errors and affect the accuracy of your results.
    
    \texttt{\# Use boolean indexing to filter the DataFrame and show only the rows with missing values}

    \texttt{rows\_with\_na = df[df.isna().any(axis=1)]}

    \texttt{rows\_with\_na.head()}
    ...
    & \\
    \midrule
    \raggedright Conceptual Model Formulation & \textbf{Other Variables that Might Influence Red Cards: Age Variable Rationale}

    Beyond just skin tone, we can consider other variables that might affect the analysis. As birthday is in the dataframe, we might want to control for age, which is a common practice in research studies, since age can affect various aspects of behavior and cognition. One reason to control for age is to account for the tendency of impulsivity, which may be associated with receiving red cards, which decreases with age... &   \\
    \midrule
    \raggedright Operationalizing Constructs & \textbf{Skin Tone Operationalization}

    Right now, skin tone rating is represented by \texttt{rater1} and \texttt{rater2}. The \texttt{rater1} and \texttt{rater2} variables could be averaged and rounded to the most central value. We could also create a binary variable based on a rating threshold. This way, we could work with only one variable for player skin tone. It is up to you to decide which decision to make to ensure the validity and reliability of your results.
    This code shows a template for representing skin tone...
    &  \\
    \midrule
    \raggedright Choosing the Statistical Model & 
    \textbf{Using a Poisson Model}

    Here, we want to investigate the relationship between a player's skin tone and the number of red cards they receive from referees. Since the outcome variable, i.e., the number of red cards received by a player is a count variable (i.e., it is a non-negative integer), it might make sense to consider a Poisson model to analyze this relationship...
    &   \\
    \midrule
    \raggedright Model Results Interpretation & \textbf{Results Interpretation}

    % The regression model suggests that skin tone and the number of goals are both significant predictors of receiving red cards. The R-squared value of 0.005 indicates that the model explains only a small proportion of the variance in the redCards variable... 
    The regression suggests that skin tone and the number of goals are significant predictors red cards. The R-squared value of 0.005 indicates that the model explains only a small proportion of the variance in the redCards variable... 
    & \\
    \midrule
    \raggedright High-Level Planning & \textbf{Consider Including Covariates}
    
Covariates are additional variables that can affect the relationship between the predictor variable and the outcome variable in an analysis. To accurately understand the relationship between the predictor and outcome variable, it is important to consider the effects of these covariates.

Including covariates in an analysis can help to control for potential confounding variables... &  \\
    \midrule
    \raggedright Execution Assistance & \textbf{Answering: Is the number of red cards associated with some unique referee ID?}
    % How does this vary among different skin ratings?}

    Here is some code to answer this question.

    % \texttt{\# Group the data by unique referee IDs}

    \texttt{referee\_groups = df.groupby('refNum')}
    ...
    &\\
    \bottomrule
    
  \end{tabular}
  \caption{Categories of suggestions informed by a literature review and a behavior-driven analysis of a crowd-sourced data analysis study. With the exception of \textit{high-level planning} and \textit{execution assistance}, the dimensions correspond to assistance during the stages in an end-to-end analysis. \textit{High-level planning} involves more general considerations.}
  \label{tab:suggestions}
\end{table*}
}

\newcommand{\resultsFig}{
\begin{figure*}[t]
  \centering
  \includegraphics[width=0.99\linewidth]{final_figures/results.pdf}
  \caption{\textbf{Study-informed Model of Analyst-Assistant Interaction Dynamics}. Based on our study findings, we model the underlying influences and interactions between an analyst and an assistant. The assistant can receive information about the analyst's initiative (A) and the analysis contents (B) to develop an understanding of the analyst's goals and background as well as the current analysis plan and context (C). Note that the analyst's initiative is optional. This, in conjunction with the assistant's programmed goals (D) (e.g., offering more planning assistance or doing only what analysts request), informs the assistance (i.e., timing, organization, location, execution vs. planning, and contents) provided to analysts (E). After a suggestion is raised to the analyst, how it is perceived (F) is impacted by the analyst's background (G) and their current analysis plan (H). This then determines the extent to which the analyst accepts the suggestion in their planning (H) and/or execution (I) processes. The loop then continues as analysts update their analysis (B) or require additional assistance (A).
  % \tim{since this come sat the top of results I think it's possible to mistake this figure for your how system/wizard worked (e.g. ``programmed goals''. I think you should say clearly in the bold text and first caption sentence that this is a model of interaction dynamics that is informed by the results of your study.}
  % \jeff{I don't totally follow the ordering here. For example the caption mentions G and H before F.} fixed ordering of sentence
  }
  \Description{A diagram split down the middle vertically separating the components on the analyst side on the left and the assistant side on the right. The analysts side includes the following components written in boxes: analyst's background and goals, analyst initiative, notebook contents, planning analysis process, execution analysis process, and analyst's perception of the assistant. The assistant side includes the assistant goals, assistant's perception of the analyst, and suggestion. Arrows point between these components to inform a  model of analyst-assistant interaction dynamics.}
  \label{fig:results}
\end{figure*}
}

\newcommand{\reactionsFig}{
\begin{figure*}[t]
  \centering
  \includegraphics[width=0.90\linewidth]{final_figures/reactions_facet7.pdf}
  \caption{\textbf{Analysts favor currently unsupported planning assistance}. \rr{Analysts saw on average 11.85 (std=4.56) suggestions, 9.85 (std=4.16) of which were planning suggestions}. All categories of \textit{intended} planning suggestions (which may include code to help execute a suggestion) were found to be helpful by at least some analysts, highlighting the need for planning assistance that current assistants lack. \rr{For planning suggestions which analysts could reasonably incorporate into their notebooks (i.e., those that were not \textit{results interpretation} and \textit{domain background}), analysts integrated suggestions 51.6\% of the time (47/91).} Analyst reactions varied within each category, with responses ranging from finding the assistance helpful to neutral, or even unhelpful in certain instances. Our interviews and observations suggest that the effectiveness of a suggestion is not solely determined by its suggestion category but also depends on various nuanced factors~(Sec.~\ref{sec:results}). We provide full examples of the raised suggestions in the appendix.
  % \tim{I didn't quickly find where you refer to this primarily. can it be closer to that?}
  }
  \Description{Two vertically stacked horizontal bar charts. The top chart is titled "Intended Planning Assistance". The y-axis is each suggestion category and the x-axis is count. Each category (y-axis tick) has three bars representing "Positive", "Neutral", and "Negative" reactions to the suggestion category. The bottom chart is titled "Intended Execution Assistance" and has one category, Execution Assistance, on the y-axis. }
  \label{fig:suggestion_reactions}
\end{figure*}
}

==> 0-macros.tex <==
\newcommand{\other}[1]{{\color{blue}{#1}}}
\newcommand{\ken}[1]{{\color{orange}{Ken: #1}}}
\newcommand{\eunice}[1]{{\color{olive}{Eunice: #1}}}
\newcommand{\tim}[1]{{\color{magenta}{Tim: #1}}}
\newcommand{\mgm}[1]{{\color{cyan}{Mgm: #1}}}
\newcommand{\jeff}[1]{\textcolor{blue}{Jeff: #1}}
\newcommand{\am}[1]{\textcolor{red}{[AM: #1]}}
% For Revise & Resubmit
\newcommand{\rr}[1]{{\color{black}{#1}}}

 \newcommand{\xhdr}[1]{\vspace{1.7mm}\noindent{{\bf #1.}}}

\usepackage{comment} % for long comments
\usepackage{xspace}
% For related work 

\newcommand{\interfont}{\fontfamily{cmss}\selectfont}
\newcommand{\githubURL}{\url{https://github.com/behavioral-data/Data-Assistant-Interface}}


\newcommand{\woz}{Wizard of Oz\xspace}
\newcommand{\litreview}{literature\xspace}

\newcommand{\mverselib}{\texttt{multiverse}\xspace}

\newcommand{\ourtool}{\textsc{Multiverse Debugger}\xspace}
\newcommand{\template}{\textit{template}\xspace}

\newcommand{\inlineheight}{0.5em}
% \newcommand{\inlineheight}{\fontcharht\font`\B}
\newcommand{\arrowConsidered}{%
  \begingroup\normalfont
  \includegraphics[height=\inlineheight]{final_figures/arrow-considered.png}%
  \endgroup
}

\newcommand{\arrowUnaware}{%
  \begingroup\normalfont
  \includegraphics[height=\inlineheight]{final_figures/arrow-unaware.pdf}%
  \endgroup
}


% For formative work
\def\cLatency{Finding bugs during the slow execution of a multiverse\xspace}
\def\cAggr{Diagnosing the source of a bug to a specific decision choice or set of choices\xspace}
\def\cDiff{Abstracting and propagating these changes to the rest of the multiverse\xspace}

% For consistent descriptions
\def\mincover{\textsc{decision cover}\xspace}
\def\errorLogAggregation{\textsc{error message aggregation}\xspace}
\def\diff{\textsc{universe-to-multiverse diff}\xspace}



% quote coloring
\usepackage{soul}
\newcommand{\hlc}[2][yellow]{{%
                  \colorlet{foo}{#1}%
                  \sethlcolor{foo}\hl{#2}}%
}
\newcommand\qt[1]{\hlc[Periwinkle!15]{``#1''}}

% For lab findings
\newcommand\shortquote[1]{\qt{\emph{#1}}}
\newcommand\longquote[1]{\qt{\emph{#1}}}
% \newcommand{\shortquote}[1]{#1}
% \newcommand{\longquote}[1]{#1}
% \newcommand{\shortquote}[1]{``\emph{#1}''}
% \newcommand{\longquote}[1]{\vspace{-1pt}\begin{quote}``\emph{#1}''\end{quote}}
\newcommand{\theme}[1]{\vspace{-1pt}\subsubsection{#1} }
\newcommand{\groupingtheme}[1]{\subsubsection{\textbf{#1}} }




==> 1-abstract.tex <==
\begin{abstract}
Data analysis is challenging as analysts must navigate nuanced decisions that may yield divergent conclusions. AI assistants have the potential to support analysts in \textit{planning} their analyses, enabling more robust decision making. Though AI-based assistants that target code \textit{execution} (e.g., Github Copilot) have received significant attention, limited research addresses assistance for both analysis execution \textit{and} planning. In this work, we characterize helpful planning suggestions and their impacts on analysts’ workflows. We first review the analysis planning literature and crowd-sourced analysis studies to categorize suggestion content. We then conduct a Wizard-of-Oz study (n=13) to observe analysts’ preferences and reactions to planning assistance in a realistic scenario. Our findings highlight subtleties in contextual factors that impact suggestion helpfulness, emphasizing design implications for supporting different abstractions of assistance, forms of initiative, increased engagement, and alignment of goals between analysts and assistants.

% Data analysis is challenging as analysts make nuanced decisions that can yield divergent conclusions \jeff{yes, but what specifically is "challenging" about this? and how might that help more concretely set up the potential of AI assistants?}. \tim{+1. We make it about planning assistance especially. perhaps we can connect to robust data science needing planning not only execution assistance. maybe sth like this sketch: AI assistants help w execution. However, diverging conclusions are a huge issue (and why) and addressing this challenge rquires planning assistance. Here we... } 
% AI assistants have the potential to support analysts in \textit{planning} their analyses, enabling more robust decision-making. In contrast to AI-powered code assistants (e.g., Copilot) which focus solely on code execution, little research exists on designing assistance for both analysis execution \textit{and} planning. In this work, we explore what characterizes a helpful planning suggestion and the impacts on analysts’ workflows. By reviewing analysis planning literature and examining analyses from a crowd-sourced analysis study, we establish a categorization of suggestion content. \tim{only content? or perhaps also other variables that matter?} Subsequently, we conduct a Wizard-of-Oz study (N = 13) to observe analysts’ reactions and preferences in a realistic scenario. 
% Our findings reveal the helpfulness of planning assistance depends on matching suggestion content and timing to an analyst’s background and goals \jeff{This does not seem surprising -- in that I think I would state this a priori. I wonder if we might surface more specific/detailed claims here?}, amongst other things. We conclude by discussing design implications for establishing common ground between the analyst and the assistant. 
\end{abstract}






% Data analysis is challenging as analysts must synthesize domain and statistical knowledge while making nuanced analytical decisions. As different analytical choices lead to divergent conclusions, analysts often struggle to draw reliable inferences. AI assistants can aid analysts navigate the analysis decision space and inform robust decision-making. In contrast to AI-powered code assistants (e.g. Copilot) which help with executing analysts' current analysis path (e.g., code completion), data analysis assistants can offer suggestions that facilitate analysis planning. This involves complex reasoning about previously made decisions, current and prior results, and alternative approaches. However, the suggestions' goals, content, and effects on analysts remain unclear. In this work, we explore what characterizes a helpful suggestion and the impacts of suggestions on analysts’ workflows. Through a literature survey and analysis of crowd-sourced analyses study, we create high-quality suggestions. We then raise these suggestions in a qualitative \woz study (N = 13). Our findings reveal \ken{todo} (insert specific finding here).

==> 2-intro.tex <==
% \tim{overall the paper is shaping up very nicely. it is fairly long and I highlighted a few densification opportunities. However we might need more. Integrating future work into design implications is the best larger move I see and recommend. perhaps we can check in with Jeff directly on what opportunities he sees. }

\section{Introduction}
\label{sec:intro}
Data analysis requires analysts to make numerous decisions regarding varied tasks, such as data collection, data wrangling, statistical modeling, and inference~\cite{Liu2019PathsEP}. 
Each choice involves \textit{analysis planning}, wherein analysts reason through the effects of potential decisions by synthesizing their results, prior experiences, and domain and statistical knowledge. 
Decisions made, their focus shifts to enacting these choices using the correct code with appropriate software tools, which we refer to as \textit{analysis execution}. After examining the outcome of their execution, the process repeats.
% Data analysis requires analysts to make many decisions across all phases of an end-to-end analysis (e.g., data collection, data wrangling, statistical modeling, inference, etc.)~\cite{Liu2019PathsEP}, and doing so involves analysis planning. \textit{Analysis planning} occurs when analysts reason through potential decisions to decide on subsequent analysis step(s). 
% or \tim{seems too narrow? what about when they forget a step and our assistant wants to bring that up?} 
% To inform their next decision, they synthesize current and past results with their own domain and statistical knowledge. Once analysts have made these decisions, their focus shifts to decision execution; \textit{analysis execution} involves implementing the decision using the correct code with appropriate software tools. 

% While execution and planning are both important, inadequate planning has significant negative ramifications.
% Researchers have identified poorly conducted analyses as a major contributor to the reproducibility crises \cite{Baker20161500SL}. Adding to the problem, analysis planning is challenging even to trained analysts. 
Inadequate analysis planning can complicate this flow and can cause analysts to risk making arbitrary and ill-founded decisions~\cite{Simonsohn2015SpecificationCD, Steegen2016IncreasingTT} for a host of reasons.
% foment \am{wc}unsubtantiate conclusions.
 % Inadequate analysis planning and execution can \am{wc}incur significant costs. 
% Lacking planning and sufficient execution skills, analysts risk making arbitrary and ill-founded decisions~\cite{Simonsohn2015SpecificationCD, Steegen2016IncreasingTT}.
% Analysts tendency ~\cite{Liu2019PathsEP, Liu2020UnderstandingTR} struggle to identify and address relevant decision points---potentially leading to unfounded conclusions. 
 Analysts often struggle to identify and address relevant decision points~\cite{Liu2019PathsEP, Liu2020UnderstandingTR}. 
 They may overfocus on low-level details, such as tuning hyperparameters, or miss high-level considerations like alternative statistical or mental models~\cite{Liu2020UnderstandingTR}.
 % , deprioritizing planning altogether. 
 They often center execution decisions tied to familiar workflows when approaches using other tools may be more applicable~\cite{Liu2020UnderstandingTR, Jun2021HypothesisFE}.
 % In this case, barriers to the execution of other decisions lead analysts to focus only on the most comfortable approaches. 
% 
% Since different decisions can lead to different conclusions, 
Further, the unconsidered flexibility in decision-making (and the biases inherent therein) contributes to the scientific reproducibility crisis~\cite{Baker20161500SL, Cockburn2020ThreatsOA, Aarts2015EstimatingTR}. 
% \jeff{Is this really a "trend"? Seems more to me to likely be a longstanding challenge we are now better putting into relief} \tim{+1. others call it a reproducibility crisis} 
For instance, given the same analysis task and dataset, analysts often derive divergent conclusions \cite{Silberzahn2018ManyAO, Breznau2022ObservingMR, Schweinsberg2021SameDD, Dutilh2018TheQO, BotvinikNezer2019VariabilityIT, Bastiaansen2019TimeTG, Menkveld2021NonStandardE}. 
% Furthermore, their inattention to key missed steps or alternative methods may make them overconfident in their findings. 
% All of this can lead to an insufficient \tim{misleading?} analysis, something researchers have identified as a major contributor to the reproducibility crisis in science \cite{Baker20161500SL}. \tim{can move the crisis up top of paragraph}

% and which leads to suboptimal decision making in industry and government. \ken{is it just industry? what about government?}.

% note to self: reproducibility crisis and divergent conclusions are two different but similar things
\textit{Data analysis assistants} seek to bridge these gaps by helping analysts execute \emph{and} plan their analyses. 
% \textit{Data analysis assistants} may improve analysts’ ability to design and enact decisions by offering execution \textit{and} planning assistance.
AI-based execution assistants (such as Copilot~\cite{githubcopilot}) help analysts implement decisions (Fig. \ref{fig:teaser}A) by suggesting code or tools. 
In contrast, planning assistance may help them reason about their decisions (Fig. \ref{fig:teaser}B and C), 
articulate hypotheses and mental models, and identify overlooked alternative decisions or rationales (Fig. \ref{fig:teaser} \arrowUnaware).
% Prior work~\cite{Liu2020BobaAA, Simonsohn2015SpecificationCD, Steegen2016IncreasingTT} indicates that systematically considering these alternative approaches could deepen analysts' understanding of the variations in outcomes inherent in their decisions. Hence, planning assistance can be seen as a pivotal step in promoting more theoretically principled, comprehensive, reliable, and therefore more robust analyses.
Systematically considering alternatives can deepen analysts' understanding of the outcome variations latent to decision-making in data analysis~\cite{Liu2020BobaAA, Simonsohn2015SpecificationCD, Steegen2016IncreasingTT}. 
% Systematically considering alternative approaches can deepen analysts' understanding of the variations in outcomes latent to their decisions~\cite{Liu2020BobaAA, Simonsohn2015SpecificationCD, Steegen2016IncreasingTT}. 
Therefore, planning assistance can be a transformative step towards more principled, reliable, and robust analyses.
% With quality assistance of both types, analysts can confidently select and accurately carry out their decisions. Altogether, such assistance may enable analysts to draw more reliable inferences. 
% 

 % LLMs are linguistic feed-forward machines that predict future text from past text \cite{Vaswani2017AttentionIA}. Thus, they are well suited to tasks in which the desired outcome is clear based on the textual context and are well-equipped for execution assistance. LLM-based code assistants like Github Copilot \cite{githubcopilot}recommend relevant code based on what the programmer has written so far (Fig. \ref{fig:quadrant}A and B). 
 % Given this functionality, LLM-powered code assistants have become increasingly popular in modern code environments. 
 % Similarly, LLM-powered analysis assistants can be tightly integrated into analysts' computational environments such as computational notebooks. 
% Similarly, LLM-based analysis assistants could in theory provide insightful recommendations for analysis planning.
 
\quadrantFig

The improved capabilities of large language models (LLMs) for coding, language, and visualization generation \cite{Brown2020LanguageMA, Bubeck2023SparksOA, Chen2021EvaluatingLL, Chowdhery2022PaLMSL, Dibia2023LIDAAT} offer an opportunity to make such planning \emph{and} execution data analysis assistants a reality.
Prior LLM-based assistants have explored practical approaches to execution assistance~\cite{Jiang2021GenLineAG, Vaithilingam2022ExpectationVE, Barke2022GroundedCH, McNutt2023OnTD, Ziegler2022ProductivityAO, Gu2023HowDA}, however planning remains unexplored (Fig.~\ref{fig:quadrant} bottom row).
% \am{finish sentence}.
% Prior research has explored the design and impacts of execution assistance from LLM-based code assistants \cite{Jiang2021GenLineAG, Vaithilingam2022ExpectationVE, Barke2022GroundedCH, McNutt2023OnTD, Ziegler2022ProductivityAO}. 
% However, additional challenges arise when considering the design of an assistant that offers both execution \textit{and} planning assistance.
% Existing assistants do not easily facilitate planning assistance (Fig.~\ref{fig:quadrant} bottom row): 


Effective planning suggestions can not be achieved by simply feeding the current analysis context into an LLM as it requires selective context, higher-level scaffolding, targeted prompts, and sensitive triggers.
The iterative nature of data analysis demands the nuanced interpretation of prior results, statistics, and domain knowledge to inform the subsequent decisions \cite{Grolemund2014ACI, Box1976ScienceAS, Jun2021HypothesisFE, Tukey1966DataAA}, which is typically unaccounted for in execution-only assistants (Fig. \ref{fig:quadrant}A and B). 
Synthesis of such decisions may require backtracking to a prior choice and deviating from the current approach (Fig.~ \ref{fig:teaser}).
Authoring effective prompts can be difficult~\cite{ZamfirescuPereira2023WhyJC, Mishra2022HELPMT}, and the right context to provide to not cause hallucinatory analyses~\cite{mcnutt2020surfacing} may be hard to identify.
Finally, data analysis is a non-linear activity that involves iterated and inter-woven actions of typing, reading, and reflecting---making the optimal timing of suggestions less clear than in software engineering.
% That is, proper planning assistance then cannot be supported through naive applications of LLMs as it requires selective context, higher-level scaffolding, targeted prompts, and sensitive triggers.



% Yet, numerous questions about the design of planning assistants are unanswered. 
% How distant can suggested alternative pathways be and still be useful? How do analysts experience planning suggestions and interventions? How do we make effective suggestions amongst the vast space~\cite{Gelman2014TheSC, Gelman2019TheGO, Simmons2014DataFP} of decision-making approaches? 
% Should assistants help analysts consider adding statistical tests (planning), think through approaching an independent variable differently (planning), or implement a statistical model (execution)? We lack knowledge of what characterizes a helpful suggestion. 
% To the best of our knowledge, no such systems exist to date.
% When providing a planning suggestion, an assistant must reason both \textit{backward} through analysts' steps and \textit{forward} into alternative approaches. It may also require backtracking to a prior decision and deviating from an analyst's current plan (Fig.~ \ref{fig:teaser}). Thus, unlike current assistants for execution assistance (Fig. \ref{fig:quadrant}A and B), it is insufficient simply to feed the current analysis context into an LLM and recommend a continuation of the current workflow. 

% Further, though analysts could directly ask an assistant for planning assistance (Fig. \ref{fig:quadrant}C), doing so would require them to be aware of what they need and how to write effective prompts~\cite{ZamfirescuPereira2023WhyJC, Mishra2022HELPMT}. Since data analysis involves non-linear reasoning and iteration, they may struggle with selecting the relevant context to pass to the assistant. 
% % \tim{I feel like this assumes that the LLM would be able to do it if it just had the right context. Do we think that's true? Should we make that more explicit?}\ken{To me, this is only one problem amongst a few other problems which we mention below. Other problems involve the data correct data source of the LM for example} 
% Better solutions would put less burden on the analyst and facilitate this process.
% Additionally, because analysts may often miss important considerations in their analyses, it is important for data analysis assistants to identify critical missed ideas (Fig. \ref{fig:quadrant}D).  
% \tim{maybe even more strongly worded? We know people miss lots of important considerations and the only way to recover this is for the assistant to take initiative and point out critical missed considerationss.} 
% It is also unclear how to best choose the optimal timing and form of assistance.
% tim{only timing or also the how/where etc?}\ken{are we basing this off of our results or what we know before again.}, as opposed to code assistants like Copilot, which are almost always active.\tim{not sure how almost always active relates to  the previous context of the sentence} 
% To summarize, proper planning assistance cannot be supported through naive applications of LLMs alone. At the very least, it requires additional and selective context, higher-level scaffolding, targeted prompts, and assistance triggers. To the best of our knowledge, no such systems exist to date.

% To form an effective assistant broader questions about the interaction between analysts and data analysis assistants must be explored. As planning assistance requires an analyst to consider approaches outside their immediate workflow, an assistant could potentially suggest alternatives that do not align with the analyst's current intent. Second, it remains unclear what preferences analysts have for assistant-initiated suggestions and interventions. Third, given the tremendous flexibility in analysts' decision-making approaches~\cite{Gelman2014TheSC, Gelman2019TheGO, Simmons2014DataFP}, there can be many specific suggestions an assistant could provide at any given moment, and which to choose in what situation is unclear. 
% For instance, should the assistant help an analyst think through performing a statistical test (planning), consider operationalizing an independent variable differently (planning), or implement a statistical model (execution)? Finally, we lack basic knowledge of elements that characterize a helpful suggestion. 

% It is unclear what characterizes a helpful suggestion and under what situations a suggestion is helpful. Likewise, prior to understanding the contextual factors for why suggestions are helpful, it is necessary to identify suggestion content that \textit{could} be helpful. 


% At the core of this uncertainty is striking a balance between execution and planning assistance. These two facets of assistance must be effectively integrated to provide comprehensive support for data analysis tasks. 

% \tim{seemed unfinished. maybe say: that this requires the assistant to prioritize and these may vary from analyst to analyst? (but I suppose we don't want to take away our findings here, e.g. need for common ground and personalization)}


% We identify the following challenges in providing both execution and analysis assistance \ken{are these just research questions but more precise?}]
% \begin{description}
% \item[Challenge 1] --- As suggestions may completely deviate from analysts current working context, it is unclear what the space of possible suggestions should be.
% \item[Challenge 2] --- As there exist different forms of initiation (e.g., user-initiated vs. assistant-initiated) and assistance (planning vs. execution assistance), it is unclear what analysts actually find helpful when working through an analysis.
% \item[Challenge 3] --- Given assistance may be offered even when analysts may not ask for it, it is unclear how suggestions impacts an analysts' workflow.
% \end{description}

% Due to the specific challenges of data analysis planning, there needs to be careful consideration of the interfaces, interactions, and processes behind creating and providing planning suggestions. Importantly, it is not obvious what characterizes a helpful suggestion and how suggestions impact an analyst’s workflow. Little is known about what content planning assistance is even comprised of.  
% \tim{here or in RQ3  we need to say a few more words about what "impact workflow" means. what are you looking for? what would be a success?}
% \tim{this paragraph overlaps with end of previous one: "it is unclear"... I wonder whether you can consolidate to tighten?}

% \tim{what are CHI norms re length? how common is 30ish pages?}

Yet, essential questions about the design of planning assistants remain unanswered.
In this work, we explore the design of such AI-based  assistants.
% , in addition to more familiar execution help. 
% Since execution assistance is relatively well-explored and planning assistance less well so, we focus on understanding the interfaces, interactions, and processes for effectively incorporating planning assistance into analysts' workflows. 
To this end, we consider the following research questions:
\begin{description}
\item[RQ 1 - Scope:] What types of specific planning assistance content could an assistant provide?
% As there are many situations that may benefit from analysis planning, what content of types of specific planning feedback should an assistant provide?
\item[RQ 2 - Helpfulness:]
% As there are different methods of interaction (e.g., user-initiated vs. assistant-initiated), forms of assistance (i.e., planning vs. execution assistance), and specific suggestions under each type of assistance (e.g., modeling or data wrangling during planning), 
% What types of suggestion content do analysts find helpful? Are there other characteristics that make a helpful suggestion?
What data analysis suggestions do analysts find helpful and under what circumstances?
\item[RQ 3 - Impact:] How do suggestions impact analysts’ workflows? To what extent do analysts prioritize their own ideas or adopt suggestions and explore alternative approaches?
% Do analysts take the suggestions over their own ideas and consider alternative approaches more frequently? \tim{unsure about second sentence - what else do we consider? perhaps whenever suggestions DO NOT get considered? right now this example question seems to "bias" our inquiry. Can you make it broader or more balanced to what you do the most or what readers to  take away?}
\end{description}


To characterize assistant suggestion content (\textbf{RQ 1}), we conducted a \litreview review and critically assessed data from a crowd-sourced analysis study~\cite{Silberzahn2018ManyAO}, wherein 29 analyst teams separately analyzed the same dataset to answer the same research question (Sec. \ref{sec:suggestions}). 
We used these findings to develop \textit{categories of assistance content} across points in the end-to-end analysis process (Table \ref{tab:suggestions}).
% By studying the literature, we identify challenges analysts face and broad categories of assistance opportunities. Likewise, by observing variations in independent analysis approaches in the crowd-sourced analysis study, we identify situations where analysts would benefit from being offered alternative approaches or reminders for key analysis steps. This process helped us develop \textit{categories of assistance content}
% % \tim{this sounds broader than the "suggestion content" mentioned in the abstract} 
% across points in the end-to-end analysis process (Table \ref{tab:suggestions}).

To observe analysts' preferences for (\textbf{RQ2}) and effects of (\textbf{RQ3}) different suggestions, we conducted a \woz study, with 13 practicing data analysts (Sec. \ref{sec:labstudy})---our first contribution. We designed the study around the scenario considered in the crowd-sourced study~\cite{Silberzahn2018ManyAO} that we looked at in our previous step.
Our participants worked through the same dataset and task while receiving suggestions from a behind-the-scenes experimenter acting as a wizard.
% , which allowed us to simulate high-quality and relatively low-latency feedback. 
% to elicit discussion about the helpfulness of a suggestion and observe factors influencing the analyst-assistant interaction. 
% Instead of evaluating the quality of an analysis assistant that is likely to be imperfect, we focus on studying how these assistants should be designed in the first place. We build on prior works on the design of code-assistants in computational notebooks \cite{McNutt2023OnTD}, and guidelines in Human-AI interaction \cite{Amershi2019GuidelinesFH, Horvitz1999PrinciplesOM}.
To facilitate our study, we developed a JupyterLab extension that allowed the wizard to surface suggestions to the participant as they used the notebook in a familiar manner\footnote{To support future notebook assistant interfaces, we release the code for this interface at \githubURL. }. 
% to act as planning assistant (aided by contemporary LLMs). 
% For the study, we developed a prototype of an analysis assistant’s interface and associated interactions. 
% We also created a wizard protocol that was not limited by current assistants and LLMs to elicit findings and design implications for LLM-based analysis assistants of the near future; we used current LLMs to generate and iteratively refine suggestions. 
This allowed the wizard (aided by LLMs) to synthesize suggestions and manipulate the selection, quality, and timing of recommendations (Fig.~\ref{fig:woz}). 
% Furthermore, we developed specific high-quality examples of suggestions for each category of assistance (Table~\ref{tab:suggestions}).

% To encourage findings around LLM-powered analysis assistants of the near future and not be limited by capabilities of current LLMs, we create a wizard protocol intimately tied to but not restricted by existing LLMs. \ken{My attempt} \tim{rephrase, in which ways is it tied? what do we want to communicate here? i havven't found the right language yet. On the one hand it should be around capabilities that LLMs may be able to support in the future. on the other hand we intentionally didn't want to restrict it by the limitations of current LLMs as well} 

% We conducted our \woz study with 13 analysts (Sec. \ref{sec:labstudy}) who were familiar with data analysis and had a background spanning a wide range of academic disciplines (Table~\ref{tab:participants}).
% \tim{say something about the participants. ... that span different areas of data science and domain expertise. s}. 
% Analysts worked through the same dataset and task as that of the crowd-sourced analysis study, which allowed us to simulate high-quality and relatively low-latency feedback. 
% \tim{, which allowed the wizard to simulate high-quality feedback and suggestions at relatively low latency?}.
% Concurrently, the wizard presented them with execution and planning suggestions. 

% In the findings of our study (Sec. \ref{sec:results}), we observed that analysts consistently favored execution assistance \tim{i wonder whether we can say this differently. it sounds like we describe planning for two pages and then say they didn't care about it. can we make that more nuanced / not undermine the planning importance. e.g. we could say that analysts are often under pressure to a degree that analysis planning is often ignored/simplified/missed and execution support is always welcome.} while having more nuanced reactions toward planning assistance.
We synthesize the findings of our study (Sec. \ref{sec:results}) into a set of design guidelines (Sec.~\ref{sec:discussion}) to align analysis intent and goals, support varying levels of suggestion assistance, and increase analyst understanding and engagement with the assistant's suggestions---our second contribution.
% Among study findings (Sec. \ref{sec:results}), 
We observed that the data analysis process can benefit from diverse forms of planning assistance, but only with careful consideration of assistance context. 
Additional factors---such as the timing of suggestions or variations in analysts' statistical and domain backgrounds---played a critical role in a suggestion's perceived helpfulness. Finally, we found differences in goals between the analyst (i.e., speed and completion) and planning assistance (i.e., methodical and robust planning).
% By characterizing these usability concerns, we hope to make planning-equipped data analysis assistants practical and effective, and thereby make data analysis more robust and reliable.

By characterizing the usability of planning-equipped analysis assistants, we seek to make data analysis more robust and reliable by enabling richer and more useful assistants.
% \am{by doing this we change the world or whatever}

% \tim{missing, say that you conduct the woz study, and what comes after (say thematic analysis of qualitative feedback etc etc.}


% The primary contributions of this paper include: 
% % The paper contributes the following:
% \begin{enumerate}

% % \item A categorization of data analysis planning suggestion content 
% % \item An open-source data analysis assistant interface prototype integrated into JupyterLab
% \item Findings from a \woz study that reveal multiple interacting factors that influence the helpfulness of data analysis planning assistance  
% \item Design guidelines for incorporating planning assistance
% % and execution assistance \tim{bit confusing to now see execution here again while we highlighted planning before. IIRC we do not highlight that these are intertwined in intro} 
% in a data analysis assistant (Table~\ref{tab:design_implications})

% \end{enumerate}



% In addition, we release the code for our assistant interface prototype used in the \woz study.\footnote{Github}



==> 3-related-work.tex <==
\section{Background and Related Work}
\subsection{Planning in Data Analysis}
\label{sec:bg_planning}
% In an interview study with professional data analysts, Alspaugh et al. \cite{Alspaugh2019FutzingAM} describe how analysts often engage in activities related to planning their analysis approach. 
Analysts often engage in planning activities~\cite{Alspaugh2019FutzingAM}. Such activities are closely related to cognitive theories of \textit{sensemaking}, whereby analysts seek and integrate new observations to build mental models~\cite{Pirolli2007TheSP, Russell1993TheCS, Klein2007ADT} that inform their decisions for collecting and analyzing data to elicit findings; these findings, in turn, inform their mental models in an iterative back-and-forth.
Thus, data analysis planning can be highly iterative and often requires revisiting decisions at various points in the analysis~\cite{Jun2021HypothesisFE, Box1976ScienceAS, Tukey1966DataAA}. 
Moreover, these processes are integral to reduce human biases in decision-making and help form robust conclusions \cite{Grolemund2014ACI}. In this work, we study how sensemaking activities in analysis planning can be improved with an AI assistant.


Similarly, analysis planning relates closely to \textit{multiverse analysis}~\cite{Steegen2016IncreasingTT, Simonsohn2015SpecificationCD}, a statistical analysis paradigm whereby analysts consider, specify, and report all reasonable decisions and combinations of decisions. Through assessing potentially thousands of analyses based on these choices, a multiverse approach highlights how different decisions can influence final outcomes. Despite the importance of analysis planning, empirical studies observed analysts struggle to reason about their analysis decisions \cite{Liu2019PathsEP, Liu2020UnderstandingTR}. Often, they are unaware of potential alternative decisions in the end-to-end data analysis process.
% (i.e., the phases of data collection, data wrangling, statistical modeling, and evaluation). 
Our work aims to guide analysts in recognizing, understanding, and reflecting on these overlooked but important decisions. 

Prior work developed systems to simplify the planning of statistical models and statistical tests~\cite{Jun2022TisaneAS, Jun2019TeaAH}. Data-driven systems (like Lodestar~\cite{Raghunandan2022LodestarSI}, EDAssistant~\cite{Li2021EDAssistantSE}, and ATENA \cite{El2020AutomaticallyGD}) add structure to analyses and offer recommendations for data science and exploratory data analysis (EDA) workflows. However, these systems focused on specific parts of the analysis process (e.g., modeling or EDA) or based their recommendations on predicting the next steps in an analysis. In contrast, \textit{we emphasize analysis planning for the entire end-to-end analysis and as a highly iterative process}. 

Specifically, we aim to support analysts in considering alternative decisions and revisiting prior decisions as new insights emerge. We view LLM-supported data analysis assistants as a promising solution. Furthermore, these assistants could be integrated with existing multiverse analysis systems~\cite{Liu2020BobaAA, Sarma2021multiverseMA, Gu2022UnderstandingAS}. % to help analysts conduct multiverse analyses. 
Thus, as planning assistants help analysts consider and structure alternative decisions, multiverse tools help them author, execute, and evaluate these decisions within a ``multiverse'' of alternative analyses.

For these benefits to be realized, we must learn what specific feedback analysts need and under what circumstances assistance would be most useful to them. To begin exploring factors that influence favorable suggestions, we first categorize suggestion content (Sec. \ref{sec:suggestions}). Using this categorization, we develop a prototype interface and conduct a \woz study (Sec. \ref{sec:labstudy}) to investigate the helpfulness and impact of such suggestions.

% With LLMs' capability to generate coherent code and text, the assistant can offer information on relevant domain knowledge and statistical concepts, along with precise code implementation.

% \tim{again, this is a nice similarity but it is critical for you do highlight significant differences, additional contributions and why they are super important in all of the sections if not paragraphs here.}

\subsection{LLM-based Assistants and Limitations for Planning Assistance}
\label{sec:llm_background}

% Modern programming assistants like Github Copilot utilize the strong text generation abilities of Large Language Models (LLMs). These LLMs are trained on extensive text corpora, often sourced from the web \cite{Brown2020LanguageMA, Zhang2022OPTOP}. 

LLMs trained on large-scale code corpora \cite{Chen2021EvaluatingLL, Chowdhery2022PaLMSL, Fried2022InCoderAG, Nijkamp2022ACP, Li2022CompetitionlevelCG} have shown proficiency in learning programming concepts, solving programming challenges \cite{Chen2021EvaluatingLL}, and covering various domains like web development \cite{Zhang2023PracticesAC} and data science problems \cite{Lai2022DS1000AN, Chandel2022TrainingAE}. While these LLMs excel at precise code implementation tasks (e.g., \textit{Consider a (6,7,8) shape array, what is the index (x,y,z) of the 100th element?} \cite{Lai2022DS1000AN}), this work focuses on situations where the problem statement and methods to apply are less clear, unspecified by the user, or at a higher level of abstraction. 
% \tim{is that it? or could it just be broader, or specified on a much higher level of abstraction?}

% Modern programming assistants such as Github Copilot are enabled by the strong text generation abilities of Large Language Models (LLMs). These LLMs are trained on vast corpora of text, often taken from the web \cite{Brown2020LanguageMA, Zhang2022OPTOP}. In particular, LLMs trained on large-scale code corpora \cite{Chen2021EvaluatingLL, Chowdhery2022PaLMSL, Fried2022InCoderAG, Nijkamp2022ACP, Li2022CompetitionlevelCG} have been shown to learn programming concepts, solve programming challenges \cite{Chen2021EvaluatingLL}, and cover a range of task domains from web development \cite{Zhang2023PracticesAC} to data science problems \cite{Lai2022DS1000AN, Chandel2022TrainingAE}. However, the tasks these LLMs address all involve very specific problem statements asking for precise code implementation (e.g., \textit{Consider a (6,7,8) shape array, what is the index (x,y,z) of the 100th element?} \cite{Lai2022DS1000AN}). In contrast, this present work addresses common situations when the problem statement is less clear or even unspecified by the user. % \tim{if they can do DS problems -- why are they still insufficient or not well enough understood as we claim here?}

LLMs are trained to predict the next token in a code/text sequence and thus form the back-end of many popular code assistants that offer execution assistance \cite{Murali2023CodeComposeAL, githubcopilot, googleblog2022, codewhisperer}. Note that we distinguish between an LLM and an assistant; the latter is a \textit{complete system} that acts as the interface between the user and the LLM. Existing code assistants typically pass the programmer's context (e.g., code, comments, etc.) to the LLM to then recommend entire statements or blocks of code. In this interaction, programmers can either initiate execution assistance with explicit comments and triggers (Fig. \ref{fig:quadrant}A) or passively let the assistant auto-complete their code (Fig. \ref{fig:quadrant}B). However, as discussed earlier  (Sec.~\ref{sec:intro}), assistants offering data planning assistance cannot naively pass the current context to an LLM given the iterative and non-linear nature of analysis planning. 
% \tim{say why -- the why is more important than the  fact you explained it before}\ken{we went thorough in this in intro and find that we would be repeating ourselves here. This was part of the densification discussed earlier}. 
This work explores the design of an LLM-supported complete system for planning assistance. 

% At their core, LLMs are trained to predict the next token in a code/text sequence. Based on this idea, LLMs form the back-end of many popular code assistants that offer execution assistance \cite{Murali2023CodeComposeAL, githubcopilot, googleblog2022, codewhisperer}. Note, we make the distinction between an LLM and an assistant, which is a full-fledged system around the LLM acting as the interface between the user and the LLM. With existing code assistants, they typically pass the programmer's context (e.g., code, comments, etc.) to the LLM to then recommend entire statements or blocks of code. Within this interaction, programmers can either initiate execution assistance with explicit comments (Fig. \ref{fig:quadrant}A) or passively let the assistant auto-complete their code (Fig. \ref{fig:quadrant}B). In data analysis, however, suggestions to help reason about analysis decisions (i.e., planning assistance) may require backtracking to points much earlier in the analysis and can deviate from the analyst's immediate context \cite{Liu2019PathsEP, Grolemund2014ACI}. As a result, unlike existing code assistants, data analysts assistants when offering planning assistance cannot naively pass the current context to an LLM. \tim{add a last sentence about what your work adds here} \tim{move figure closer to here}


% The assistants include additional interfaces and interactions between the user and the LLM.


More recently, general-purpose LLMs, such as InstructGPT \cite{Ouyang2022TrainingLM} and GPT-4 \cite{OpenAI2023GPT4TR}, 
have reached a level of performance that is now deployable in various contexts and domains~\cite{Bubeck2023SparksOA}.
% have achieved human-level \tim{i hesitate to call it that since it's easily misleading. is there a good other way to specify the level of performance?} performance across many difficult tasks in various domains \cite{Bubeck2023SparksOA}.  
% They are fluent in human-style conversations and can naturally engage in multi-turn conversations with the user.
The assistant ChatGPT~\cite{ChatGPT}, supported by LLMs, has exploded in popularity \cite{statista}. In the context of data analysis, ChatGPT can offer basic planning assistance, integrating broader domain expertise, software libraries, and statistical knowledge with code when given precise instructions (e.g., \textit{Show me the correlation between Height and Weight in a scatter plot})~\cite{Cheng2023IsGA}.

However, ChatGPT requires users to actively prompt it for information (Fig.~\ref{fig:quadrant}C). Prior work found that non-AI experts often struggle to write effective prompts \cite{ZamfirescuPereira2023WhyJC} and experience significant cognitive load~\cite{Jiang2022PromptMakerPP}. Data analysis planning can further exacerbate this issue since analysts must synthesize information from various points in the analysis to pass to the assistant. Thus, the burden is on the analyst to decide what they want, where to find relevant context in a likely messy analysis \cite{Head2019ManagingMI, Kery2018TheSI, Rule2018ExplorationAE}, and craft a prompt or series of prompts. In addition, since analysts are often unaware of the entire space of analytical decisions, they may also need planning assistance they do not directly ask for. However, current assistants like ChatGPT do not naturally support assistant-initiated planning assistance (Fig. \ref{fig:quadrant}D). 
Further, since analysts may be alternating between planning and execution, the optimal timing of planning assistance is unclear. 
% Given all these challenges, current LLMs cannot be naively employed for planning assistance. 

Our work aims to understand the design of data analysis assistants that involve all forms of assistance and initiation. Since planning assistance presents new and largely unexplored challenges, we focus our efforts here. Notably, we monitor analysts' reactions to an assistant that offers new planning information that possibly differs from their current analysis context (i.e., analysis code and notes). In accomplishing this, we also explore an assistant that raises suggestions without direct invocation from the analyst. 


\subsection{Designing for Human-AI Interaction}
In general, designing AI-based user-facing systems is challenging since designs must face issues that include explainability \cite{Liao2020QuestioningTA, Kim2022HelpMH}, trust \cite{Kunkel2019LetME, Liao2022DesigningFR, Toreini2019TheRB}, user control \cite{Shneiderman2020HumanCenteredAI, Horvitz1999PrinciplesOM}, and user expectations \cite{Luger2016LikeHA, Kocielnik2019WillYA}. As a result, there is a rich history of literature on design guidelines for Human-AI interaction to address these challenges \cite{Horvitz1999PrinciplesOM, Amershi2019GuidelinesFH}.
Similar practitioner-facing guidelines have also been released in large companies \cite{PAIRGuidebook, appleML, IBMDesignAI}. 

% Horvitz's foundational work on mixed-initiative user interfaces  outlined principles for having humans and automated services interact effectively \cite{Horvitz1999PrinciplesOM}. Twenty years later, Amershi et al. \cite{Amershi2019GuidelinesFH} built on Horvitz's set of principles and formulated 18 generally applicable guidelines for Human-AI interaction. 
% In creating these guidelines, Amershi et al. explored AI products and guidelines in industry and academic literature about AI design. They also went through multiple phases of evaluation and refinement to create the final set. \tim{maybe unnecessary detail} 
% Similar practitioner-facing guidelines have also been released in large companies \cite{PAIRGuidebook, appleML, IBMDesignAI}. 

Though these resources address common challenges in Human-AI interaction design, designing a system still requires support for domain-specific examples and proper problem formulation \cite{Yildirim2023InvestigatingHP}.
In other words, these resources do not address the specific Human-AI interaction challenges surrounding the design of data analysis assistants (e.g., the timing of assistant-initiated planning assistance).
% \tim{can we say that they don't and perhaps provide evidence or an example?}
Our work focuses exclusively on identifying precise goals and problems for designing analysis assistants. Based on findings from a \woz study, we propose design guidelines specifically for developing these assistants (Table~\ref{tab:design_implications}). 

% With respect to designing assistants for data analysis, McNutt et al. \cite{McNutt2023OnTD} studied the design of AI-powered code assistants in computational notebooks. Their work focused on the computational notebook as a medium to provide execution assistance. They conducted an interview study and presented analysts with slide-based prototypes of interfaces. 
With respect to designing analysis assistants, McNutt et al. \cite{McNutt2023OnTD} studied computational notebooks as a medium to provide AI-based execution assistance for data scientists. They conducted an interview study and presented participants with slide-based prototypes of interfaces.
In contrast, our work concentrates on the open challenges in understanding the scope of (Sec.~\ref{sec:suggestions}) and developing for (Sec.~\ref{sec:discussion}) planning assistance.
% , we take extra consideration into studying planning assistance. \tim{extra consideration sounds very vague...} 
Instead of focusing on the medium where the assistant resides, we focus on identifying factors that make assistance helpful.






==> 4-suggestions.tex <==
\section{Categorizing Suggestion Content}
\label{sec:suggestions}

\tableSuggestions


To identify the circumstances in which planning suggestions are helpful (\textbf{RQ 2}), we first establish categories of relevant suggestion content (\textbf{RQ 1}). In our subsequent \woz study (Sec.~\ref{sec:labstudy}), we use this categorization to derive suggestions and observe analysts' reactions and preferences.
% under a realistic analysis setting. 
% 
We conducted a literature review 
% \tim{conduct a literature review? given that we end up w six papers and do not conduct a formal, comprehensive lit review I think we should try to find a different name for this. How about "theory driven"?} 
to identify existing challenges data analysts face. We then examined results from a crowd-sourced analysis study, where multiple independent analysts made decisions given the same data and research question. This helped us understand variations in  decision-making, determine points where alternative approaches would be plausible, and observe what these approaches might look like. 
% From studying a crowd-sourced analysis study, we build specific, highly-relevant examples of planning suggestions. 
% Our investigation offers a categorization of data analysis assistance content. 

 % \tim{readers may not know what this means. you need to explain that this is an ideal scenario where you observe the process and decision making of multiple independent analysts and that this helps to understand the variation in decision making and what alternative approaches are plausible. }
\subsection{Literature Review}
We began by identifying works that study the data analysis process and present opportunities for assistance. We searched Google Scholar with the keywords "sensemaking data analysis" from which we iteratively snowball sampled~\cite{Wohlin2014GuidelinesFS}. 
% \tim{would everyone understand that this is presumably done via references?}. 
We sought papers that discussed the end-to-end data analysis process and challenges suitable for a text-based assistant. 
% Because planning assistance is less understood and often has no invocation/guidance from the analyst, we direct our efforts toward this.
 Therefore, we did not focus on problems with specific systems \cite{Shrinivasan2008SupportingTA, Kang2012ExaminingTU} or address common analysis challenges related to software and debugging \cite{Kandel2012EnterpriseDA, Chattopadhyay2020WhatsWW, Gu2022UnderstandingAS}, communication \cite{Zheng2022TellingSF, Wang2021DocumentationMH}, and data provenance \cite{Kery2018TheSI, McNutt2023OnTD, Xu2015AnalyticPF}. 


Our review resulted in 15 publications that addressed data analysis in various domains (e.g., food delivery, education, medical imaging, etc.), analysis tasks, and groups of data workers (e.g., enterprise workers, researchers, college students, etc.). From these works, we conducted thematic analysis on excerpts describing data analysis challenges and identified broad categories of assistance. 
 % \jeff{Only six papers? Can we more clearly indicate how we identified these and ruled out any others?} 
 These included: \textit{domain expertise information} \cite{Jun2021HypothesisFE, Liu2020UnderstandingTR, Wongsuphasawat2019GoalsPA, Boukhelifa2017HowDW, Wild1999StatisticalTI}, \textit{additional statistical knowledge} \cite{Jun2021HypothesisFE, Liu2019PathsEP, Liu2020UnderstandingTR}, \textit{guidance for statistical modeling} \cite{Jun2021HypothesisFE, Huber2011DataAW, Wild1999StatisticalTI, Bissell1988ProblemSA, Grolemund2014ACI}, \textit{guidance for analysts' hypothesis derivation} \cite{Jolaoso2015TowardAD, Battle2019CharacterizingEV, Kang2011CharacterizingTI, Alspaugh2019FutzingAM}, \textit{alternative decisions} \cite{Liu2019PathsEP, Liu2020UnderstandingTR, Kale2019DecisionMakingUU}, and data analysis specific \textit{execution assistance} \cite{Raghunandan2022CodeCE, Liu2020UnderstandingTR, Wongsuphasawat2019GoalsPA, Jun2021HypothesisFE, Alspaugh2019FutzingAM}.  
 We then refined these categories by comparing independent analyses from a crowd-sourced analysis study, described next.

\subsection{Behavior-Driven Analysis of a Crowd-Sourced Data Analysis Study}
\label{subsec:crowdsourced_study}
In crowd-sourced data analysis studies \cite{Silberzahn2018ManyAO, Breznau2022ObservingMR, Schweinsberg2021SameDD, Dutilh2018TheQO, BotvinikNezer2019VariabilityIT, Bastiaansen2019TimeTG, Menkveld2021NonStandardE}, numerous independent teams of analysts conduct analyses answering the same research question with the same dataset. Though originally intended by authors to study variations in analytical choices and how they impact analysis conclusions, these studies also offer high-fidelity data about code and rationales behind analysts' decisions. 

In this work, we chose a crowd-sourced study \cite{Silberzahn2018ManyAO} that addresses the research question: \textit{Are soccer players with a dark skin tone more likely than those with a light skin tone to receive red cards from referees?} The study provides a real-world dataset for answering the research question and includes analyses from 29 teams of analysts. The question and dataset are of moderate practical difficulty and complexity, encouraging different but reasonable analytical approaches. Furthermore, the domain of the study, soccer, is approachable to general audiences, reducing the likelihood of substantial differences in analysts' domain expertise.

We analyzed the soccer dataset for alternative approaches to an analysis decision at any point in the analysis process (e.g., data wrangling, statistical modeling, inference, etc.). To do so, we looked for decisions with high variance between analysis teams (e.g., choosing specific covariates).
% \mgm{What does this mean -- us analyzing for alternative approaches? Alternative to what?} 
From these decisions, we observed approaches (e.g., choosing player position as a covariate) that could help introduce other analysts to alternative approaches and mental models. These decisions informed categories of suggestions that aid in the various stages of the end-to-end analysis process.

These categories both corroborate and make more specific those outlined in the \litreview review. For instance, \textit{guidance for statistical modeling} from the \litreview review includes two aspects we uncovered in the crowd-sourced study: \textit{conceptual model formulation} and \textit{operationalizing constructs}. Likewise, \textit{alternative decisions} captures both \textit{high-level planning} (which helps analysts consider broader analysis decisions) and more specific planning decisions better summarized by the other categories. 
% We discuss different abstractions of planning assistance in Section~ \ref{sec:discussion_helpful}. 
From studying independent analyses of the crowd-sourced data, new categories, such as \textit{data wrangling} and \textit{model results interpretation}, also became apparent.

\wozFig

\subsection{Results}
 A summary of our suggestion categorizations is shown in Table \ref{tab:suggestions}, which includes examples we later developed for our \woz study (Sec.~\ref{sec:labstudy}). Full examples of suggestions in each category are also in the appendix. The \litreview review spanned domains and tasks, covering broad categories of assistance (e.g., \textit{guidance for statistical modeling}). 
% and guidelines (i.e., incorporate relevant domain and statistical knowledge) for crafting suggestions. 
Examination of the crowd-sourced study then helped facilitate more specific and new categories of help aimed at critical steps in the end-to-end analysis process (e.g., \textit{choosing the statistical model}). All categories except \textit{execution assistance} are \textit{intended} as planning assistance, helping the analyst reason about and consider alternative analysis decisions. Likewise, while the categories may not cover every possible helpful suggestion, based on our research, we expect high coverage. 

Overall, these categories encapsulate the collective approaches and rationale of expert-written analyses. Thus, they are likely to be helpful for analysts working on a variety of research problems. 
However, it is unclear to what degree suggestions from these categories would be helpful and what factors influence this judgment. To answer this, we conducted a \woz study.


==> 5-woz-new.tex <==

\section{\woz Study}
\label{sec:labstudy}
We conducted an exploratory lab study using a \woz protocol~\cite{Maulsby1993PrototypingAI, Dahlbck1993WizardOO} to understand the types of suggestions analysts prefer and how these suggestions might affect their workflow. 
In our study, participants interacted with a data analysis assistant housed in a customized JupyterLab interface which, unbeknownst to them, was controlled by a human ``wizard''. 
Our wizard (Fig. \ref{fig:woz}) simulated an LLM-based data analysis assistant. 
The wizard managed the LLM interaction manually, drawing from a predefined list of answers to make planning and execution suggestions while participants carried out a data analysis task.
% since analysts understandably may not have known how and when to best utilize LLMs. 
% We relaxed the constraint to have an automated process that creates prompts, consistently generates high-quality suggestions, and times the LLM's response. 
% \am{stuff}
% Through this process, we can obtain high-fidelity observations of how analysts work conduct an analysis with an assistant. Analysts are also better able to provide specific feedback about the assistant and its suggestions. Moreover, a \woz approach helps us reliably ensure high-quality suggestions and control the types of suggestions analysts encounter.



\xhdr{Participants}
% With our study, we wanted to understand analysts' preferences towards and the subsequent impact of planning assistance. We imagine novice analysts may be too bogged down by execution challenges that there never is any time or consideration for analysis planning (even if offered planning assistance). Moreover, if even trained analysts struggle with analysis planning \cite{Kale2019DecisionMakingUU, Liu2019PathsEP}, then understanding how to support these analysts is a crucial first step to supporting all analysts. Therefore, we focused on recruiting data analysts who are already familiar with statistical analysis. 
We recruited participants who were already familiar with statistical analysis and programming experience.
% and were likely to engage in analytical reasoning.
We contacted potential participants through analysis-related mailing lists at our institution.
From a pool of 60 volunteers, we invited those who rated their programming and statistics proficiency 4 out of 5 or greater and were familiar with computational notebooks, selecting a final 13 on a first come basis (Table \ref{tab:participants}).
% We imagine \tim{can we cite related work to inform this expectation and provide some justification?} novice analysts may be too bogged down by execution challenges that there never is any time or consideration for analysis planning (even if offered planning assistance). 
We chose not to consider novices, as they would be too limited by execution challenges \cite{Liu2020UnderstandingTR, Kandel2012EnterpriseDA} to be able to benefit from our analysis planning.
% in its current form. 
% Similarly, we thought that individuals lacking general statistical knowledge would struggle to comprehend the full range of recommended decisions \cite{Liu2019PathsEP}. 
Since even trained analysts face difficulties in analysis planning \cite{Kale2019DecisionMakingUU}, supporting those with expertise is a crucial step in supporting everyone.
Participants received a \$50 gift card as compensation. We denote participants by anonymous identifiers, like AX, and quote them, \shortquote{like so}. 

\tableParticipants


\xhdr{Procedure}
We conducted our study in a lab on a MacBook Pro on a 27-inch monitor. One author, in the lab with participants, served as the coordinator. Another author, the wizard, participated from a physically separate room over Zoom (which was also used to record the session with consent) under a pseudonym. Participants were unaware of the wizard and that the wizard was able to hear and see their screen.



The study lasted roughly 2 hours and consisted of three phases, consisting of a tutorial ($\sim$15 minutes), the primary task detailed below ($\sim$75 minutes), and a semi-structured interview ($\sim$30 minutes). 
In the last of these phases, the coordinator asked participants to review each suggestion they saw, give a positive, neutral, or negative reaction to whether the suggestion was helpful, and explain why (Fig.~\ref{fig:suggestion_reactions}). 
% \tim{do what degree did they do this live vs all retrospective during this interview?} 
We then asked about the impact the assistant's recommendations had on the participant's process, what participants valued from the assistant, and what sorts of actions or information they would have liked the assistant to provide. 
At the end of the study, we revealed how the assistant actually worked.
% , that is, its suggestions were a mix of manually written and ChatGPT-generated text, and its curation and raising of suggestions were done by a human wizard. 
Prior to the study, participants were asked about their preferred programming language and the analysis libraries. We created a notebook for each participant with their preferred language and tools. We wanted to ensure that the lab environment was as familiar as possible.
The study coordinator took notes throughout the analysis phase and the semi-structured interview. One author viewed the recordings, transcribed relevant episodes, and logged whether suggestions were included in participants' working analyses. To define common themes that emerged, two of the authors conducted iterative open coding on the recordings. 



\xhdr{Task} The bulk of the study consisted of a data analysis  task---namely the task conducted in the crowd-sourced study\footnote{In the interest of time, we made some minor adjustments to the dataset.
We sampled a subset of the data to simplify computational manipulation while maintaining the overall distribution of the dependent variable (red cards) across levels of the main independent variable (skin tone).
Additionally, we focused on the ten most frequently used variables across analyst teams in the original crowd-sourced study.} considered in Sec. \ref{sec:suggestions}---in the context of a JupyterLab notebook customized to have a planning equipped assistant (Fig. \ref{fig:interface}).  
Participants were asked to imagine they were leading a research team that had collected the dataset, following a similar methodology from Jun et al.~\cite{Jun2021HypothesisFE}.
% \tim{I'm confused -- I thought someone other than Eunice collected the red cards data?!} 
To prime participants,
% to consider how their decisions could affect results, 
we told them that their analysis results would impact a major policy decision---namely whether the soccer league invests money in bias training.
We stressed the importance of having reasonable rationales for their analysis decisions and that their decisions must be robust against alternative assumptions.
Likewise, to encourage comfort with the lab environment, we mentioned that we were not interested in the completion of the analysis but in their analysis process. 



Once participants were familiar with the task, the coordinator toggled on the assistant and introduced how its suggestions were raised. We described what the system can do (e.g., make suggestions based on the notebook context), being careful not to anthropomorphize the assistant to facilitate accurate evaluations~\cite{Khadpe2020ConceptualMI}. 
% \tim{curious. why is the latter important?}
We encouraged participants to think aloud or document their process in a notebook. They were free to use any external resources. 
% We wanted to give them adequate time to work through major phases of the analysis process (i.e., exploring the data, identifying relevant variables, running a model, and interpreting the results). 

 


% A wizard can abstract some of these issues and let us focus first on factors that contribute to helpful and successful planning assistance. 
% We also avoid pitfalls with LLMs that occur when non-AI experts struggle to produce effective prompts~\cite{ZamfirescuPereira2023WhyJC,  Mishra2022HELPMT}.



% Additionally,  using a \woz study lets us minimize the time spent on implementing a fully automated system~\cite{Dow2005WizardOO, Martin2012UniversalMO, Browne2019WizardOO}:  
% % \tim{~ backslash cite is a good default avoid weird linebreaks.} 
% our goal is not to evaluate the quality of a fully formed analysis assistant, but to study how to design such assistants from the ground up, assuming that generative approaches will eventually be able to provide suggestions of higher quality. Rather than automating the interface between the analyst and the LLM, the wizard, an experienced user of LLMs, can assume this responsibility. The wizard chooses relevant suggestions, selects the appropriate context, crafts the prompt, ensures the LLM generation is applicable and coherent, and determines suggestion timing (Fig. \ref{fig:woz} right).
 
% In our study, the wizard acts as the critical interface between the analyst and the LLM. 
% Building on prior work~\cite{Browne2019WizardOO, Amershi2019GuidelinesFH, McNutt2023OnTD, Horvitz1999PrinciplesOM, Dahlbck1993WizardOO, Fraser1991SimulatingSS, Riek2012WizardOO}, we developed our user interface, interactions, and the wizard protocol for creating and raising suggestions. 
% Informed by prior work on design principles for Human-AI interaction, we designed the study so that future LLM-powered systems would likely be able to  simulate the wizard's actions with the appropriate data and prompts.
% \tim{how certain are we of this? or should we say: likely would be able to...} 

% \tim{just highlighting broken ref}

% \ken{maybe we are overloading the word interface with user interface} \tim{seems fine to me personally} 
% The wizard identifies triggers when the analyst needs help and develops suggestions. These suggestions are curated from analyses written by trained analysts and further refined by prompting an LLM. 

% Likewise, while a wizard creating and delivering the suggestions raises a potential downside of being slower to respond than an automated system, we choose to conduct our study with a single analysis task and dataset to allow us to prepare high-quality suggestions in advance. In particular, we reuse the same task and dataset as that of the crowd-sourced analysis study we had previously studied (Sec. \ref{subsec:crowdsourced_study}). This enables us to both ensure high quality and rich diversity of suggestion content and timing, while only being slightly slower than a fully automated approach. 


% \tim{I think with planning assistance a bit higher latency is  probably more fine than for execution assistance? is there any way to back that up. Because execution is linear and you'd be waiting and wasting time potentially it's worse. but if you backtrack or suggest alternative plans, this necessarily requires a shift in focus and that can happen in parallel without taking time away with slow latencies. what do you think? I think we should add here? May also fit discussion perhaps?}\ken{Yes, more fitting for discussion imo}

% The goal of this approach is to convincingly simulate an automated data analysis assistant. We design our analysis assistant to seamlessly integrate into computational notebooks, a popular tool for data analysis \cite{Rule2018ExplorationAE}. 
% Building on prior work \cite{Browne2019WizardOO, Amershi2019GuidelinesFH, McNutt2023OnTD, Horvitz1999PrinciplesOM, Dahlbck1993WizardOO, Fraser1991SimulatingSS, Riek2012WizardOO} we develop our user interface, interactions, and the wizard protocol for creating and raising suggestions. Informed by prior work on design principles for Human-AI interaction, we design the study such that future LLM-powered systems would likely be able to  
% % \tim{how certain are we of this? or should we say: likely would be able to...} 
% simulate the wizard's actions with the appropriate data and prompts.


\interfaceFig

\xhdr{Assistant Design}
The design of our assistant closely followed recent explorations for assistants in notebooks~\cite{McNutt2023OnTD} and is shown in Fig. \ref{fig:interface}. We focused on notebooks because they are an extremely common medium for data analysis~\cite{Shen2014InteractiveNS, Rule2018ExplorationAE}.
% \subsection{User Interface}
% \am{intrp?????}
% We chose to integrate our assistant in computational notebooks\footnote{We include details of the interface implementation in the appendix}, a popular medium for data analysis~\cite{Shen2014InteractiveNS, Rule2018ExplorationAE}. The design of assistant UI drew on McNutt et al.'s~\cite{McNutt2023OnTD} design space of code assistants in computational notebooks.
% through surveying existing notebook systems and performing an interview study. 
% \tim{this sounds like what you want  to do in this paper? can you add a couple of words to clearly differentiate their contributions from yours?}\ken{did this in related work, still necessary here?} 
% A central design decision was the location of the assistant within the notebook UI. We opted for a side panel interface, which offers a global perspective of access to information for the assistant. This global scope is helpful because it implies that the suggestions integrate information from all parts of an analyst’s notebook. Additionally, by keeping the suggestions separate from the analyst's working notebook, we minimize any interference with an analyst's code, notes, and overall process.  
We place our assistant within a side panel which affords an apparently global perspective across the notebook. This scope helpfully implies that the suggestions integrate information from across the notebook. By keeping the suggestions separate from the participant's working notebook, we minimize any interference with their code, notes, and overall process.  
% 
As in other triggerless systems~\cite{jayagopal2022exploring}, participants received suggestions from the system without needing to take specific action. Given this design, there is no direct UI element for controlling the generated topics or to refine suggestions (similarly to Copilot's tab view). Also like Copilot, participants could influence the assistant by writing specific comments in their notebook. 
% While we did not not explicitly describe this interaction to participants, this behavior naturally emerged across multiple participants.
This comment writing behavior was not described in our introduction but emerged naturally across multiple participants. 
As suggestions from the wizard began to reference participant comments as the relevant notebook context, some participants took notice and wrote additional comments, expecting assistant help. 
% After early feedback, we included a copy button for suggested code blocks to help participants quickly incorporate recommended code (Fig. \ref{fig:interface}G). 

% In our side panel, suggestions appear as individual cards (Fig. \ref{fig:interface} right). Each suggestion card includes the relevant context \cite{Amershi2019GuidelinesFH} at a cell or line granularity (Fig. \ref{fig:interface}D1). 
% \tim{our goal is to empower... (and add why we think that is the right thing to do. it has to be more than an "empty belief"} 
% As AI suggestions can be imperfect and users of AI systems can overrely on the AI's suggestions and suffer from complacency bias \ken{TODO: citations}, our goal is to empower the analyst to exercise their own judgment in deciding whether to use the suggestions we provide.

% \tim{for all figures, neatly integrate them into the text via reference}


% Furthermore, since the study focuses on observing which suggestions analysts prefer and their effect on analysts, we implement additional features to encourage analysts to observe new suggestions. When a new suggestion occurs, the side panel shows a loading animation of variable duration to call attention to it; variability in duration aims to indicate that the system is working and simulate a real system computing and generating a suggestion~\cite{Fraser1991SimulatingSS, Riek2012WizardOO}. Moreover, to make new suggestions easily distinguishable from old ones, we highlight the borders of each new suggestion in yellow (Fig. \ref{fig:interface}D). Once analysts click on it, this highlight disappears. 


% \subsection{User Interactions}
% \label{sec:woz_user_interaction}
% We design the assistant to enable user interactions for planning assistance. 
% Execution assistance is widely studied and generally well-supported by current systems (Sec. \ref{sec:llm_background}). On the other hand, it is less clear how to design for planning assistance and how these suggestions may affect analysts.
% \tim{I know I've used the same language but we need to find a way to say this more precisely. For example, what are the  open questions? why do we not know how to do it? We need to be super super clear about this and we need to consistenntly describe this from abstract, intro etc...} 
% We aim to help analysts gain insights into analysis decisions, rationales, and statistical thinking that they may not be aware of. Consequently, we choose a design that focuses less on analyst initiative and more on system initiative. 

% Our \woz study was ideal since it let us adapt to these preferences. We discuss this topic further in Sec. \ref{sec:results_how}.
 % \tim{did they know that? were they instructed to do so?}

% To make the simulation more convincing, give the analyst a sense of agency, and support efficient invocation or dismissal \cite{Amershi2019GuidelinesFH}, we included an on/off toggle for the assistant (Fig. \ref{fig:interface}B). To encourage comfort and familiarize participants with the assistant \cite{Kahn2008DesignPF}, we displayed a startup message in which the assistant introduces itself when the analyst first toggles it on (Fig. \ref{fig:interface}C). Likewise, to encourage granular user feedback \cite{Amershi2019GuidelinesFH}, we provided thumbs up and thumbs down buttons for each suggestion (Fig. \ref{fig:interface}F).
% To support easy navigation in a commonly messy notebook~\cite{Head2019ManagingMI, Kery2018TheSI, Rule2018ExplorationAE}
% Clicking on a suggestion automatically scrolled the notebook to the corresponding context for that suggestion (Fig. \ref{fig:interface}D1-D2). 

% \tim{great job with all this!}


% \subsection{\woz Protocol}

% With these considerations, it is important to develop realistic suggestions that are helpful and reasonable from an LLM. 

% \tim{One potential misunderstanding is that you simulate the entire LLM away. But actually you still use an LLM, you just relax the constraint to have an automated process that consistently creates the best prompts and consistently generates high quality feedback by allowing yourself to manually manage this process and LLM interaction (whereas analysts understandably may not know how and when to best utilize LLMs.)} 

\xhdr{Raising and Creating Suggestions} 
When and what suggestions the wizard raised were guided by several principles. 
The wizard raised suggestions when they were relevant to the notebook, with priority given to the most recent additions \cite{Amershi2019GuidelinesFH}. When possible, the wizard offered planning suggestions,
% , which are less well understood and supported by current systems (Sec. \ref{sec:llm_background}). 
% To maintain trust and show contextually relevant information \cite{Amershi2019GuidelinesFH, Horvitz1999PrinciplesOM}, 
but execution assistance was provided when it was deemed required. 
Examples include when participants were stuck debugging outputs or wrote notebook comments asking for specific help (Sec. \ref{sec:results_how}).
% \tim{were they instructed that they could do that? did it happen naturally? how many people did that?}
The wizard attempted to strike a balance between a rich diversity of suggestions and not overwhelming the participant with excessive feedback. 
Finally, we simulated an assistant that could learn over time what suggestions the analyst found helpful--following common Human-AI guidelines~\cite{Amershi2019GuidelinesFH}. To wit, the categories of suggestions we raised depended on whether the suggestions already given were considered or taken. If the participant disregarded many suggestions that addressed alternative variables, we raised these suggestions less often.

% \xhdr{Creating Suggestions} 
% \label{subsec:building_suggestions}
 % \tim{this subsubsection doesn't seem to be about creating suggestions but seems to be about potential limiations of the approach?} \tim{"limit the domain of possible suggestions" itself sounds like a HUGE downside and threat to validity. It's also confusing after your previous section 3 where you tried to give a comprehensive set of possible suggestions.} 


  
 % As mentioned at the beginning of this section (Sec. \ref{sec:woz_design}), we plan for analysts interacting with our system to work with the same dataset and research question. This choice enables us to prepare common suggestions prior to the study that might be relevant. To prepare high-quality suggestions, we intentionally chose the same task and dataset as that of the crowd-sourced analysis study that first informed our categories of assistance (Sec. \ref{subsec:crowdsourced_study}).  \tim{para could be tightened}
 
 % Since we already created high-quality and often reusable suggestions through our analysis of a crowd-sourced analysis study (Sec. \ref{sec:suggestions}), we choose the same task and dataset from the crowd-sourced study for our \woz study. \tim{no :) rephrase last sentence. You did not happen to already have created these. You intentionally choose the same task and dataset because that enables you to create high-quality suggestions in preparation. Examples were described in Section XX.}\ken{Not sure exactly what the flow is we want to convey now. Is the categorization section (Sec. \ref{sec:suggestions}) only about finding out categories of suggestions and not creating them? Is the work of creating all in this section now? I can also see what I wrote below as making this more confusing}
Creating suggestions followed the analysis conducted in the previous section (Sec.~\ref{sec:suggestions}).
For categories such as \textit{domain background} and \textit{operationalizing constructs} (Table \ref{tab:suggestions}), the same or very similar suggestions could be given to different participants. To speed up the assistant's response time, we prepared a spreadsheet of suggestions (based on Table~\ref{tab:suggestions}) in these categories before the study for the wizard to draw from (Fig. \ref{fig:woz}B). 
% The spreadsheet had the categories in Table \ref{tab:suggestions}, except each category could have multiple prepared suggestions. 
We created 32 suggestions across these categories. We deliberately crafted all suggestions with pertinent explanations and relevant domain and statistical knowledge. For most suggestions, we also included example execution assistance code to help participants grasp and implement the given recommendation. Though these planning suggestions featured execution assistance elements, their primary intent was to aid in analysis planning.

For categories \textit{execution assistance} or \textit{model results interpretation} (Table \ref{tab:suggestions}), suggestions were closely tied to the context of the working analysis which precluded previously created suggestions.
% Therefore, suggestions created previously could not be used. 
For these categories, we leveraged ChatGPT \cite{ChatGPT} and constructed prompts to build suggestions. Prior to the study, we created a general prompt introducing the task and dataset.
% and specific prompts for different categories. 
% During the study, ChatGPT was tightly integrated into the suggestion creation process. 
% \tim{we should be consistent. are we building/developing/creating suggestions? I don't have a strong opinion but like creating.} 
In addition to this general prompt, the wizard, who prepared the spreadsheet of suggestions and is experienced in using LLMs, crafted prompts in real-time using the notebook context (Fig. \ref{fig:woz}A) or parts of pre-written suggestions (Fig. \ref{fig:woz}B). The wizard then passed the prompt to ChatGPT to generate the suggestion of interest (Fig. \ref{fig:woz}C). 
% Given their experience and preparation, 
% the wizard primarily wrote prompts in real-time. 
% \tim{didd you do these from scratch every time? it reads that way.}\ken{basically yes because it was so varied with approaches and prompts were not super difficult to write in the momment} \tim{okay. then say that the wizard did write these prompts largely in real-time, but their experience allowed them to do this relatively quickly} 
% Further, the wizard used 
ChatGPT was further used to refine some generated code---for example, to convert code between programming languages or shorten the length of a prior generation (Fig. \ref{fig:woz}C-D loop). 
The wizard sometimes manually corrected the output of a ChatGPT generation (e.g., changed the wording or variable names) to ensure high-quality suggestions. 
% since raw ChatGPT generations might not perfectly fit analysts' current code, whether due to the limited capabilities of ChatGPT or insufficient context being provided as part of the prompt. 
% \tim{is this for correction / and to ensure high quality? (whereas even SOTA LLMs demonstrate these various mistakes?) }\ken{i don't think ChatGPT was necessary incorrect, its just that it was given more general prompts that didn't include all the code from the analyst. This would have been hard to do as the wizard in the momment. How can we write this?} \tim{took a stab at integrating above} 
% Overall, this protocol proved effective in helping us learn about specific types of suggestions while incorporating the capabilities of current LLMs.
% \tim{again integrate the figure and also refer to ABCD... like in the caption}



% \tim{how much of a limitation is it that analysts didn't have another way of interacting with the assistant? if our focus was execution assistance that seems to be bigger problem than with planning assistance.}

% \subsection{Implementation}
% We implemented the wizard and user interface for the Jupyter environment \cite{Prez2007IPythonAS} as a JupyterLab extension. We extended the JupyterLab Commenting and Annotation extension \cite{jupyterlabcomments} and incorporated two modes: wizard mode and analyst mode. Both modes work with the same underlying notebook file and share a similar side panel interface. In \textit{wizard mode}, the wizard can highlight code or cells and add corresponding suggestions to the side panel. All suggestions were stored on disk as an underlying suggestion file. The extension, when in \textit{analyst mode}, polled this file for changes and updated the side panel when new suggestions were added to the file. 

% In the study, both the analyst and wizard worked with the same notebook in the same file system.  We hosted the notebook on the wizard's machine. Accordingly, we connected the analyst’s machine remotely to the wizard’s machine using SSH. To ensure the wizard did not update actual notebook contents, we gave wizard mode no edit permissions.  





% \tim{why?}\ken{Not sure if I defended the choice of analysts enough} 

% We advertised an opportunity to work with a data analysis assistant tool.
% In the initial interest form, we asked analysts to self-rate their statistical background on a 5-point scale (higher being more familiar). In this scale, 4 described analysts who have taken graduate-level courses related to statistical analysis, and 5 described analysts having multiple years of experience with real-world projects involving statistical and data analysis. \tim{will readers ask about 1-3?} We also asked analysts to rate their familiarity with R or Python on a 5-point scale with 1 “being equivalent to having taken an introductory course” and 5 being having “5+ years of industry experience”. 
% 60 analysts volunteered, which we filtered down to 13. 

% (4s and 5s on a 5-point scale), background diversity, and familiarity with writing analyses in computational notebooks.
% We aimed for analysts from diverse domain backgrounds, who were quite familiar with R or Python, and have non-trivial experience in statistical analysis. 
% We wanted to observe analysts who are unlikely to be bogged down by execution challenges but likely to engage in analytical reasoning.
% Moreover, we made sure to select analysts who have not seen the dataset or study before. \tim{did that actually occur?}
% We also selected analysts who were familiar with writing analyses in computational notebooks.


% for their time. 

% \xhdr{Data}
% % Analysts in our study worked through the same task as the teams in the crowd-sourced data analysis study~\cite{Silberzahn2018ManyAO}. To ease dataset understanding, help analysts focus on planning, and help us study a variety of suggestions over the course of one lab session, 
% We made minor adjustment to the dataset to simplify the task.
% We sampled a subset of the data to improve simplify the task and improve computational efficiency while maintaining the overall distribution of the dependent variable (red cards) across levels of the main independent variable (skin tone).
% Additionally, we focused on the ten most frequently used variables across analyst teams in the original crowd-sourced study. 
% Due to our study's time constraints, \tim{we can say that "nicer". it's not a constraint/downside. Instead, you made minor adaptations to make XYZ easier, help analysts focus on XYZ, to enable us to study a variety of suggestions over the course of an X-hour study.... This is a general pattern in my feedback. Always say why you made a choice and why this was a good reason/process to do so. Be careful with things that sound like downsides and explain them and what you did about them.} we made minor adaptations to the dataset. 
% We wanted to allow analysts to identify important analytical decisions while still preserving realistic variation in the data; therefore, 

% Additionally, we focused on the most relevant independent variables based on the analyses from the original crowd-sourced study. Specifically, we included the ten most frequently used variables across all analyst teams. 

% Specifically, we included the ten most frequently used variables across all analyst teams. 


% For consistency across sessions, another author, who developed the JupyterLab extension and prepared the suggestions, acted as the wizard. 
% This ensured that the behavior of the assistant remained consistent across analysts. 

% Before the study, we obtained analysts’ consent to record their screens and audio. 
%  they often worked with and might expect to work with for the study


% We recorded the study using a Zoom meeting. The wizard attended the virtual meeting under the pseudonym of the coordinator and was physically in a separate room. Analysts were unaware of the wizard and that the wizard was able to hear and see their screen.



% In the first phase of about 15 minutes, the coordinator introduced the task and guided analysts through the JupyterLab notebook. 
% We discuss the notebook in detail in Appendix~\ref{appendix:notebook_detail}.

% \xhdr{Task}
% Following by Jun et al. \cite{Jun2021HypothesisFE}, which aimed to understand analysts' statistical thinking and sensemaking processes, 


% Most analysts did not finish their analysis  \tim{that sounds like a contrast to the prev sentence. is this a concern? does it add limitations?}\ken{yes can discuss in limitations that they didn't come to the end with a full and confident analysis conclusion.} 




% This study was determined exempt by the IRB at our institution. 

% \xhdr{Data Analysis}
% In addition to the recordings of participants’ audio and screens, 

% The authors met over multiple sessions to refine codes on any observations related to the helpfulness of suggestions and the overall interaction between the analyst and assistant. 
% They also met to code all suggestions that were raised into the suggestion categories summarized in Table \ref{tab:suggestions}.

% \tim{should we say anything here about agreement between the two, how disagreement was resolved?}

% . \tim{great, make these specific section references}\ken{I think supplemental material is different then appendix}

% We also tracked all suggestions that were raised and documented analysts' ratings of their helpfulness (i.e., positive, neutral, negative). \ken{TODO add sentence or two based on results}

\reactionsFig

\xhdr{Limitations} While able to elicit a variety of realistic user reactions to a new form of assistant this design has some limitations.
While a complete implementation of full system would be useful, our goals in this work are to better understand the design of such assistants rather than their implementation. 
Similarly, through this approach we are not limited by the capabilities of current LLMs (Sec. \ref{sec:llm_background}) or participants non-expert prompt engineering abilities~\cite{ZamfirescuPereira2023WhyJC,  Mishra2022HELPMT}.
% \am{sentence}
Having a wizard create and deliver suggestions also raises a potential downside of being slower to respond than an automated system. However, we chose to conduct our study with a single analysis task and dataset so we could prepare high-quality suggestions in advance. 
% In particular, we used the same task and dataset as the one from the crowd-sourced analysis study we examined~(Sec. \ref{subsec:crowdsourced_study}). 
This helped us both ensure a high quality and rich diversity of suggestion content and timing while being only slightly slower than a fully automated approach. 

==> 5-woz.tex <==
% \section{Motivating a \woz Study}
% \label{sec:woz_motivation}

% % With the categorization of suggestions encompassing assistance opportunities throughout the end-to-end analysis process (Sec. \ref{sec:suggestions}), we want to observe analysts' reactions to different categories of suggestions and their impact on the analyst's analysis process. A \woz study \cite{Kelley1983AnEM} is ideal for helping us efficiently and effectively answer our research questions. 

% In a \woz study, analysts interact with an assistant interface which, unbeknownst to them, is controlled by a human ``wizard'' \cite{Maulsby1993PrototypingAI, Dahlbck1993WizardOO}. Through this process, we can obtain high-fidelity observations of analysts working through an analysis with an assistant. Analysts are also better able to provide specific feedback about the assistant and its suggestions. Moreover, a \woz approach enables us to reliably ensure high-quality suggestions and control the types of suggestions analysts face.

% Importantly, by using this approach, we are not limited by the capabilities of current LLMs (Sec. \ref{sec:llm_background}).
% A wizard can abstract some of these issues and allow us to focus first on what contributes to favorable planning assistance. 
% We also avoid pitfalls with LLMs when non-AI experts struggle to produce effective prompts \cite{ZamfirescuPereira2023WhyJC,  Mishra2022HELPMT} (see also Sec. \ref{sec:llm_background}).

% Likewise,  through a \woz study, we minimize the time spent on implementing a fully automated system \cite{Dow2005WizardOO, Martin2012UniversalMO, Browne2019WizardOO}.  We are not evaluating the quality of an analysis assistant that is likely to be imperfect. Instead, we focus on studying how these assistants should be designed in the first place, assuming that generative approaches will eventually be able to provide suggestions of sufficient quality. Rather than automating the interface between the analyst and the LLM, the wizard, who is experienced with using LLMs, can take on this responsibility. The wizard chooses what suggestion is relevant, selects the right context, crafts the prompt, ensures the LLM generation is applicable and coherent, and determines the timing of the suggestion (Fig. \ref{fig:woz} right).





\wozFig
\section{Designing a \woz Study}
\label{sec:woz_design}

\am{missing intro} In a \woz study, analysts interact with an interface which, unbeknownst to them, is controlled by a human ``wizard'' \cite{Maulsby1993PrototypingAI, Dahlbck1993WizardOO}. Through this process, we can obtain high-fidelity observations of how analysts work conduct an analysis with an assistant. Analysts are also better able to provide specific feedback about the assistant and its suggestions. Moreover, a \woz approach helps us reliably ensure high-quality suggestions and control the types of suggestions analysts encounter.

Importantly, by using this approach, we are not limited by the capabilities of current LLMs (Sec. \ref{sec:llm_background}).
A wizard can abstract some of these issues and let us focus first on factors that contribute to helpful and successful planning assistance. 
We also avoid pitfalls with LLMs that occur when non-AI experts struggle to produce effective prompts~\cite{ZamfirescuPereira2023WhyJC,  Mishra2022HELPMT}.

Additionally,  using a \woz study lets us minimize the time spent on implementing a fully automated system~\cite{Dow2005WizardOO, Martin2012UniversalMO, Browne2019WizardOO}:  
% \tim{~ backslash cite is a good default avoid weird linebreaks.} 
our goal is not to evaluate the quality of a fully formed analysis assistant, but to study how to design such assistants from the ground up, assuming that generative approaches will eventually be able to provide suggestions of higher quality. Rather than automating the interface between the analyst and the LLM, the wizard, an experienced user of LLMs, can assume this responsibility. The wizard chooses relevant suggestions, selects the appropriate context, crafts the prompt, ensures the LLM generation is applicable and coherent, and determines suggestion timing (Fig. \ref{fig:woz} right).
 
In our study, the wizard acts as the critical interface between the analyst and the LLM. Building on prior work~\cite{Browne2019WizardOO, Amershi2019GuidelinesFH, McNutt2023OnTD, Horvitz1999PrinciplesOM, Dahlbck1993WizardOO, Fraser1991SimulatingSS, Riek2012WizardOO}, we developed our user interface, interactions, and the wizard protocol for creating and raising suggestions. Informed by prior work on design principles for Human-AI interaction, we designed the study so that future LLM-powered systems would likely be able to  
% \tim{how certain are we of this? or should we say: likely would be able to...} 
simulate the wizard's actions with the appropriate data and prompts.


% \tim{just highlighting broken ref}

% \ken{maybe we are overloading the word interface with user interface} \tim{seems fine to me personally} 
% The wizard identifies triggers when the analyst needs help and develops suggestions. These suggestions are curated from analyses written by trained analysts and further refined by prompting an LLM. 

% Likewise, while a wizard creating and delivering the suggestions raises a potential downside of being slower to respond than an automated system, we choose to conduct our study with a single analysis task and dataset to allow us to prepare high-quality suggestions in advance. In particular, we reuse the same task and dataset as that of the crowd-sourced analysis study we had previously studied (Sec. \ref{subsec:crowdsourced_study}). This enables us to both ensure high quality and rich diversity of suggestion content and timing, while only being slightly slower than a fully automated approach. 


% \tim{I think with planning assistance a bit higher latency is  probably more fine than for execution assistance? is there any way to back that up. Because execution is linear and you'd be waiting and wasting time potentially it's worse. but if you backtrack or suggest alternative plans, this necessarily requires a shift in focus and that can happen in parallel without taking time away with slow latencies. what do you think? I think we should add here? May also fit discussion perhaps?}\ken{Yes, more fitting for discussion imo}

% The goal of this approach is to convincingly simulate an automated data analysis assistant. We design our analysis assistant to seamlessly integrate into computational notebooks, a popular tool for data analysis \cite{Rule2018ExplorationAE}. 
% Building on prior work \cite{Browne2019WizardOO, Amershi2019GuidelinesFH, McNutt2023OnTD, Horvitz1999PrinciplesOM, Dahlbck1993WizardOO, Fraser1991SimulatingSS, Riek2012WizardOO} we develop our user interface, interactions, and the wizard protocol for creating and raising suggestions. Informed by prior work on design principles for Human-AI interaction, we design the study such that future LLM-powered systems would likely be able to  
% % \tim{how certain are we of this? or should we say: likely would be able to...} 
% simulate the wizard's actions with the appropriate data and prompts.

\interfaceFig

\subsection{User Interface}
We chose to integrate our assistant in computational notebooks\footnote{We include details of the interface implementation in the appendix}, a popular medium for data analysis~\cite{Shen2014InteractiveNS, Rule2018ExplorationAE}. When designing the assistant user interface, we built on relevant findings from McNutt et al.~\cite{McNutt2023OnTD}, which outlined the design space of code assistants in computational notebooks through surveying existing notebook systems and performing an interview study. 
% \tim{this sounds like what you want  to do in this paper? can you add a couple of words to clearly differentiate their contributions from yours?}\ken{did this in related work, still necessary here?} 
A central design decision was the location of the assistant within the notebook UI. We opted for a side panel interface, which offers a global perspective of access to information for the assistant. This global scope is helpful because it implies that the suggestions integrate information from all parts of an analyst’s notebook. Additionally, by keeping the suggestions separate from the analyst's working notebook, we minimize any interference with an analyst's code, notes, and overall process.  
% \tim{our goal is to empower... (and add why we think that is the right thing to do. it has to be more than an "empty belief"} 
% As AI suggestions can be imperfect and users of AI systems can overrely on the AI's suggestions and suffer from complacency bias \ken{TODO: citations}, our goal is to empower the analyst to exercise their own judgment in deciding whether to use the suggestions we provide.

% \tim{for all figures, neatly integrate them into the text via reference}

In our side panel, suggestions appear as individual cards (Fig. \ref{fig:interface} right). Each suggestion card includes the relevant context \cite{Amershi2019GuidelinesFH} at a cell or line granularity (Fig. \ref{fig:interface}D1). Furthermore, since the study focuses on observing which suggestions analysts prefer and their effect on analysts, we implement additional features to encourage analysts to observe new suggestions. When a new suggestion occurs, the side panel shows a loading animation of variable duration to call attention to it; variability in duration aims to indicate that the system is working and simulate a real system computing and generating a suggestion~\cite{Fraser1991SimulatingSS, Riek2012WizardOO}. Moreover, to make new suggestions easily distinguishable from old ones, we highlight the borders of each new suggestion in yellow (Fig. \ref{fig:interface}D). Once analysts click on it, this highlight disappears. 


\subsection{User Interactions}
\label{sec:woz_user_interaction}
We design the assistant to enable user interactions for planning assistance. 
% Execution assistance is widely studied and generally well-supported by current systems (Sec. \ref{sec:llm_background}). On the other hand, it is less clear how to design for planning assistance and how these suggestions may affect analysts.
% \tim{I know I've used the same language but we need to find a way to say this more precisely. For example, what are the  open questions? why do we not know how to do it? We need to be super super clear about this and we need to consistenntly describe this from abstract, intro etc...} 
We aim to help analysts gain insights into analysis decisions, rationales, and statistical thinking that they may not be aware of. Consequently, we choose a design that focuses less on analyst initiative and more on system initiative. Analysts receive suggestions from the system but do not need to take specific action. There is no explicit UI design that lets the analyst control the topics that are generated or refine the suggestions. However, analysts can influence the assistant by writing specific comments in their notebook. 
% While we did not not explicitly describe this interaction to participants, this behavior naturally emerged across multiple participants.
This comment writing behavior was not described a priori in our introduction of the assistant but naturally emerged across multiple participants. 
As suggestions from the wizard began to reference analyst comments as the relevant notebook context, some analysts took notice and began to write additional comments, expecting assistant help. Our \woz study was ideal since it let us adapt to these preferences. We discuss this topic further in Sec. \ref{sec:results_how}.
 % \tim{did they know that? were they instructed to do so?}

To make the simulation more convincing, give the analyst a sense of agency, and support efficient invocation or dismissal \cite{Amershi2019GuidelinesFH}, we included an on/off toggle for the assistant (Fig. \ref{fig:interface}B). To encourage comfort and familiarize participants with the assistant \cite{Kahn2008DesignPF}, we displayed a startup message in which the assistant introduces itself when the analyst first toggles it on (Fig. \ref{fig:interface}C). Likewise, to encourage granular user feedback \cite{Amershi2019GuidelinesFH}, we provided thumbs up and thumbs down buttons for each suggestion (Fig. \ref{fig:interface}F). To support easy navigation in a commonly messy notebook~\cite{Head2019ManagingMI, Kery2018TheSI, Rule2018ExplorationAE}, clicking on a suggestion automatically scrolled the notebook to the corresponding context for that suggestion (Fig. \ref{fig:interface}D1-D2). Finally, after early feedback from analysts, we included a copy button for suggested code blocks to help analysts quickly incorporate recommended code (Fig. \ref{fig:interface}G). 
% \tim{great job with all this!}


\subsection{\woz Protocol}
Our \woz protocol (Fig. \ref{fig:woz}) simulated an LLM-powered data analysis assistant. Behind the scenes, the wizard manually managed LLM interaction since analysts understandably may not have known how and when to best utilize LLMs. We relaxed the constraint to have an automated process that creates prompts, consistently generates high-quality suggestions, and times the LLM's response. 
% With these considerations, it is important to develop realistic suggestions that are helpful and reasonable from an LLM. 

% \tim{One potential misunderstanding is that you simulate the entire LLM away. But actually you still use an LLM, you just relax the constraint to have an automated process that consistently creates the best prompts and consistently generates high quality feedback by allowing yourself to manually manage this process and LLM interaction (whereas analysts understandably may not know how and when to best utilize LLMs.)} 

\subsubsection{Creating Suggestions} 
\label{subsec:building_suggestions}
 % \tim{this subsubsection doesn't seem to be about creating suggestions but seems to be about potential limiations of the approach?} \tim{"limit the domain of possible suggestions" itself sounds like a HUGE downside and threat to validity. It's also confusing after your previous section 3 where you tried to give a comprehensive set of possible suggestions.} 

Having a wizard create and deliver suggestions raises a potential downside of being slower to respond than an automated system. However, we chose to conduct our study with a single analysis task and dataset so we could prepare high-quality suggestions in advance. In particular, we used the same task and dataset as the one from the crowd-sourced analysis study we examined~(Sec. \ref{subsec:crowdsourced_study}). This helped us both ensure high quality and rich diversity of suggestion content and timing while being only slightly slower than a fully automated approach. 
  
 % As mentioned at the beginning of this section (Sec. \ref{sec:woz_design}), we plan for analysts interacting with our system to work with the same dataset and research question. This choice enables us to prepare common suggestions prior to the study that might be relevant. To prepare high-quality suggestions, we intentionally chose the same task and dataset as that of the crowd-sourced analysis study that first informed our categories of assistance (Sec. \ref{subsec:crowdsourced_study}).  \tim{para could be tightened}
 
 % Since we already created high-quality and often reusable suggestions through our analysis of a crowd-sourced analysis study (Sec. \ref{sec:suggestions}), we choose the same task and dataset from the crowd-sourced study for our \woz study. \tim{no :) rephrase last sentence. You did not happen to already have created these. You intentionally choose the same task and dataset because that enables you to create high-quality suggestions in preparation. Examples were described in Section XX.}\ken{Not sure exactly what the flow is we want to convey now. Is the categorization section (Sec. \ref{sec:suggestions}) only about finding out categories of suggestions and not creating them? Is the work of creating all in this section now? I can also see what I wrote below as making this more confusing}

For categories such as \textit{domain background} and \textit{operationalizing constructs} (Table \ref{tab:suggestions}), the same or very similar suggestions could be given to different analysts. To speed up the assistant's response time, we prepared a spreadsheet of suggestions in these categories before the study for the wizard to draw from (Fig. \ref{fig:woz}B). The spreadsheet had the categories in Table \ref{tab:suggestions}, except each category could have multiple prepared suggestions. 

In total, we created 32 suggestions across these categories. (See Appendix \ref{appendix:suggestion_examples} for complete examples of these suggestions.) We deliberately crafted all suggestions with pertinent explanations and relevant domain and statistical knowledge. For most suggestions, we also included example execution assistance code to help analysts grasp and implement the given recommendation. Though these planning suggestions featured execution assistance elements, their primary intent was to aid in analysis planning.

For categories \textit{execution assistance} or \textit{model results interpretation} (Table \ref{tab:suggestions}), suggestions were closely tied to the context of the working analysis. Therefore, suggestions created previously could not be used. For these categories, we leveraged ChatGPT \cite{ChatGPT} and constructed prompts to build suggestions. Prior to the study, we created a general prompt introducing the analysis task and dataset and specific prompts for different categories. 

During the study, ChatGPT was tightly integrated into the suggestion creation
% \tim{we should be consistent. are we building/developing/creating suggestions? I don't have a strong opinion but like creating.} 
process. Along with directly using the general prompt, the wizard crafted prompts using the notebook context (Fig. \ref{fig:woz}A) and/or parts of pre-written suggestions (Fig. \ref{fig:woz}B). The wizard then passed the prompt to ChatGPT to generate the suggestion of interest (Fig. \ref{fig:woz}C). Given their experience and preparation, the wizard primarily wrote prompts in real-time. 
% \tim{didd you do these from scratch every time? it reads that way.}\ken{basically yes because it was so varied with approaches and prompts were not super difficult to write in the momment} \tim{okay. then say that the wizard did write these prompts largely in real-time, but their experience allowed them to do this relatively quickly} 
Further, the wizard used ChatGPT to refine generations,  for example, to convert code between programming languages or shorten the length of a prior generation (Fig. \ref{fig:woz}C-D loop). Throughout this process, the wizard manually adapted and corrected the output of a ChatGPT generation to the current analysis (e.g., changed the wording or variable names in code). This was to ensure high quality since raw ChatGPT generations might not perfectly fit analysts' current code, whether due to the limited capabilities of ChatGPT or insufficient context being provided as part of the prompt. 
% \tim{is this for correction / and to ensure high quality? (whereas even SOTA LLMs demonstrate these various mistakes?) }\ken{i don't think ChatGPT was necessary incorrect, its just that it was given more general prompts that didn't include all the code from the analyst. This would have been hard to do as the wizard in the momment. How can we write this?} \tim{took a stab at integrating above} 
Overall, this protocol proved effective in helping us learn about specific types of suggestions while incorporating the capabilities of current LLMs.
% \tim{again integrate the figure and also refer to ABCD... like in the caption}

\subsubsection{Raising Suggestions} 
When and what suggestions the wizard raised were guided by several principles. First, the wizard raised suggestions when they were relevant to the text, with priority given to the most recent additions \cite{Amershi2019GuidelinesFH}. When possible, the wizard offered planning suggestions, which are less well understood and supported by current systems (Sec. \ref{sec:llm_background}). However, to maintain trust and show contextually relevant information \cite{Amershi2019GuidelinesFH, Horvitz1999PrinciplesOM}, the wizard also provided suggestions in situations when it was clear that the analyst needed execution assistance. Examples include when analysts were stuck on a coding task (e.g., debugging outputs) or when analysts, after learning the behavior of the system, naturally wrote notebook comments asking for specific help (Sec. \ref{sec:results_how}).
% \tim{were they instructed that they could do that? did it happen naturally? how many people did that?}
The wizard attempted to strike a balance between a rich diversity of suggestions and not overwhelming the analyst with obviously excessive feedback. 
Finally, we simulated an assistant that could learn over time what suggestions are helpful to the analyst \cite{Amershi2019GuidelinesFH}; the categories of suggestions we raised depended on whether the suggestions already given were considered/taken. For instance, if the analyst disregarded many suggestions that addressed alternative variables, we raised these suggestions less often.

% \tim{how much of a limitation is it that analysts didn't have another way of interacting with the assistant? if our focus was execution assistance that seems to be bigger problem than with planning assistance.}

% \subsection{Implementation}
% We implemented the wizard and user interface for the Jupyter environment \cite{Prez2007IPythonAS} as a JupyterLab extension. We extended the JupyterLab Commenting and Annotation extension \cite{jupyterlabcomments} and incorporated two modes: wizard mode and analyst mode. Both modes work with the same underlying notebook file and share a similar side panel interface. In \textit{wizard mode}, the wizard can highlight code or cells and add corresponding suggestions to the side panel. All suggestions were stored on disk as an underlying suggestion file. The extension, when in \textit{analyst mode}, polled this file for changes and updated the side panel when new suggestions were added to the file. 

% In the study, both the analyst and wizard worked with the same notebook in the same file system.  We hosted the notebook on the wizard's machine. Accordingly, we connected the analyst’s machine remotely to the wizard’s machine using SSH. To ensure the wizard did not update actual notebook contents, we gave wizard mode no edit permissions.  

% \tim{we can consider sharing this code? how valuable to others would it be?}

==> 5-woz_old.tex <==
\section{Motivating a \woz Study}

With the categorization and creation of suggestions informed by expert written analyses, we want to observe analysts' reactions to these suggestions and the impact on their analysis process. Accordingly, we design a \woz study \cite{Kelley1983AnEM}. 

\section{Designing a \woz Study}
\label{sec:woz_design}

% With a \tim{sounds defensive? is there a way to be specific about contribution/quality without that?} categorization of assistant suggestions, 

With the categorization and creation of suggestions informed by expert written analyses, we want to observe analysts' reactions to these suggestions and the impact on their analysis process. Accordingly, we design a \woz study \cite{Kelley1983AnEM}. 

\subsection{Motivation}
A \woz study is ideal for helping us efficiently and effectively answer our research questions. In a \woz study, analysts interact with an assistant interface which, unbeknownst to them, is controlled by a human “wizard” \cite{Maulsby1993PrototypingAI, Dahlbck1993WizardOO}. Through this process, we can obtain high-fidelity observations of analysts working through an analysis with an assistant. Moreover, a \woz approach enables us to reliably control the types of suggestions analysts face. 

In our study, the wizard acts as the critical interface between the analyst and the LLM. 
% \ken{maybe we are overloading the word interface with user interface} \tim{seems fine to me personally} 
The wizard identifies triggers when the analyst needs help and develops suggestions. These suggestions are curated from analyses written by trained analysts and further refined by prompting an LLM. 

Most importantly, by using this approach, we are not limited by the capabilities of current LLMs. 
% \tim{say this more clearly as an advantage and perhaps the most important consideration} 
LLMs, by design, cannot raise suggestions that deviate from the current analysis context (e.g., to highlight an important step the analysis may have missed). Thus, we are able to provide a richer diversity and higher quality of feedback to explore this design space. We also avoid pitfalls with LLMs when non-AI experts struggle to produce effective prompts \cite{ZamfirescuPereira2023WhyJC, Mishra2022HELPMT}. With LLMs alone, all the burden is placed on the analyst to know when to interact with the assistant, come up with, and refine the prompts. This can cause significant cognitive load \cite{Jiang2022PromptMakerPP}, suboptimal quality of feedback \cite{ZamfirescuPereira2023WhyJC}, and even missed opportunities for feedback.
% \tim{we can add here that expecting the analyst to know when to interact with the assistant and to come up with the prompts themselves puts all the burden on the analysts. This leads to worse experience, suboptimal quality of feedback, missed opportunities for feedback etc. Is there a good reference we could use here?} 
Furthermore, a \woz study enables us to consider the effects of disruptions and adapt suggestions quickly through the suggestion refinement process.
% \tim{I suggest to rework this paragraph in a subsection titled advantages of woz. You can then have a ``potential disadvantages of woz and mitigation strategies'' and describe those (might be slower, but you prepare a bunch ahead of time etc)}\ken{I'm not sure if we want a overtly negative subsection and this whole intro part seems like a motivation or benefits of woz. Maybe I can just have a motivation subsection?}


Therefore, through a \woz study, we minimize the time spent on implementing a fully functioning system \cite{Dow2005WizardOO, Martin2012UniversalMO, Browne2019WizardOO}. We do not need to collect training data and prompts, and develop algorithms for the timing of suggestion feedback for every assistance situation. Moreover, we are not evaluating the quality of an analysis assistant that is likely to be imperfect. Instead, we focus on studying how these assistants should be designed in the first place, assuming that generative approaches will eventually be able to provide suggestions of sufficient quality. We direct our efforts to exploring the design space of suggestions and the interface between the analyst and the LLM. 
% \tim{maybe we can say that even more clearly, also in intro etc. Instead of evaluating the quality of an analysis assistant that is likely to be imperfect, we focus on studying how these assistants should be designed in the first place.  (assuming that generative approaches will eventually be able to provide suggestions of sufficient quality.}

\tim{curious what others think but I find it imprecise and misleading to suggest that "just an LLM" can provide all this feedback. A language model wouldn't provide interfaces, interactions, processes, triggers, tools to aid implementation of feedback, considerations of disruptions etc. Clearly LLMs are critical and quite possibly all these can be solved by using LLMs in the right way.} \tim{still feel that way. can we refine this and discuss this early on, likely in intro, that assistants and helpful interactions are a lot more than a LLM alone.}
% Moreover, we do not need to  \tim{can we be more precise what it can and can't do and what is supported by the wizard.}, such as collecting training data, prompts, and evaluating the model .

At the core of this approach is to convincingly simulate a data analysis assistant. We design our analysis assistant to seamlessly integrate into computational notebooks, a favored tool for data analysis. Informed by prior work \cite{Browne2019WizardOO, Amershi2019GuidelinesFH, McNutt2023OnTD, Horvitz1999PrinciplesOM, Dahlbck1993WizardOO, Fraser1991SimulatingSS, Riek2012WizardOO} we develop our user interface, interactions, and the wizard protocol for building and raising suggestions. Informed by prior work on design principles for Human-AI interaction, we design the study such that future LLM-powered systems could simulate the wizard's actions with the appropriate data and prompts.

\interfaceFig
\subsection{User Interface}
We choose to integrate our assistant in computational notebooks as they are a popular medium for data analysis. In designing the assistant interface, we follow relevant findings from McNutt et al. \cite{McNutt2023OnTD}, which outlined the design space of code assistants in computational notebooks. A central design decision is the location of the assistant within the notebook UI. We opt for a side panel interface, which offers a global perspective of access to information for the assistant. This global scope is helpful because it implies that the suggestions integrate information from all parts of an analyst’s notebook. Additionally, by keeping the suggestions separate from the analyst's working notebook, we ensure our suggestions do not overly interfere with analysts' code and notes. We believe in empowering the analyst to exercise their own judgment in deciding whether to use the suggestions we provide.

In the side panel, suggestions exist as individual cards. In each suggestion card, we include the relevant context \cite{Amershi2019GuidelinesFH} at a cell or line granularity. Furthermore, as the focus of the study is to observe how suggestions are preferred by and affect analysts, we implement additional features to encourage analysts to observe a new suggestion. When new suggestions occur, the side panel shows a loading animation of variable duration to bring attention to them. The variable duration aims to simulate a real system computing and generating a suggestion \cite{Fraser1991SimulatingSS, Riek2012WizardOO}. Moreover, to make new suggestions easily distinguishable from old ones, we highlight the borders of each new recommended suggestion. Once analysts click on the suggestion, the highlight disappears. 

\subsection{User Interactions}
Regarding the assistant's interactions, we design the assistant to enable planning assistance. Because planning assistance brings about so many alternative approaches, it is less clear what suggestions should be offered and subsequently how these suggestions may affect analysts.
% \tim{I know I've used the same language but we need to find a way to say this more precisely. For example, what are the  open questions? why do we not know how to do it? We need to be super super clear about this and we need to consistenntly describe this from abstract, intro etc...} 
We want to help analysts gain insights into analysis decisions, rationales, and statistical thinking that they are previously unaware of. Consequently, we choose a design that focuses less on analyst initiative when interacting with the system. Analysts receive suggestions from the system without requiring specific action. Likewise, there is no explicit design for the analyst to control the topics that are generated or refine the suggestions. However, analysts are able to influence the assistant by writing specific comments within the notebook. 

To make the simulation more convincing, enable a sense of control in the analyst, and support efficient invocation or dismissal \cite{Amershi2019GuidelinesFH}, we include an on/off toggle for the assistant. To encourage comfort with the assistant, we display a startup message in which the assistant introduces itself when the analyst first toggles on the assistant \cite{Kahn2008DesignPF}. Likewise, to encourage granular user feedback \cite{Amershi2019GuidelinesFH}, we provide a thumbs up and a thumbs down button for each suggestion. Additionally, to support easy navigation between an often messy notebook \cite{Head2019ManagingMI, Kery2018TheSI, Rule2018ExplorationAE}, we let clicking on a suggestion automatically scroll the notebook to the corresponding context for that suggestion. Lastly, after early feedback from analysts, we include a copy button for suggested code blocks to enable analysts to quickly incorporate recommended code. 
\tim{great job with all this!}


\subsection{\woz Protocol}
In our \woz protocol, we simulate an AI-powered assistant for data analysis. \tim{One potential misunderstanding is that you simulate the entire LLM away. But actually you still use an LLM, you just relax the constraint to have an automated process that consistently creates the best prompts and consistently generates high quality feedback by allowing yourself to manually manage this process and LLM interaction (whereas analysts understandably may not know how and when to best utilize LLMs.)} Therefore, it is important to develop realistic suggestions that are helpful and reasonable from an LLM. 

\subsubsection{Creating Suggestions} 
\label{subsec:building_suggestions}
A wizard creating and delivering the suggestions raises a potential downside of being slower to respond than an automated system. To mitigate this effect, we choose to study with one analysis to allow us to prepare comments and suggestions. \tim{this subsubsection doesn't seem to be about creating suggestions but seems to be about potential limiations of the approach?} \tim{"limit the domain of possible suggestions" itself sounds like a HUGE downside and threat to validity. It's also confusing after your previous section 3 where you tried to give a comprehensive set of possible suggestions.} We plan for analysts interacting with our system to work with the same dataset and research question. This choice enables us to prepare common suggestions prior to the study that might be relevant. Since we already developed high-quality and often reusable suggestions through our analysis of a crowd-sourced analysis study (Section \ref{sec:suggestions}), we choose the same task and dataset from the crowd-sourced study for our \woz study. 

For dimensions such as {\interfont \texttt{Literature Review}} and {\interfont \texttt{How to Operationalize Constructs}}, the same or very similar suggestions could be given to different analysts. As a result, we prepare a spreadsheet of suggestions in these dimensions before the study.  \tim{might be confusing. The spreadsheet is to allow you fast copy paste? maybe refer back to your table here.} 

For other dimensions, such as {\interfont \texttt{Natural Language Intent to Code}} or {\interfont \texttt{Results Interpretation}}, the suggestions are closely tied to the context of the working analysis. Therefore, suggestions developed previously cannot be directly used. For these dimensions, we leverage ChatGPT \cite{ChatGPT} and construct prompts to build suggestions \tim{prior to the study}. Prior to the study, we create a general prompt introducing the analysis task and dataset. 

During the study, ChatGPT is tightly integrated into the suggestion development \tim{we should be consistent. are we building/developing/creating suggestions? I don't have a strong opinion but like creating.} process. Along with directly using the general prompt, the wizard crafts specific prompts for ChatGPT to generate the suggestion of interest. \tim{didd you do these from scratch every time? it reads that way.} Furthermore, the wizard uses ChatGPT to refine generations such as converting code between programming languages or shortening the length of a prior generation. Throughout this process, the wizard may manually adapt a prewritten suggestion or output of a ChatGPT generation to the current analysis (e.g., changing the wording or variable names in code). \tim{is this for correction / and to ensure high quality? (whereas even SOTA LLMs demonstrate these various mistakes?) } Overall, this protocol enables us to learn about the specific types of suggestions while incorporating the capabilities of current LLMs.

\wozFig
\subsubsection{Raising Suggestions} 
When and what suggestions we raise are guided by several principles. 

First, we raise suggestions relevant to the text in the working notebook with priority given to the latest additions \cite{Amershi2019GuidelinesFH}. We bias \tim{instead: especially focus on. Focus has positive connotation :) } suggestions toward planning assistance when possible as these suggestions are less understood. However, to maintain trust and show contextually relevant information \cite{Amershi2019GuidelinesFH, Horvitz1999PrinciplesOM}, we also provide suggestions in situations when it is clear the analyst needs execution assistance. Examples include when analysts are stuck on a coding task (e.g., debugging outputs) or when analysts write comments asking for specific help.

Next, to time suggestions based on the user's current progress \cite{Amershi2019GuidelinesFH}, we raise suggestions at a frequency commensurate with the level of activity or new information within the notebook. In other words, if the analyst has not updated their notebook for a while, we do not raise new suggestions. \tim{why is this good? if they didn't update that sounds to me like they could be stuck. Above that seems to be a trigger to help, which is the opposite?} Conversely, if analysts consistently update their notebooks, we generate suggestions more frequently. \tim{why is this a reasonable approach? } \ken{Hopefully, this sentence addresses this?}This serves to not bombard the analyst with suggestions when their focus may be elsewhere. Moreover, it ensures consistent behavior with respect to the timing of suggestions. \tim{what do you mean by that?} 

Finally, we simulate that the assistant can learn over time what suggestions are helpful to the analyst \cite{Amershi2019GuidelinesFH}. The types of suggestions we raise depend on whether the suggestions given so far are considered/taken. For instance, if the analyst disregards many suggestions that consider alternative variables, we raise these suggestions less often.


\subsection{Implementation}
We implement the wizard and user interface for the Juptyer environment \cite{Prez2007IPythonAS} as a JupyterLab extension. We extend the JupyterLab Commenting and Annotation extension \cite{jupyterlabcomments} and incorporate two modes: wizard mode and analyst mode. Wizard mode and analyst mode work with the same underlying notebook file and share a similar side panel interface. In wizard mode, the wizard can highlight code or cells and add corresponding suggestions to the side panel. All suggestions are stored on disk as an underlying suggestion file. The extension, when in analyst mode, polls this file for changes and updates the side panel when new suggestions are added to the file. 

In the study, both the analyst and wizard work with the same notebook in the same file system.  We host the notebook on the wizard's machine. Accordingly, we connect the analyst’s machine remotely to the wizard’s machine using SHH. To ensure the wizard cannot update the actual notebook contents, wizard mode has no edit permissions. 

To support the development of future notebook assistant interfaces, we release our JupyterLab extension code to the public \footnote{\githubURL}.

% \tim{we can consider sharing this code? how valuable to others would it be?}

==> 6-study.tex <==
\section{Study Protocol}
\label{sec:labstudy}
We conducted an exploratory lab study using our \woz protocol to learn what types of suggestions analysts prefer and how these suggestions might affect their workflow. 

\tableParticipants
\xhdr{Participants}
% With our study, we wanted to understand analysts' preferences towards and the subsequent impact of planning assistance. We imagine novice analysts may be too bogged down by execution challenges that there never is any time or consideration for analysis planning (even if offered planning assistance). Moreover, if even trained analysts struggle with analysis planning \cite{Kale2019DecisionMakingUU, Liu2019PathsEP}, then understanding how to support these analysts is a crucial first step to supporting all analysts. Therefore, we focused on recruiting data analysts who are already familiar with statistical analysis. 
We recruited data analysts who were already familiar with statistical analysis and programming and were likely to engage in analytical reasoning. 
% We imagine \tim{can we cite related work to inform this expectation and provide some justification?} novice analysts may be too bogged down by execution challenges that there never is any time or consideration for analysis planning (even if offered planning assistance). 
We considered novice analysts lacking programming expertise to be too limited by execution challenges \cite{Liu2020UnderstandingTR, Kandel2012EnterpriseDA} to consider analysis planning even when provided assistance. Similarly, we thought that individuals lacking general statistical knowledge would struggle to comprehend the full range of recommended decisions \cite{Liu2019PathsEP}. Since even trained analysts face difficulties in analysis planning \cite{Kale2019DecisionMakingUU}, supporting these analysts is a crucial initial step in supporting all analysts.

% \tim{why?}\ken{Not sure if I defended the choice of analysts enough} 
We contacted data analysts through analysis-related mailing lists at our institution. We advertised an opportunity to work with a data analysis assistant tool.
% In the initial interest form, we asked analysts to self-rate their statistical background on a 5-point scale (higher being more familiar). In this scale, 4 described analysts who have taken graduate-level courses related to statistical analysis, and 5 described analysts having multiple years of experience with real-world projects involving statistical and data analysis. \tim{will readers ask about 1-3?} We also asked analysts to rate their familiarity with R or Python on a 5-point scale with 1 “being equivalent to having taken an introductory course” and 5 being having “5+ years of industry experience”. 
A total of 60 analysts volunteered, which we filtered down to 13. 
We selected analysts with the highest self-reported language and statistics proficiency (4s and 5s on a 5-point scale), background diversity, and familiarity with writing analyses in computational notebooks.
% We aimed for analysts from diverse domain backgrounds, who were quite familiar with R or Python, and have non-trivial experience in statistical analysis. 
% We wanted to observe analysts who are unlikely to be bogged down by execution challenges but likely to engage in analytical reasoning.
% Moreover, we made sure to select analysts who have not seen the dataset or study before. \tim{did that actually occur?}
% We also selected analysts who were familiar with writing analyses in computational notebooks.
Table \ref{tab:participants} shows a summary of participants.

\xhdr{Data}
As mentioned in Section \ref{subsec:building_suggestions}, analysts in our study worked through the same task as the teams in the crowd-sourced data analysis study~\cite{Silberzahn2018ManyAO}. To ease dataset understanding, help analysts focus on planning, and help us study a variety of suggestions over the course of one lab session, we made minor adaptions to the dataset. % Due to our study's time constraints, \tim{we can say that "nicer". it's not a constraint/downside. Instead, you made minor adaptations to make XYZ easier, help analysts focus on XYZ, to enable us to study a variety of suggestions over the course of an X-hour study.... This is a general pattern in my feedback. Always say why you made a choice and why this was a good reason/process to do so. Be careful with things that sound like downsides and explain them and what you did about them.} we made minor adaptations to the dataset. 
We wanted to allow analysts to identify important analytical decisions while still preserving realistic variation in the data; therefore, We sampled a subset of the data to improve computational efficiency while maintaining the overall distribution of the dependent variable (red cards) across levels of the main independent variable (skin tone).
% Additionally, we focused on the most relevant independent variables based on the analyses from the original crowd-sourced study. Specifically, we included the ten most frequently used variables across all analyst teams. 
Additionally, we focused on the ten most frequently used variables across analyst teams in the original crowd-sourced study. 
% Specifically, we included the ten most frequently used variables across all analyst teams. 

\xhdr{Procedure}
Our study was conducted in a lab using a designated MacBook Pro computer on a 27-inch monitor. One author, in the lab with participants, served as the coordinator. For all study sessions, another author, who developed the JupyterLab extension and prepared the suggestions, acted as the wizard. This ensured that the behavior of the assistant remained consistent across analysts. 

Before the study, we obtained analysts’ consent to record their screens and audio. We also asked analysts about their preferred programming language and the libraries they often worked with and might expect to work with for the study. We created a notebook for each analyst in their preferred language and installed, imported, and tested all libraries mentioned. We wanted to ensure an analysis environment that was familiar and as close to analysts' own experiences as possible.

We recorded the study using a Zoom meeting. The wizard attended the virtual meeting under the pseudonym of the coordinator and was physically in a separate room. Analysts were unaware of the wizard and that the wizard was able to hear and see their screen.

The study lasted roughly 2 hours and consisted of three phases. In the first phase of about 15 minutes, the coordinator introduced the task and guided analysts through the JupyterLab notebook. We discuss the notebook in detail in Appendix~\ref{appendix:notebook_detail}.

Inspired by Jun et al. \cite{Jun2021HypothesisFE}, which aimed to understand analysts' statistical thinking and sensemaking processes, we asked analysts to imagine they were leading a research team to answer the research question and that their team collected the dataset used in the study 
% \tim{I'm confused -- I thought someone other than Eunice collected the red cards data?!} 
To prime analysts to consider how their decisions could affect results, we told them that their analysis results would impact a major policy decision, i.e., whether the soccer league invests money in bias training;  we stressed the importance of having reasonable rationales for their analysis decisions and that their decisions must be robust against alternative assumptions.Likewise, to encourage comfort with the lab environment, we mentioned that we were not interested in the completion of the analysis but in their analysis process. 

Once analysts were familiar with the task, the coordinator toggled on the assistant and introduced how its suggestions were raised. We described what the system can do (e.g., make suggestions based on the notebook context), being careful not to anthropomorphize the assistant to facilitate accurate evaluations~\cite{Khadpe2020ConceptualMI}. 
% \tim{curious. why is the latter important?}

In the second phase, lasting around 1 hour and 15 minutes, analysts worked on the task while the wizard made suggestions. We encouraged analysts to think aloud or document their process in a notebook. They were free to use any external resources they saw fit. We wanted to give them adequate time to work through major phases of the analysis process (i.e., exploring the data, identifying relevant variables, running a model, and interpreting the results). 

% Most analysts did not finish their analysis  \tim{that sounds like a contrast to the prev sentence. is this a concern? does it add limitations?}\ken{yes can discuss in limitations that they didn't come to the end with a full and confident analysis conclusion.} 

In the third and final phase, the study coordinator conducted a semi-structured interview lasting 30 minutes. We asked analysts to review each suggestion they saw, give a positive, neutral, or negative reaction to whether the suggestion was helpful, and explain why . 
% \tim{do what degree did they do this live vs all retrospective during this interview?} 
Afterward, we asked questions that explored the impact the assistant's recommendations had on the analyst's process, what analysts valued from the assistant, and what sorts of actions or information they would have liked the assistant to provide. At the end of the study, we revealed how the assistant actually worked, that is, its suggestions were a mix of manually written and ChatGPT-generated text, and its curation and raising of suggestions were done by a human wizard. 

Analysts received a \$50 Amazon gift card as compensation for their time. 
% This study was determined exempt by the IRB at our institution. 


\xhdr{Data Analysis}
In addition to the recordings of participants’ audio and screens, the study coordinator took notes throughout the analysis phase and the semi-structured interview. One author viewed the recordings and transcribed all episodes of interest to the analyst-assistant collaboration process. To define common themes that emerged, two of the authors conducted iterative open coding. These authors met over multiple sessions to refine codes on any
observations related to the helpfulness of suggestions and the overall interaction between the analyst and assistant. They also met to code all suggestions that were raised into the suggestion categories summarized in Table \ref{tab:suggestions}.

% \tim{should we say anything here about agreement between the two, how disagreement was resolved?}

% . \tim{great, make these specific section references}\ken{I think supplemental material is different then appendix}

% We also tracked all suggestions that were raised and documented analysts' ratings of their helpfulness (i.e., positive, neutral, negative). \ken{TODO add sentence or two based on results}




==> 7-results.tex <==

\resultsFig

\section{Results}
\label{sec:results}
% From our \woz study, we observe \tim{be consistent in terms of present  or past tense} many interesting behaviors and reactions to our system that bring new insights into  Human-AI collaboration in the context of a data analysis assistant. 


Our \woz study explored two main questions: ``\emph{what characterizes helpful suggestions?} (\textbf{RQ2}), and \emph{how do these suggestions impact analysts' workflows?} (\textbf{RQ3}).

With respect to \textbf{RQ2}, we found that analysts preferred suggestions that matched their analysis plan and their statistical and domain background (Sec.~\ref{sec:results_who}).  They preferred both execution \textit{and} planning assistance, though planning required more cognitive effort (Sec.~\ref{sec:results_what_assistance}). As a result, explanations provided in code, code comments, and natural language greatly assisted analysts in understanding the intent and rationale of suggestions (Sec.~\ref{sec:results_what_qualities}). Due to the extra effort to consider planning assistance, analysts valued suggestions that were well-timed to their current task (Sec.~\ref{sec:results_when}).

For \textbf{RQ3}, we found well-timed and contextual planning assistance often helped analysts consider and make alternative decisions (Secs.~\ref{sec:results_what} and ~\ref{sec:results_when}). In contrast, analysts were reluctant to accept suggestions that mismatched with their expertise or task. Likewise, we observed potential drawbacks of AI-assistance: some analysts became distracted or overly reliant on the assistant's suggestions, often without taking the time to critically assess their relevance or correctness (Sec.~\ref{sec:results_why}). Nevertheless, these impacts were not uniform across all scenarios and varied depending on the individual analyst (Sec.~\ref{sec:results_who}), the type of assistance (Sec.~\ref{sec:results_what}), and when the suggestion was made (Sec.~\ref{sec:results_when}).

% Overall, analysts' reactions to raised suggestions  show that suggestions from all categories were helpful, 
Overall, analysts generally saw suggestions from all categories as helpful (Fig. \ref{fig:suggestion_reactions}),
% although some found the assistance to be unhelpful in certain situations (Sec.~\ref{sec:results_who} and Sec.~\ref{sec:results_when}). 
some situations excepted (Secs.~\ref{sec:results_who} and ~\ref{sec:results_when}).
Triangulating their ratings with interview data revealed subtleties in analyst-assistant interaction dynamics, which we summarize in Fig. \ref{fig:results}. 
 Here, we consider suggestion helpfulness, their analysis impact, and the overall experience using a "\emph{Who, What, When, Why, and How}" framework to organize our findings.
While analysts expressed preferences for ``\emph{where}'' the assistant should be placed on the UI, these preferences did not fundamentally impact their overall workflow, and so we include our observation to this effect in the appendix. 
% Thus, we include our observations regarding assistant's location in the appendix.
 % To this end, we describe observations that relate to the analyst's background (\emph{Who}, Sec. \ref{sec:results_who}; Fig. \ref{fig:results}G), the suggestion content (\emph{What}, Sec. \ref{sec:results_what}; Fig. \ref{fig:results}E), the timing of suggestions (\emph{When}, Sec. \ref{sec:results_when}; Fig. \ref{fig:results}E), reasons to use a data analysis assistant (\emph{Why}, Sec. \ref{sec:results_why}), and analyst vs. assistant initiative (\emph{How}, Sec. \ref{sec:results_how}; Fig. \ref{fig:results}A). 
 % ~\ref{appendix:results_where}.



% \subsection{Results Summary}
% \label{sec:results_summary}

% In our \woz study, we aimed to explore two main questions: what characterizes helpful suggestions (RQ2) and how these suggestions impact analysts' workflows (RQ3).

% With respect to RQ2, we find suggestions are most preferred when they match the analysts' analysis plan, and statistical and domain background (Sec.~\ref{sec:results_who}). Furthermore, we notice analysts value suggestions when they are responsive and relevant to their current workflows (Sec.~\ref{sec:results_when}). Finally, explanations provided in plain language, supplemented by code comments and the code itself, greatly assist in analysts' understanding of the intent and logic of suggestions (Sec.~\ref{sec:results_what_qualities}).

% For RQ3, while we find planning assistance often helps analysts broaden their consideration of alternative decisions (Sec.~\ref{sec:results_what}), we observe a potential drawback in that analysts become more distracted and less engaged (Sec.~\ref{sec:results_why}). Moreover, these impacts are not uniform across all scenarios. They vary depending on the individual analyst (Sec.\ref{sec:results_who}), the way the suggestion content is presented (Sec.\ref{sec:results_what}), and when the suggestion is made (Sec.~\ref{sec:results_when}).

% In section \ref{sec:discussion}, we discuss the implications of our findings and design considerations to improve suggestion helpfulness and analyst engagement.


\subsection{\emph{Who}---Analyst Background}
\label{sec:results_who}

Our study revealed many aspects of an analyst's background that influenced their perception of suggestions and overall experience. Here, we discuss their analysis plan (Sec. \ref{sec:results_who_analysisplan}), statistical and domain backgrounds (Sec. \ref{sec:results_who_expertise}), and prior experiences with and curiosity about AI-based assistants (Sec. \ref{sec:results_who_curiosity}). 



\subsubsection{Analysis Plan}
\label{sec:results_who_analysisplan}
Analysts exhibited varying levels of analysis forethought and rigidity in their analysis plans. While all analysts had a rough plan, some took extra time to explicitly detail their analysis steps [A3, A5, A9, A10, A11]. For example, A9 spent the first 20 minutes planning on scratch paper before writing a single line of code. 
Others employed on familiar strategies, for instance, A4's initial plan drew on their familiarity with  Species Distribution Modeling \cite{Franklin2010MappingSD}.
% ---a statistical approach that predicts species' geographic distribution based on environmental variables.
% In other instances, analysts considered approaches that were familiar. F
% for instance, A4, who was familiar with Species Distribution Modeling \cite{Franklin2010MappingSD} (i.e., a statistical approach that predicts species' geographic distribution based on environmental variables), mentioned that approach as an initial idea for planning. 
% \tim{sounds interesting -- was this at all related to the task?}
% Likewise, 
Analysts (8/13) often liked suggestions that matched their own ideas or plans.
% [A3, A4, A5, A7, A9, A11, A12, A13]. 
They appreciated that the included code offered additional execution assistance to implement their plan. 
For example, in reference to a suggestion recommending Age as a variable, A12 noted \shortquote{I really liked this one... I think it actually somehow knew that I was going to do this, and then it suggested a very efficient way to do so.} 
Furthermore, for A5, such suggestions reaffirmed their decisions: \shortquote{The assistant actually gave the same conclusion that I had typed, so that was helpful.} 
% Overall, analysts frequently favored suggestions that matched their analysis plan. 
% \am{weak return}
% Given variations in how they plan, they also wanted ways to specify the level of assistance they received~(Sec.~\ref{sec:results_how}).
Given these planning variations, it is unsurprising that participants also expressed interest in controlling the level of assistance received~(Sec.~\ref{sec:results_how}).

\subsubsection{Statistical and Domain Knowledge Expertise}
\label{sec:results_who_expertise}
% We observed disparities in individual levels of statistical and domain expertise across analysts and throughout the course of the analysis. This affected how analysts reacted to the assistant's suggestions. 
Analysts' varying levels of statistical and domain expertise affected how they reacted to presented suggestions.
Most analysts (11/13) had no trouble understanding the feedback for most suggestions, with many (10/13) finding them to be well-matched with their expertise and helped them consider new approaches.
% [A1, A2, A3, A4, A5, A7, A9, A10, A11, A12, A13] \jeff{This is a rather long list, maybe (11/13 participants) or somesuch would be more useful?} \tim{+1 (and you can keep the records e.g. in comment or elsewhere}. 
% Likewise, 10/13 analysts found suggestions helpful when they were well-matched with their expertise and helped them consider new approaches.
% [A2, A3, A4, A5, A6, A7, A9, A10, A12, A13]. 
% For example, A7 appreciated an important reminder from the assistant about how to encode a categorical variable: \shortquote{This is a great suggestion. I didn't know I could just do that instead of having to encode it. So it takes care of it instantly.} However, a few analysts found some suggestions overly basic for their own expertise and therefore did not benefit from them [A1 A3, A5, A7, A8]. For example, A1 did not gain any insight from a results interpretation suggestion: \shortquote{It was giving me comments on my results. It was not telling me whether it was good or bad which I knew already.} However, these same analysts also noted that the suggestions would be quite helpful for beginners [A1, A3, A7].  
However, some analysts found suggestions overly basic and unnecessary [A1 A3, A5, A7, A8], due to their statistical expertise. This was most evident with the results interpretation suggestions created using ChatGPT. Some analysts liked these suggestions [A5, A6, A7, A10, A11, A12], while others adopted a more neutral stance [A8, A4]. A1, a statistics professor with extensive expertise in computational social science, regarded the suggestions as unhelpful: \shortquote{It was giving me comments on my results. It was not telling me whether it was good or bad which I knew already.} 

Suggestions were occasionally unfamiliar since some analysts lacked an adequate statistical background [A3, A5, A6, A8, A9, A13]. This led to varying behaviors: A3, A5, and A13 chose to ignore unfamiliar suggestions completely;
A6 and A8 spent time trying to understand the suggestion but were left confused; and A9 considered referencing external sources to interpret the suggestions: \shortquote{My first idea is to try and copy and search on the internet to see how this kind of generalized linear model could help me.}
Suggestions that were mismatched with the analyst's statistical background were unhelpful or required significant additional effort to understand, highlighting that assistant usage might usefully begin with an alignment phase. 
% This compounds the already intense concentration and effort needed to consider planning assistance~(Sec.~\ref{sec:results_what_assistance}).\am{suggesting what}

% \subsubsection{Prior Experience with and Curiosity about AI-based Assistants}
\subsubsection{Prior Experience with AI-based Assistants}
\label{sec:results_who_curiosity}

We found that analysts' own past experiences with AI led to behaviors and reactions that diverged from the immediate analysis task. 
Analysts had mixed prior experiences working with AI-based code assistants (i.e., Github Copilot, ChatGPT). Over half (7/13) had no experience while others ranged from using code assistants a few times in total to regularly using them (Table~\ref{tab:participants}). 
These prior experiences caused some analysts to be skeptical about suggestion correctness. For instance, A8 and A13 questioned the resources that informed it.
Referring to a suggestion that referenced external studies, A8 mentioned, \shortquote{I have less trust of something that is a more generated summary of stuff that exists outside of the notebook, that I didn't know where the information came from.}
% \tim{do you discuss this later? interesting and important observation/design rec around trust}
% In contrast, A4 was surprised by the suggestions the assistant provided given prior experience using ChatGPT: \longquote{I am very surprised because when you ask ChatGPT about something really obscure, it might give you good information or something bullshit, and this seemed tightly reasoned. It's a little spooky.}\am{comment on the wizard of oz study nature}
Some analysts became distracted by the novelty of using an assistant. For instance, A8 was distracted from their task by their curiosity: \longquote{It made me want to understand how this (worked). I was getting distracted. What is it learning from? Is it from the data and knows all the variables or from what I am asking for? I feel like I was experimenting a lot with putting little notes and seeing what would happen.}  
% We suggest that as AI-based assistants become ubiquitous, such issues will likely be more limited.
% Without knowing many details about how the system worked, some analysts were curious about the assistant [A1, A4, A8, A12] \am{in what capacity}. 
% % A4, for example, was open to what the assistant suggests: \shortquote{We can try a basic linear model, which should not be very good, but I'm curious to see what (the assistant) tells me after that.} 
% % A8, on the other hand, became more distracted by their curiosity: 
% For instance, A8 was distracted from their task by their curiosity: \longquote{It made me want to understand how this (worked). I was getting distracted. What is it learning from? Is it from the data and knows all the variables or from what I am asking for? I feel like I was experimenting a lot with putting little notes and seeing what would happen.}  
% We suggest that as AI-based assistants become ubiquitous, such issues will likely be more limited. 
Our observations agree with existing work~\cite{Liao2022DesigningFR} that models trustworthy AI, where a user's attitude towards an AI system (and therefore subsequent reactions to the system) depends on individual, environmental, and cultural contexts in addition to the system's trustworthy cues.
% \mgm{Conclusions to each section may be helpful, esp if people are skimming. What was agreed upon vs not among different analysts}



\subsection{\emph{What}---Suggestion Content}
\label{sec:results_what}
% We noticed broader qualities relating to \jeff{Sentence incomplete!}
Though we found that the exact category of planning content (e.g. Table \ref{tab:suggestions}'s categories) was less important for depicting the helpfulness of a suggestion~(Fig.~\ref{fig:suggestion_reactions}), the type (planning and execution) and specificity of assistance were preferred in different situations (Sec. \ref{sec:results_what_assistance}). Moreover, we found well-reasoned explanations to be important to analysts (Sec. \ref{sec:results_what_qualities}).


\subsubsection{Execution vs. Planning Assistance}
\label{sec:results_what_assistance}
All analysts appreciated execution assistance, occasionally rating it negatively only when it came too late or differed from what they had intended. In our study, execution assistance occurred either on its own---when analysts were struggling with executing their plan---or as part of intended planning suggestions. 
Analysts (8/13) appreciated that execution assistance saved time and prevented them from having to search the internet.
% [A1, A3, A4, A5, A7, A9, A11, A12]. 
For example, A3 liked that a suggestion to consider a BMI variable included the code to calculate it, noting that \shortquote{I don't know how to calculate BMI off the top of my head, and it was like `Hey, here's how you calculate it'. Perfect, saves me a Google.} These preferences are in line with prior observations~\cite{Vaithilingam2022ExpectationVE, Ziegler2022ProductivityAO} that expediency and reduced online searching are major perceived benefits of AI-based code assistants. 
Some analysts would have preferred even more execution assistance [A2, A3, A4, A5, A13]. For example, A5 and A13 expected more help when faced with errors, while A3 wanted it to make visualization for them.
% . Likewise, A3 wanted the assistant to execute the code for them, such as for visualizations.  
% \mgm{i think there was more people who wanted this, on the Mural from day 1 --> my side of stickies --> interaction considerations --> prefers automatic, it was P4 too and then 2 other stickies that don't have a Participant written down}. 
% Similarly, A2 wanted high-level help with \shortquote{understanding the differences between libraries.}

Reciprocally, most analysis found planning assistants to be helpful, although this utility 
% With respect to planning assistance, most analysts found it to be helpful. Helpfulness 
depended less on suggestion type than on the timing (Sec. \ref{sec:results_when}).
% with respect to analysts' own paths (Sec. \ref{sec:results_when}). 
Most analysts (12/13) noted that planning suggestions often presented ideas that they had not previously considered.
% [A2, A3, A4, A5, A6, A7, A8, A9, A10, A11, A12, A13]. 
For instance, A10 contrasted our assistant's planning merits with other assistants: \longquote{Auto-complete code (assistants) are very good, but they are looking at what you are doing right now and maybe the last cell. This agent could take a more overall approach and help you think about the overall approach.}
In other situations, the suggestions also helped analysts realize key steps they would have otherwise missed. For instance, A2 found observed that  \shortquote{this is helpful. I didn't realize that skin tone rating was a combination of rater one and rater two.} 
% \shortquote{Interesting, this is helpful. I didn't realize that skin tone rating was a combination of rater one and rater two.} 

However, while most suggestions the assistant presented were tied to specific moments in the analysis process, some analysts wanted broader analysis planning help [A2, A3, A6, A7, A8].  A3, for example, mentioned how at the beginning of the analysis, \shortquote{recommendations for how to think about the problem would (have been) good.} Similarly, A2 wanted suggestions that could provide a whole analysis plan: \longquote{Given the dependent variables and the data structures, what are some of the analyses I could run? If I need to run different analyses, how would I need to transform the data, with suggestions or sample code of how I can do that?} In these situations, analysts might benefit from workflow scaffolding recommendations similar to those in \textit{Lodestar}~\cite{Raghunandan2022LodestarSI} or \textit{litvis}~\cite{Wood2019DesignEW}.



\subsubsection{Suggestion Explanations}
\label{sec:results_what_qualities}
Several analysts  [A2, A5, A6, A7, A8, A9] specifically noted that they liked the explanations included in the suggestions. 

For A5 and A9, both the included code and comments acted as explanations that helped them understand what the assistant was trying to do. 
% \tim{bit confused here about "explanation" vs "code". is the comments the explanation?} 
A9 felt that explanations helped bridge a lack of trust in the assistant about a new calls-per-game variable suggestion, noting that \shortquote{I'm not trust(ing) with the calls-per-game, so I checked with every line of the code if they actually write what I'm thinking about.} Meanwhile, explanations for why a planning suggestion should be considered were also preferred. A2 was especially enthusiastic: \shortquote{I love the justification of why you would want to use age.} 
% Similarly, A7 valued the pros and cons offered by the explanation, which they felt gave them control of the final decision. 
In contrast, A8 connected their statistical expertise (Sec. \ref{sec:results_who_expertise}) to their willingness to accept a suggestion:
% they liked the suggestion overall and the explanation seemed to be logically sound, but they were not sure whether it was the right path to follow:
\longquote{I don't know if I was being led astray by the assistant but I found this very convincing. But I don't have the fresh statistical knowledge to actually know if it was a good statistical approach or not.}
% \longquote{I haven't thought about this kind of statistics since I was a sophomore 13 years ago... The description here seemed like this would be better... I don't know if I was being led astray by the assistant but I found this very convincing. But I don't have the fresh statistical knowledge to actually know if it was a good statistical approach or not.}


% \mgm{If i remember correctly, there were some participants who were more likely to like the outputs because of the justifications. Specifically thinking about this quote: "I am very surprised at ... because when you ask ChatGPT about something really obscure it might give you good information or something bullshit, and this seemed tightly reasoned. It's a little spooky" - 1:30:30}

% \mgm{Other explanation-related stickies that I think are interesting: 

% \textbf{Likes that it's a pro & con in explanation for decision making}
% Star status – this was something he didn't go over either. Would've loved to if he had more time
% A good suggestion, though he didn't use it
% Likes that it gives an `although' so it gives a pro and a con as information for him to make the final decision -1:40:10 -p7

% \textbf{Uncertainty, but the narrative seems good so more likely to follow}
% Modeling strategy GLM
% haven't thought about these kinds of statistics since she was a sophomore in college 13 years ago
% So maybe it is a good idea? I don't know? But the description here makes iher think it might be better. So went back to other studies to see what they had done
% She found it very convincing to see if it was a good idea, and don;t know if she was led astray by the assistant but doesnt have the fresh statistical knowledge to know if it was the right idea
% But given the narrative was like “seems great” :1:11:30 -P8
% }

The explanations were also seen as detrimental at times [A2, A6, A8, A13], depending on the analyst's expertise (Sec. \ref{sec:results_who_expertise}) and focus on their own analysis plan (Sec. \ref{sec:results_when}). A13 ignored suggestions when \shortquote{there is too much explanation}. Similarly, A2, who appreciated the explanation for the inclusion of age, thought that some suggestions contained too much text. 
% From a cost-benefit perspective~\cite{vasconcelos2023explanations}, the cost of engaging with the suggestions was too high.
A6 noted that \shortquote{Because I didn't understand why it was trying to include goals per game, I was kind of confused}. 
This is akin to how programmers working with AI-based code assistants sometimes struggle to understand the suggested code~\cite{Vaithilingam2022ExpectationVE}, highlighting the importance and fragility of explanation design.
% This sentiment is similar to those expressed by programmers working with AI-based code assistants; they struggled to understand the suggested code which hindered their ability to solve tasks ~\cite{Vaithilingam2022ExpectationVE}.
% Moreover, for A6, the explanation was insufficient and so confused them: \shortquote{Because I didn't understand why it was trying to include goals per game, I was kind of confused}. This sentiment is similar to those expressed by programmers working with AI-based code assistants; they struggled to understand the suggested code which hindered their ability to solve tasks ~\cite{Vaithilingam2022ExpectationVE}.
% \mgm{New paragraph? since not about explanations?} 


\subsection{\emph{When}---Timing of Suggestion}
\label{sec:results_when}
% A common factor that influenced analysts' perception of suggestions' helpfulness was the timing of suggestion presentation relative to their current progression and goals.
% The timing of when a suggestion was presented (relative to the current task) was central to whether or not analysts perceived it as helpful.
Timing has long been a central part of designing interactions with autonomous agents, and like previous studies~\cite{Horvitz1999PrinciplesOM, Fogarty2005PredictingHI}, we find that inopportunely offered suggestions risk being ignored.
% and \am{we find blah blah blah}
% in the end-to-end analysis process.  
% Many analysts found some suggestions to be irrelevant to their plan and thus unhelpful (9/13 analysts).
% [A1, A2, A3, A4, A5, A8, A10, A12, A13]. 

We observed that when engrossed in a particular analytical task, analysts were often resistant to diverting their focus toward distracting suggestions. 
% When analysts  [A5, A6, A10, A11, A12, A13] found the suggestions out of sync with their current analysis plans, they would ignore them to continue their previous line of thinking. 
For instance, A5 found that suggestions were often discordant with their current objectives:
% For A5, suggestions often seemed unresponsive to their current workflow: 
\longquote{very often the suggestions aren't in line with what you're currently typing. It goes in a whole different direction, and now you have to think of whether you want to take that direction or your direction.} 
Similarly, A3 wanted to focus on their current step: \shortquote{``I ignored it because I was focused on the variables at the time.} For A5, poor timing also led them to ignore it: \shortquote{I don't know if this was relevant or not. I didn't read it completely because I was trying to complete what I already started.} 
% Timing issues also slowed down A5's process since they had to stop and consider the merits of the suggested direction. 
% Given the costs of considering planning assistance, appropriate or non-intrusive timing of suggestions is even more crucial. 
Notably, most analysts (9/13) felt that ``unhelpful'' suggestions, would have been useful if they had been offered at a different moment. 






% % In most situations, when analysts focused on their own plan, suggestions considered unhelpful at the moment would have been helpful if offered at a different time (9/13 analysts).
% % \longquote{(With) this assistant, very often the suggestions aren't in line with what you're currently typing. It goes in a whole different direction, and now you have to think of whether you want to take that direction or your direction.} In most situations, when analysts focused on their own plan, suggestions considered unhelpful at the moment would have been helpful if offered at a different time (9/13 analysts).
% % [A2, A3, A6, A7, A8, A9, A10, A11, A13]. 
% % Many analysts thought unhelpful suggestions would have been helpful later on [A6, A7, A8, A9, A10, A11].  
% % For A7 and A10, 
% % Yet, some suggestions that were unhelpful in the moment aided in future decision making. 
% For example, A7 mentioned: \shortquote{If I think it deviates too much, then I ignore it. There were a couple of times for the CHI-squared where I was like `Oh yeah that's a good idea.' I didn't do it at the time, but I put a pin on it.} In other cases, analysts  [A3, A6, A13] thought the suggestions came past after they were needed in their analysis. A6 would have preferred a covariate suggestion to come earlier: \shortquote{It did explain how it would be necessary, but maybe if it came before I did the covariate analysis (and) before I coded it out}.



When suggestions deviated only slightly from the current tasks analysts [A2, A5, A7, A9, A12] were open to them. For instance, while working through some statistical models, A7 took a recommendation to use the existing birthday column to create an age variable: \longquote{Honestly, birthday didn't hit me at that moment before the suggestion that popped up to calculate age. Without the suggestion, I wouldn't have thought of it unless I ended up reading about it and then including it a lot later.} This suggests that while suggestions should be aware of the current task, they need not \emph{exclusively} service that task as adjacent ones might usefully highlight alternative analysis paths---a key planning assistant goal.

% \tim{somewhat of a note to myself: do we discuss anywhere that "perceived helpful by analyst" may not be the only important outcome. They may all feel disrupted but what if it was an important thing they missed or that would have impacted their conclusions?}

Inherent in these observations is the tension between not disrupting the analyst and highlighting choices that might impact the analyst's conclusions. 
% Given the consequences of spurious analysis conclusions, the perceived helpfulness of suggestions may not be the only important outcome. 
% Similarly, 
From a cost-benefit perspective \cite{vasconcelos2023explanations}, execution assistance is less intrusive, with its time-saving benefits more easily recognizable. Conversely, planning assistance demands more mental effort as analysts evaluate multiple analytical paths, underlying rationales, and the alignment with their prevailing strategies. 
% \tim{and in addition implementing these plans likely would come with additional cost, right?}\ken{yes but this can be reduced through exec assistance. The ones mentioned so far are I think the most central at being costly} 
This complicates the assessment of the utility of planning assistance and amplifies the drawbacks of sub-optimal suggestions.
% We discuss this in Sec.~\ref{sec:discussion_helpful} and ~\ref{sec:discussion_balance}.


% Further, the perceived "unhelpfulness" of some planning suggestions was often due to \textit{when} these suggestions were presented~(Sec.~\ref{sec:results_when}).




\subsection{\emph{Why}---Reasons to Work with the Assistant}
\label{sec:results_why}
% \mgm{An intro sentence about what we mean by 'why' could be helpful, since first few sentences now summarize things that were already said}
% Analysts expressed a variety of preferences for \textit{why} they would want to work with a planning enabled assistant, inclyding its  its impacts on their workflows (\textbf{RQ3})
% We now describe analysts' overall experiences with the assistant and explore the reasons \textit{why} they want to use one. 
% These reasons are influenced by its impacts on their workflows (\textbf{RQ3}), which is in turn shaped by various elements of the assistant, such as the timing (Sec. \ref{sec:results_when}) and content (Sec. \ref{sec:results_what}) of the suggestions.

Most analysts (11/13) thought the assistant was helpful for both planning and execution-centric tasks, and expressed a variety of preferences as to \emph{why} they would want to work with this style of assistant.
% in their analysis process.
% [A2, A3, A4, A5, A6, A7, A8, A9, A10, A12, A13]. 
% They frequently liked the code that was provided (Sec. \ref{sec:results_what_assistance}), both for execution \textit{and} planning assistance. 
% For instance, A4 appreciated that the assistant saved them time by doing frequent coding tasks: \shortquote{The one thing that I really liked about it is that it saves me from having to do a lot of mundane stuff like setting up a testing and training dataset for some sort of machine learning model.} 



% \am{boiler plate and blank page problem are great make them be more featured}

%  (Sec. \ref{sec:results_what_assistance})
Analysts valued the planning assistance content provided by the assistant.
For instance, A9 found it helped them to consider alternative decisions: \shortquote{The (assistant) is helpful for me to indicate some aspects to think about. Though I did not take all of them, I see this is something that I may need to take a look at.} Furthermore, A2 liked having a clear rationale for why they should incorporate a suggestion (Sec. \ref{sec:results_what_qualities}): 
\longquote{As compared to when I'm typing in Gmail where it (suggests) words, this I find is much more helpful because it not only gives me the code but also gives the justification and rationale.} 
This suggests that planning assistance can be perceived as being of use to the data analysis process. 
% \longquote{I see a lot of potential and utility for this. As compared to when I'm typing in Gmail where it (suggests) words, this I find is much more helpful because it not only gives me the code but also gives the justification and rationale.} 

% Gordon \etal{} \cite{gordon2023co} notes that some of these beliefs 
% \am{this also has some to do with positioning and the culturallly understood role that it has, cf andy's ai-audit paper}

Even though our design primarily was centered on helping analysts consider alternative but reasonable approaches, they also frequently liked execution assistance. 
% Despite our design that mainly provided suggestions to help analysts consider alternative but reasonable approaches, analysts frequently liked execution assistance. 
For instance, A4 appreciated that \shortquote{it saves me from having to do a lot of mundane stuff like setting up a testing and training dataset for some sort of machine learning model.}
Similarly, A5 appreciated execution assistance for helping them move past roadblocks, noting that when \shortquote{you are stuck... and (the assistant saved) you that trouble of going somewhere else and googling things.}
% \shortquote{It was fascinating, to be honest. Because very often you're doing things, and you are stuck... and (the assistant saved) you that trouble of going somewhere else and googling things.}
This is consistent with the preferences found in prior works that studied code execution assistants \cite{Vaswani2017AttentionIA, Liang2023UnderstandingTU, Ross2023ThePA}, and suggests that having both both planning \emph{and} execution is critical for the design of this style of assistant. 
 
However, given the quality and quantity of assistance provided by our assistant, A8 believed that it made them less engaged in critical thinking. For A8, the reason to use the assistant was to reduce their own cognitive load rather than to have an AI guide their decision making: \shortquote{I feel like this `friend' was great, but it also made me this clicking machine (rather) than an analytical thinker... Autopilot was a welcome path that I could choose.} This follows the findings in empirical Human-AI collaboration studies in which people often over-rely on AI support~\cite{bansal2021does, buccinca2021trust, lai2019human, Buccinca2020ProxyTA}.
% am: todo, if accepted add cites to tarot paper + leilani and michael's health rec paper which also says this
% \am{wip} Similarly, the ``position''~\cite{gordon2023co} that the system tool (assistant rather than evaluator) was likely central to this perspective. 

% \tim{We should discuss this later if we haven't yet. danger to make things worse, especially if the assistant is not worthy of the trust put in it.}

% Similarly,  A4 appreciated the reasoning behind suggestions and compared it to that of existing assistants: \shortquote{I am very surprised because when you ask ChatGPT about something really obscure, it might give you good information or something bullshit and this seemed tightly reasoned.}

% \mgm{Everything here seems related to past sections (two of the quotes I had suggested as additions to prior sections lol). Might be worth discussing how to pitch this one as different. Like the effects of what the suggestion says and when / how it is raised depend on why the analyst considers the assistant helpful?}

\tableResults

\subsection{\emph{How}---Analyst or Assistant Initiative}
\label{sec:results_how}
% \mgm{defining initiative coßuld be helpful.}
% Finally, our interviews elicited comments about whether analysts preferred the assistant or themselves to initiate suggestions. 
Analysts espoused a variety of preferences about whether they wanted to initiate suggestions themselves or have the assistant do it for them. 
A few analysts [A4, A7, A9, A11] appreciated the assistant taking the initiative. For example, A11 liked that it \shortquote{proactively goes ahead and gives you suggestions.} 

Some analysts  [A2, A3, A4, A9] wanted the assistant to take even more initiative. A2, for instance, wanted the assistant to automatically run code given their current workflow: \longquote{[I would want the assistant to get...]  a sense of what my workflow is, has been, and is intended to be and pre-populate stuff for me. So if I normally run an OLS with varying degrees of variables, some included and some not included, generate a histogram for each. Do that for me.}

However, others felt that assistance would be more effective if it was delivered on demand.  
% \am{this repeats with that run visualizations for me from above}
Given the preference for both assistant and analyst-initiated assistance, 
multiple analysts [A6, A7, A9, A13] suggested that this could be a configuration option. 
% multiple analysts [A6, A7, A9, A13] suggested that this choice could be left for the analyst to control. 
To wit, A9 proposed: \longquote{Maybe two modes: lazy mode and (control) mode. If I am in lazy mode, you should already construct things and add them (to the notebook). If I want to take over everything, please be quiet here. If I want you, I'll call you.} This is akin to the two \textit{acceleration} and \textit{exploration} modes observed in prior work on AI-assisted programming~\cite{Barke2022GroundedCH}, indicating that planning suggestions might operate in a similar way as those of execution.

% \mgm{I like this section a lot! I'ts a bit sad it's last in teh who what where when why how ordering haha}



% \am{these two aren't about initiative per se their about expression modality}
Mediating these desires was the way in which the assistant was triggered.
For instance, analysts [A3, A8, A10] liked that the assistant responded to requests made in comments. 
% During the study, analysts naturally wrote comments down in their notebooks, which the assistant occasionally used as the context for suggestions. 
% Realizing this, some analysts continued requesting help in this way. A particularly illustrative example is when A8 typed \shortquote{assistant: how do I control for leagueCountry?} into a cell. Though our design primarily assumed assistant-initiated planning assistance, since some analysts showed a preference for their own initiative during the study, we treated analysts' comments as an initiative to elicit assistance.
% % enabled this behavior. \tim{what do we mean by enable?}
Some analysts wanted additional and different ways to directly ask the assistant for suggestions. A5, A6, and A7 wanted to ask the assistant for suggestions via a text prompt \`a la ChatGPT-style assistants.
% For example, A5 wondered if they \shortquote{could have typed something that says `plot discrete values scatter plot.'}  
Similarly, A11 wondered if the assistant could provide a list of relevant next steps via a keyboard shortcut.
% Designing an assistant to have a \am{various set} that can be adapted

This diversity of preferences suggests that having multiple ways to interact with the assistant that can be modified to taste and task is essential for effective assistant design. 
% , reminiscent of the functionality in Visual Studio Code \tim{did they mention this software specifically or is this functionality specific to that software (sounds surprising but I don't know)} where typing a keyboard shortcut on a specific part of the syntax yielded code auto-complete suggestions. 


==> 8-discussion-future-work.tex <==

\section{Discussion}
\label{sec:discussion}
In this work, we explored the potential of AI-based data analysis assistants that incorporate execution \textit{and} planning assistance.
 To identify the scope of suggestion content, we initially performed a \litreview review and a behavioral-driven analysis of independent analyses from a crowd-sourced analysis study (Sec. \ref{sec:suggestions}) to define categories of relevant suggestions (Table \ref{tab:suggestions}).
% To understand the space of helpful suggestion content, we perform a \litreview review and a behavior-driven study to establish a categorization of suggestion content. 
To explore the essential components of a helpful suggestion,  we conducted a \woz study to elicit the circumstances in which suggestions are helpful. 
% To explore the essential components of a helpful suggestion, we design and conduct a \woz study that is inspired by but not limited by the capabilities of existing LLM-based assistants. 
% This work contributes the first user study involving analysts working on a real dataset and task to better understand how to design and incorporate planning assistance into analysts' workflows. 
% In addition, we provide an open-source implementation of an assistant interface building on prior work. 
% We found that analysts saw many categories of planning assistance helpful, highlighting the potential of incorporating planning assistance. However, to achieve this, it is crucial to comprehend and address the contextual factors that influence analysts' willingness to consider planning suggestions. 

% Among these are aligning the analysis and the assistant on shared analysis goals and adding measures to reduce overreliance and promote trust in this new analyst-assistant paradigm. 
% \tim{what could we say here to be  more specific about engagement? promote trust but not overreliance? etc?}

We found that analysts had varying perspectives on what planning assistance was helpful. In some moments, planning assistance was about assistance for specific analysis steps; during others, it was about guidance for their overall workflow~(Sec. \ref{sec:results_what_assistance}). Some analysts found suggestions occasionally distracting, preferring to focus on their own analysis plan~(Sec. \ref{sec:results_when}). 
Similarly, we observed that there exists an inherent tension between the intended goals of the assistant and the goals of the analyst who might predominantly favor execution assistance, leading to divergent views on what constitutes ``helpfulness.''  Though analysts' goals are primary, assistants can play a crucial role in creating higher quality and more robust data analyses. Thus, supporting analysts with only execution assistance may not lead to such outcomes. Balancing analysts' perspectives of helpfulness and the assistant's impact on the workflow is crucial for providing truly valuable suggestions. Given that planning suggestions often require deeper consideration, a mutual understanding of their appropriate timing is also imperative. Developing affordances to enable analysts understanding and usage of such assistants is essential to those the design of those assistant. 
% An ``ideal'' assistant would completely understand the analyst's background, overall goals, and current plan (Fig.~\ref{fig:results}G and H) and reconcile this with its own goals (Fig.~\ref{fig:results}D). Further, the analyst should  understand the assistant's raison d'etre in addition to its capabilities. 
% Similarly, we found that while execution assistance offers time-saving advantages, it does not necessarily improve the robustness of analysis conclusions. Without well-reasoned planning considerations, execution assistance may focus on misguided directions resulting in wasteful efforts or misleading outcomes. 

% Beyond recommending analysts consider alternative decisions, data analysis assistants could prioritize helping analysts flesh out their analysis plan. Alternatively, assistants could only provide execution assistance in speeding up analysts' analysis plans. Or, the assistant could serve in a teaching role. 


Here, we synthesize these and other findings as design guidelines (Table~\ref{tab:design_implications}) to highlight design implications for future AI-based analysis assistants and reflect on limitations of our design. 


% In this work, we examined how to incorporate planning assistance into AI-based analysis assistants. To identify the scope of suggestion content, we performed a \litreview review and a behavioral-driven analysis of crowd-sourced analyses (Sec. \ref{sec:suggestions}) to define categories of relevant suggestions (Table \ref{tab:suggestions}). Next, we designed and conducted (Sec. \ref{sec:labstudy}) a \woz study to understand the circumstances in which suggestions are helpful. Here, we discuss takeaways from our study findings and design guidelines for creating helpful assistants (Table~\ref{tab:design_implications}).
% % First, we examine various ways of defining the goals of raising suggestions, and how that may impact the design of the assistant (Sec. \ref{sec:discussion_helpful}). We then explain why establishing common ground is critical to achieving these defined goals (Sec~\ref{sec:discussion_commonground}). Using the framework of common ground and integrating our observations from our study, we share design implications for building a data analysis assistant (Sec~\ref{sec:discussion_design_guidelines}). We conclude our discussion by reviewing study limitations (Sec.~\ref{sec:discussion_limitations}) and discussing avenues for future research (Sec~\ref{sec:discussion_future}).

% In this work, we examined how to incorporate planning assistance into AI-based analysis assistants. To identify the scope of suggestion content, we initially performed a \litreview review and a behavioral-driven analysis of independent analyses from a crowd-sourced analysis study (Sec. \ref{sec:suggestions}) to define categories of relevant suggestions (Table \ref{tab:suggestions}). Next, we conducted (Sec. \ref{sec:labstudy}) a \woz study to elicit the circumstances in which suggestions are helpful. Here, we discuss takeaways from our study findings and design guidelines for creating helpful assistants (Table~\ref{tab:design_implications}).


% This paper explores the potential of AI-based data analysis assistants that incorporate execution \textit{and} planning assistance. To understand the space of helpful suggestion we conducted a \woz study (Sec. \ref{sec:labstudy}), backed by a \litreview a behavioral-driven analysis of crowd-sourced analyses (Sec. \ref{sec:suggestions}). This work contributes the first user study involving analysts working on a real dataset and task to better understand how to design and incorporate planning assistance into analysts' workflows. 
% In addition, we provide an open-source implementation of an assistant interface building on prior work. 

 % Here, we discuss takeaways from our study findings and design guidelines for creating helpful assistants (Table~\ref{tab:design_implications}).

%  In this work, we examined how to incorporate planning assistance into AI-powered analysis assistants. To identify the scope of suggestion content, we initially performed a \litreview review and a behavioral-driven analysis of a crowd-sourced study's results (Sec. \ref{sec:suggestions}) to define categories of relevant suggestions (Table \ref{tab:suggestions}). Next, we designed (Sec. \ref{sec:woz_design}) and conducted (Sec. \ref{sec:labstudy}) a \woz study to elicit  the circumstances in which suggestions are helpful. Here, we discuss takeaways from our study findings and design guidelines for creating helpful assistants (Table~\ref{tab:design_implications}).
% We find that analysts found many categories of planning assistance helpful, highlighting the potential of incorporating planning assistance. However, in order to achieve this, it is crucial to comprehend and address the contextual factors that influence analysts' willingness to consider planning suggestions. We synthesize these findings to highlight design implications for future AI-based analysis assistants. Among these are aligning the analysis and the assistant on shared analysis goals and adding measures to reduce overreliance and promote trust 
% % \tim{what could we say here to be  more specific about engagement? promote trust but not overreliance? etc?}
% in this new analyst-assistant paradigm. 





% \subsection{Analyst Perspectives on Planning Assistance}
% \label{sec:discussion_helpful}

% To define what categories of suggestions content may be helpful, we created a categorization of suggestion content as shown in Table~\ref{tab:suggestions}. In our subsequent \woz study, we found both execution and planning suggestions were considered helpful (Sec. \ref{sec:results_what_assistance}). We provided analysts a thumbs up and down button (Fig. \ref{fig:interface}F) such that they can apply their own definition of helpfulness towards each suggestion. However, while execution assistance was almost always considered beneficial, analysts' reception of planning assistance was more varied.

% Contextual factors which we described in Section~\ref{sec:results}, were often referenced as reasons for why planning suggestions were preferred.

% In our study, we noticed the same planning suggestion content (e.g., interpreting the outputs of a linear model) was received differently depending on contextual factors (Sec.~\ref{sec:results}).

% As opposed to analysis execution, in which the focus is to write code to execute the current analysis step, analysis planning can be much more varied and personalized depending on the analyst's background (Sec. \ref{sec:results_who}) and analysis progress (Sec.~\ref{sec:results_when}). Within analysis planning, there are also different levels of abstraction. For example, analysts may make broader planning decisions about the choice of the statistical model, or after choosing the statistical model, make fine-grained choices of model regularization parameters. 





% Further, the perceived "unhelpfulness" of some planning suggestions was often due to \textit{when} these suggestions were presented~(Sec.~\ref{sec:results_when}). When engrossed in a particular analytical task, analysts were often resistant to diverting their focus toward distracting suggestions. 
% From a cost-benefit perspective \cite{vasconcelos2023explanations}, execution assistance is less intrusive, with its time-saving benefits more easily recognizable. Conversely, planning assistance demands more mental effort as analysts evaluate multiple analytical paths, underlying rationales, and the alignment with their prevailing strategies. 
% % \tim{and in addition implementing these plans likely would come with additional cost, right?}\ken{yes but this can be reduced through exec assistance. The ones mentioned so far are I think the most central at being costly} 
% This not only complicates the assessment of the utility of planning assistance but amplifies the drawbacks of sub-optimal suggestions.



% \subsection{Balancing Planning and Execution Assistance}
% \label{sec:discussion_balance}
% Unsurprisingly, analysis execution takes lots of time and this is what execution assistance tools focus on. For planning assistance, the stakes are understandably higher. Planning assistance is more intrusive on the analyst's workflow as analysts must consider multiple possible analysis decisions, rationales behind these decisions, and where the suggestion fits into their overall analysis plan. This increases the negative impacts when suggestions are not helpful.

% Though execution assistance offers time-saving advantages, it does not necessarily improve the robustness of analysis conclusions. Without well-reasoned planning considerations, execution assistance may focus on misguided directions resulting in wasteful efforts or misleading outcomes. 

% % Beyond recommending analysts consider alternative decisions, data analysis assistants could prioritize helping analysts flesh out their analysis plan. Alternatively, assistants could only provide execution assistance in speeding up analysts' analysis plans. Or, the assistant could serve in a teaching role. 

% There exists an inherent tension between the intended goals of the assistant and the goals of the analyst who might predominantly favor execution assistance, leading to divergent views on what constitutes ``helpfulness.''  Though analysts' goals are primary, assistants can play a crucial role in creating higher quality and more robust data analyses. Therefore, supporting analysts with only execution assistance may not lead to such outcomes. Striking a balance between understanding analysts' perspectives of helpfulness and the assistant's impact on the workflow is crucial for providing truly valuable suggestions. Given that planning suggestions often require deeper consideration, a mutual understanding of their appropriate timing is also imperative. An ``ideal'' assistant would completely understand the analyst's background, overall goals, and current plan (Fig.~\ref{fig:results}G and H) and reconcile this with its own goals (Fig.~\ref{fig:results}D). Further, the analyst should also understand the assistant's raison d'etre in addition to its capabilities. 

% To summarize, the assistant's goals (Fig.~\ref{fig:results}C) should take into account the analyst's goals (Fig.~\ref{fig:results}G) in the context of its own design and functionality (Fig.~\ref{fig:results}D). Likewise, the analyst's perception of the assistant (Fig.~\ref{fig:results}F) should take into account their goals for analysis (Fig.~\ref{fig:results}G) and how the assistant can meet them (Fig.~\ref{fig:results}D). This common understanding is the basis from which truly helpful assistance can be provided and perceived. 


% Therefore, to surface helpful suggestions, ideally, the assistant will strike a balance between understanding and acting upon the analyst's view of what is helpful and the assistant's objective of its impact on the analyst's workflow.

% For example, if the assistant's goal is to broaden the analysts' understanding of the analysis decision space, then it might prefer offering planning assistance over execution assistance despite analysts' affinity towards execution assistance. Therefore, to surface helpful suggestions, ideally, the assistant will strike a balance between understanding and acting upon the analyst's view of what is helpful and the assistant's objective of its impact on the analyst's workflow.

% \tim{in the paragraphs above we should say more clearly that analyst and assistant have goals. While analysts goals are primary, assistant goals, even those in potential tension with analysts, might be important. I see our planning assistance towards higher quality / more robust data analysis as such a goal. of course these need to be reconciled but the point is that an assistant  only serving the analyst what they want on their initiative may not lead to important outcomes that we are after. }

%%%%%%%%%%%%%%%%%%%%
% We defined a lot of helpful suggestions via literature review. Included both execution (previously done) and planning (relatively new) in our study. Found overall in our study that most people found planning and execution helpful. 


% We did the goal of being open to new workflows, focused on the content they put into the jupyter notebook. However, because of the variety in analysis perspective,  This happened even wiht a defined AI designer perspective, and that could change depending on the context. 


% We define this ``helpfulness'' very loosely on purpose, because it may vary. 

% Varies along analysts perspective
% - sometimes want lazy assistance
% - sometimes wants to open new workflows
% - sometimes wants speed
% - sometimes a combination
% - level of abstraction they're looking for
% - sometimes changes along analysts (they discussed wanting toggles and stuff)
% - What is the end goal? even with same data set (and sometimes same question too), could be different approaches or levels of rigor or where they feel lost.


% Also varies along AI designer's perspective. In our study, we focused on getting anlaysts to consider new workflows
% - Is it to help along with current analysis path with small misses?
% - Is it to just help the analyst on whatever they want to do?
% - Is it to challenge the analyst and get towards some specific goal? 
% - is it to update analysts beliefs only or also their actions?


% To surface helpful suggestions, ideally, assistant will find a balance between understanding and acting upon analyst's view of what is helpful and it's objective of how much to challenge with vs smoothly support the analyst's workflow.


% \subsection{The Importance of Common Ground}
% \label{sec:discussion_commonground}

% To create the alignment necessary for helpful suggestions, it is critical to establish common ground. Common ground is the shared understanding between two participants in a dialogue or interaction. In psychology, “two people’s common ground is, in effect, the sum of their mutual, common, or joint knowledge, beliefs, and suppositions”~\cite{clark1996using}. With people, this common ground is established through many means, including a contextual understanding of the setting of interaction, shared cultural knowledge, shared experiences, and social and transactional dialogue~\cite{clark2019makes}. 

% Computer science research also notes the importance of establishing common ground through dialogue between an agent and a person. For example, when communicating with a robot, prior work has emphasized having a shared understanding of the world and communicating internal representations from the robot to the user~\cite{chai2014collaborative,chai2016collaborative}. In conversational models, common ground is a crucial component of effective communication and personalization to the context and person of that interaction~\cite{clark2019makes,kopp2021revisiting}. 

%  We find that common ground between the analyst and the assistant is also important for AI-powered planning and execution assistance. In this application, common ground refers to understanding the analyst's and the assistant's analysis goals, the assistant's capabilities, the analyst's analysis process, and the analyst's domain, statistical, and AI backgrounds. In our study, we observed analysts often found suggestions unhelpful when the content and timing of the suggestion did not align with the analyst's background and current focus. Throughout the analysis process, an ideal assistant would completely understand the analyst's background, overall goals, and current plan (Fig.~\ref{fig:results}G and H) and reconcile that with the assistant's own goals (Fig.~\ref{fig:results}D). On the other hand, the analyst should also understand the assistant's goals in addition to the assistant's capabilities. 

% To summarize, the assistant's perception of the analyst (Fig.~\ref{fig:results}C) should be matched with the analyst's goals (Fig.~\ref{fig:results}G) while considering the assistant's own goals (Fig.~\ref{fig:results}D). Likewise, the analyst's perception of the assistant (Fig.~\ref{fig:results}F) should match the analyst's goals for the analysis (Fig.~\ref{fig:results}G) while also considering the assistant's goals (Fig.~\ref{fig:results}D). This common understanding is the basis from which helpful assistance can be provided and perceived. 

% \tim{or vice versa?}

% \subsection{Creating common ground between analyst and agent}
% \label{sec:discussion_initiative}
% \
% The analyst and assistant need to establish common ground in the beginning about the analyst's background, needs and goals. They then should continue creating common ground about the analyst's updating plan throughout the analysis process. Unfortunately, a perfect level of common understanding is unrealistic, as the methods of communication are just the assistant's suggestions, the notebook contents, and the agent's initiative. In our study, as described in Section~\ref{sec:results_how}, the analyst's initiative to interact with the agent is just the content they type into the notebook, and we briefed them on this method of interaction in the beginning of the study. Throughout the study, users continued to try different ways of interacting and typing commands to see the impacts of their actions. In follow interviews, users were especially interested in how to expand this ability to establish their own initiative (e.g. \mgm{TODO: direct query, specifying when to get results, wishes for less initiative and more initiative of the agent,}). Methods for creating this common ground on the ever-changing and variable task of data analysis is an interesting path for future work that we discuss in more detail in Section~\ref{sec:discussion_future}.

% Furthermore, at the moment our assistant does not explicitly request any information from the user (e.g. their goal, statistical background, etc). Our assistant also does not provide any intro specifically to build up basics first so person has understanding of what the tool can do. More explicit definition of these aspects may be helpful in establishing common ground. 


% \subsection{Updating common ground over time}
% \label{sec:discussion_when}

% An incredibly important factor was the time the suggestion was raised in relation to the workflow, as described in Section~\ref{sec:results_when}. The users' needs are different in the beginning, middle, and end of the analysis process \mgm{TODO: cite?}, and often go in iterative refinement loops. If the suggestion raised is too different from the analyst's perspective of their current needs, they will ignore, get distracted, or put a pin in it for later. If the suggestion is completely in line with their current practices, execution help may help it become faster, but the assistant's helpfulness for planning is limited. 

% The time at which suggestions are raised seems critically important from our user study, but this phenomenon can be much more rigorously studied. We discuss these potential avenues for future work in Section~\ref{sec:discussion_future.} \mgm{Right now not very in detail in the future work section. I think either flesh out more details, or bring up future work here so doesn't need to stand alone as much}

%%% Not sure if to include or not:
% Additionally, what the assistant surfaces in the beginning impacts the analyst's perspective of the assistant over time. 
%  possibly include here how it relates to how llms like to just do sequencing and stuff? 

\subsection{Design Guidelines}
\label{sec:discussion_design_guidelines}
Based on our results and discussion, we highlight seven design guidelines that extend Human-AI Interaction guidelines \cite{Amershi2019GuidelinesFH} for designing a data analysis assistant.

\subsubsection{Assistants should communicate with the analyst to align on analysis goals}
% The old  Creating common ground between analyst and agent could probably fit in here.
\label{sec:discussion_design_implications_match_goals}


% In this paragraph talk about how it should be on the agent to establish it? Or maybe in the parapgrah on how to establish

During the analysis portion of our study, the wizard was occasionally misaligned with the analyst's goals (Sec.~\ref{sec:results_when}). Likewise, analysts spent time figuring out the assistant's goals (Sec.~\ref{sec:results_who_curiosity}).
% \tim{it stands out to me that this is the "opposite direction"} 
% A few curious analysts typed comments seeking suggestions from the assistant and were curious about the assistant's resulting suggestions to understand the assistant (Sec.~\ref{sec:results_who_curiosity}).
% For example, participants noted if the assistant gave information similar to queries they had typed in comment boxes [A3, A8, A10]~\mgm{include A-X descriptions here if it's included in results section?}, and noted when the assistant did not respond to other kinds of artifacts in the notebook, such as error messages [A5, A13]. \ken{i usually just refer to results section but we can see what others think. Also I think this discussion was more about capabilities then goals.}
% Moreover, analysts in our study wanted more agency (e.g. directly prompting, choosing from a list of options, and specifying when they wanted to receive inputs) to direct the assistant toward their goals (Sec.~\ref{sec:results_how}).
Therefore, the analyst and assistant should establish shared goals at the beginning of the analysis, and this understanding should evolve over time. During its introduction, the assistant can describe its objectives for improving the analysis quality, highlight the value of planning assistance, and warn against the pitfalls of prioritizing execution assistance only. Furthermore, the assistant can communicate this information through interactive model cards~\cite{Crisan2022InteractiveMC}. Although prior work on conversational agents has found users prioritize their goals and needs over the assistant~\cite{clark2019makes}, we posit that it remains vital to consider both parties in the interest of quality analytical results. 
% In the context of data analysis, 
Adhering only to analysts' execution preferences may perpetuate poor analysis decisions and practices, leading to misguided inferences or biased results~\cite{mcnutt2020surfacing}. 
% ~(Sec.~\ref{sec:discussion_balance})
% Thus, it is necessary for an assistant to communicate clearly the goals of planning assistance to the analyst. Then, the analyst and assistant can coordinate the optimal collaboration. 
Understanding the best ways to establish, integrate, and uphold shared goals over time is an important area for future exploration.


% \tim{this is great, just make this a bit more clear above or argue for why it should only be in one section?}


\subsubsection{Assistants should provide suggestion content suited to the analyst's background}
\label{sec:discussion_design_implications_match_bg}

% different people had different prior knowledge, preffered one staistical approach over the other, had different levels of understanding, coding expertise etc. 
Analysts differ in their statistical, domain, and coding backgrounds. 
We observed that the same suggestion considered helpful by some participants, could be found by others to be too elementary, too distracting, too far from their expertise (making correctness auditing difficult), or too different from their usual analysis or coding practices to be useful~(Sec.~\ref{sec:results_who}). 
% We observed that these differences affected their analysis plan and reactions to suggestions~(Sec.~\ref{sec:results_who}). The same suggestion considered helpful by some participants, could be found by others to be too elementary, too distracting, too distinct from their expertise (making testing its validity was prohibitively difficult), or too different from their usual analysis or coding practices to be useful (Sec. \ref{sec:results_who_expertise}). 
% Thus, assistants should match suggestion content to the analyst's background.
In situations when a suggestion is too difficult or different to comprehend, the assistant should provide options to explain further or offer additional resources---e.g., links to relevant documentation and tutorials. Likewise, the assistant could suggest  more approachable alternatives on demand. 
% These additional explanations or approaches could be visible through a show/hide toggle.
% \tim{just a comment: I like allowing the user to expand/contract details rather than trying  to have the assistant always get it right. just allow them to hide or ask for more explanation. }
 % Prior work on conversational agents found many users thought the system should take on the burden of establishing common ground to personalize outputs~\cite{clark2019makes}\mgm{This seems to be an interesting point but I'm not quite sure where to put it.}. 
In our study, the assistant did not gather any information on task or background from the analyst. A more explicit definition of the analyst's expertise, such as through analyst initiative (Fig. \ref{fig:results}A), may help establish common ground.
For instance, on first-usage analysts could have a quick conversation with chatbot to elicit their educational background, coding competency, and typical workflows (akin to how we asked participants about their preferred environments before the study). 
% For instance, analysts could configure their backgrounds by providing a short bio 
% \tim{do we really think a bio would be the right thing to use?  more specific questions seem more targeted and more likely to succeed?} 
% or a completed template describing their educational background, a self-rating of their coding expertise, typical workflows, and preferences for analysis methods and software packages. 
The assistant could then use this as relevant context to customize LLM-based assistant suggestions \cite{Andreas2022LanguageMA, Kirk2023PersonalisationWB}. 

% different levels of explanation for different audiences
\subsubsection{Assistants should match the analyst's preferred level of planning assistance abstraction.}
\label{sec:discussion_design_implications_match_abstraction}

There are multiple perspectives on what consitutes helpful planning assistance. These can range from guiding hyper-parameter selections to providing a comprehensive plan with multiple analysis steps.
Future assistants should account for analysts' preferences regarding desired levels of planning assistance and how these preferences may change throughout the analysis process.
% The assistant could learn analysts' preferences by observing their behavior across multiple analyses and within single analysis, goals may different between sessions. 
% More simply, this could be communicated explicitly by the analyst in the UI. 
% For instance, analysts may want to iteratively refine their intent for assistance such as in \textit{Wrex}, a non-LLM-based notebook extension that generates code through programming by example \cite{Drosos2020WrexAU}.
For instance, the assistant could offer explicit modal dials to guide suggestion content---such as an ``\textit{execution}'' mode that focuses on code execution, a ``\textit{think}'' mode for specific planning suggestions, a ``\textit{reflection}'' mode for connecting decisions and highlighting potential missed steps, and an ``\textit{exploration}'' mode for higher-level planning suggestions.
% ---although such a partitioning would need to be designed to be in accord with the interleaved and iterated structure of data analysis.
Likewise, the level of planning abstraction also relates closely to the scope of the analysis code that the assistance affects. An analytical decision could be one parameter, line, function, code block, or even multiple chunks of code \cite{Liu2020BobaAA}. Suggestions that impact large parts of the analyst's analysis require more willingness from the analyst to consider and adopt. 
Both sets of levels could be configured from the UI or learned through observation of the users across analyses.
% and within single analysis.
% Thus, future assistants should consider the scope of analysis that a suggestion influences.
% \tim{I wonder whether it's "dangerous" to only consider planning as/in exploration. If the analyst makes mistakes or misses key things wouldn't they likely want to know, even if they weren't currently  in exploration mode?}\ken{tried to add reflection mode to hint at this}
% ikewise, there could be a "exploration" mode for when the analyst needs more consideration of planning focused suggestions while coordinating these with their current analysis. 


% \ken{any works similar to this with different modes for abstraction to cite} \tim{maybe check in w Jeff directly}. 

% At a finer scale, since analysts' needs may differ between analyses, the assistant should also learn analysts' goals and behavior for the current analysis. 
% Recent work \cite{Park2023GenerativeAI} in the context of simulating human behavior in AI agents leverages ChatGPT to store experiences in memory and dynamically retrieve relevant background to inform agent behavior. Data analysis assistants could utilize a similar framework to store analyst background and actions and use the appropriate information to determine the appropriate level of planning assistance  to provide at different moments in the analysis. Future research could explore how LLMs can support this framework and identify characteristic behaviors of analysts engaged in execution and planning.
% However, this is no easy task. This was partially what the wizard was trying to do in our study and was difficult even with additional inputs from analysts' screens and audio. Future work could explore the extent to which LLMs can support this and what sorts of behaviors are characteristic of analysts engaging in analysis execution and planning

% \am{would like to grind this upwards}


\subsubsection{Assistants should time suggestions based on the analyst's openness to considering alternative approaches.}
\label{sec:discussion_design_implications_timing}

Analysts  in our study felt that some suggestions were good but were not well-timed based on their current task~(Sec. \ref{sec:results_when}). 
When analysts are focused on executing a specific analysis decision or plan, they may prefer execution rather than planning suggestions. Conversely, when they are considering their next steps, they may be more open to guidance for analysis planning.
% Therefore, assistants should strive to recognize when analysts are open to planning assistance. 
Analysts could explicitly communicate their timing preferences to the assistant or use a ``remind me later'' response to raised suggestions. Additionally, organizing and tagging suggestions could help them easily find and revisit suggestions.
% even if their timing were not ideal. 
 Meanwhile, the assistant could also learn appropriate timing from analysts' behaviors. For instance, prior works have used probalistic utility modeling~\cite{Horvitz1999PrinciplesOM} and sensors to model and predict human interruptibility~\cite{Fogarty2005PredictingHI}. 
 % The assistant could also follow a utility model for mixed-initiative AI intervention by considering the expected utility of different actions~\cite{Horvitz1999PrinciplesOM}. 
We note that this may be challenging if analysts fixate on rigid analysis plans and highlight the importance of establishing shared goals between the analyst and assistant (Sec. \ref{sec:discussion_design_implications_match_goals}). 
% While many analysts may prefer planning assistance, others may not. Given this tension and difficulty, considerations for the timing of suggestions may also benefit from the recommendations of \textit{polite computing}~\cite{Whitworth2005PoliteC}.
% \tim{the last sentence speaks to the question: Is there ever a good time to engage the analyst on planning assistance. It sounds  like while this is the case for many, it isn't for some and that's an inherent tension. perhaps clarify that slightly here.}

\subsubsection{Assistants should provide multiple ways to request content at different levels of abstraction.}
\label{sec:discussion_design_implications_initiative}

We observed diverse opinions (Sec.~\ref{sec:results_what_assistance}) about assistant-versus-analyst initiative and levels of planning assistance, a heterogeneity which might be met by supporting multiple means of requesting assistance.
% Though preferring assistant-initiated suggestions, analysts also wanted to exert their own initiative in requesting suggestions (Sec.~\ref{sec:results_how}). 
% \jeff{I'm a bit thrown off by this, as I thought we said earlier that participants liked having suggestions initiated by the system} 
% Further, they showed different preferences for the level of planning assistance (Sec.~\ref{sec:results_what_assistance}). Desires which would be supported by support multiple means of requesting assistance.
% Therefore, assistants should provide analysts with multiple ways to request assistance for different levels of abstraction. 
% In terms of design, there is flexibility in the input mechanism and initiative. For example, analysts could write comments, select text, trigger suggestions via a hotkey, request proactive suggestions in a side panel, etc. Each could carry implicit context regarding the level of feedback they desire \cite{McNutt2023OnTD}. Ambient and textual interfaces (i.e., assistant follows the cursor and can be invoked via an action) suggest localized context and help. For example, a common workflow with execution assistants such as Github Copilot has the programmer write comments that detail what the lines of code should be to complete the task \cite{Vaithilingam2022ExpectationVE}. Meanwhile, a side-panel interface with controls outside the immediate notebook suggests global context and assistance. 
While existing systems usually offer one form of invocation, LLM-based analysis assistants should allow and interleave multiple forms of invocation and context for different levels of assistance. It is also essential to clarify the context for the LLM in each form of interaction. For example, a hotkey trigger at the line level could indicate a focus on execution assistance using only the current cell. On the other hand, analysts could specify broader suggestions when requesting feedback in the side panel and choose the LLM context by selecting relevant cells. 
Interactive visualizations could also be employed to show and help analysts make decisions and consider alternative choices \cite{Liu2019PathsEP, Liu2020BobaAA}. These visualizations (e.g., Fig~\ref{fig:teaser}), tied to the analysis code, could help analysts review their steps and select areas where additional assistance is needed.


\subsubsection{Assistants should mitigate suggestion overreliance by promoting engagement and critical thinking.}
\label{sec:discussion_design_implications_trust}

% Results relations
    % Errors exist -- and this is a known problem
% LLMs are adaptable and powerful, but they can have erroneous outputs~\cite{Amershi2019GuidelinesFH,bender2021dangers}. 
% As data analysis often informs high-stakes decisions~\cite{Baker20161500SL, Cockburn2020ThreatsOA, Aarts2015EstimatingTR}, it is critical for analysts to be aware of the \am{wc}decisions and rationales that comprise their analysis even as the assistant makes seemingly sensible recommendations---particularly given LLM's hallucinatory tendencies~\cite{Amershi2019GuidelinesFH,bender2021dangers}. 
As data analysis often informs high-stakes real-world decisions~\cite{Baker20161500SL, Cockburn2020ThreatsOA, Aarts2015EstimatingTR}, it is essential that analysts be able to understand and think critically about their analyses, regardless whether they received execution or planning assistance.
% Likewise, different individuals' trust in automation can impact their response to erroneous outputs~\cite{lee2004trust,zhang2020effect}. 
% skepticism towards the suggestion quality and 
In our study, analysts showed varying levels of  thoroughness in validating the model's decisions, code, and outputs (Sec.~\ref{sec:results_who_curiosity})---sometimes critically disengaging and going on \shortquote{autopilot}. 
% % For example, A4 caught an error in which a ChatGPT-generated suggestion described a p-value of $0.15$ as significant. 
%     % Varying trust levels and understanding of LLMs
% For instance, A8 \shortquote{acted on autopilot} over-relying on the assistant's suggestions without critical engagement (Sec.~\ref{sec:results_why}), while A4 caught an incorrect LLM-based suggestion that p-value of 0.15 is significant.
% Gordon et al. \cite{gordon2023co} sketch the growing area of tools for auditing AI generate code output. 
% Therefore, assistants should reduce overreliance by introducing mechanisms to promote engagement and critical thinking with their suggestions.
% One way to increase engagement is to provide explanations that make it easier to understand and verify the assistant's suggestions~\cite{vasconcelos2023explanations}. 
 Over-reliance on AI is well documented in other scenarios ~\cite{buccinca2021trust,bussone2015role,vasconcelos2023explanations,yin2019understanding}, and developing mechanisms for skepticism is a growing concern~\cite{gordon2023co}.
% We might 
Designing assistants with critical affordances is essential to preventing them becoming AI-mediated p-hacking machines. 
% Embracing some of these approaches is of critical importance \am{to making our assitant a good boy}
One approach might be to reduce the cognitive effort of engaging with suggestions~\cite{vasconcelos2023explanations}, freeing analysts to be more scrutinous.
% may be less prone to accept the assistant's recommendation without scrutiny~\cite{vasconcelos2023explanations}. 
% \tim{I wonder whether that's always true. You could reduce cognitive effect with an 1click "accept and implement" but this could of course backfire. is it perhaps not only about cost/effort? your next paragraph suggests that as well}\ken{just talking about explanations and not about adopting the suggestions -- changed from "are" to "may be"} 
For example, the system could present a visualization mapping the overall decision paths (\`{a} la Fig.~\ref{fig:teaser})  to demonstrate how a given recommendation would influence the overall analysis.
% The visualization could highlight decisions that would be affected or illustrate alterations in the decision paths. 
% Similarly, the assistant can reduce the cost of contemplating their decisions and invite critical thinking by providing a series of reflective questions~\cite{Wood2019DesignEW}. \tim{is that really reducing cost? or increasing it if we ask more? it might depend on what we view as the alternative/counterfactual. it's more work compared to not doing anything or simply accepting it. but it's less cost relative to having to think through all of this carefully without helpful scaffolding. I think readers could get confused here.} 
% Additionally, incorporating multiple explanation methods could improve comprehension among analysts, a design guideline we further elaborate on in Sec.~\ref{sec:discussion_design_implications_explanation}.
% Besides simplifying the process of understanding the assistant's suggestions, 
Similarly, assistants could introduce cognitive forcing functions~\cite{buccinca2021trust} to increase the cost of relying on the assistant. For example, the assistant could require a  scaffold of the analysis plan before providing suggestions or by requiring that code be typed out manually rather than automatically inserted. 
Forced low-level participation may prompt better engagement with the assistant---although it is crucial to ensure that these interventions do not deter analysts from utilizing assistance altogether.
% By requiring analysts to participate on a low-level that may become more engaged with the assistant.
% In doing so, analysts may become more engaged with the suggestion.
% Other measures might include making it more challenging to adopt a suggestion, such as by omitting a direct code copy-paste option, or offering only pseudocode or a code template. 
% Presenting multiple suggestion options could also compel analysts to make the final decision independently.
% However, it is essential to strike a balance. 
% However, while such engagement is important, it is  crucial to ensure that these interventions do not deter analysts from utilizing assistance altogether.
% ---although cultivating critical thinking remains challenging~\cite{Aliakbari2013TeachersPO, Zhang2022TheRO, Yuan2020StudentTP, Saleh2019CRITICALTA}.
% , as underscored by a wealth of pedagogical research~\cite{Aliakbari2013TeachersPO, Zhang2022TheRO, Yuan2020StudentTP, Saleh2019CRITICALTA}.


% As discussed in Section~\ref{sec:results_who_curiosity}, analysts expressed varying levels of skepticism towards the suggestion quality and thoroughness in validating the model's decisions, code, and outputs. For example, A8 acted on ``autopilot'' by relying on suggestions without critical engagement.

% \mgm{I think the above paragraph still makes the most sense for critical engagement place??}

% % Calibrated trust is X. One commonly studied and more measurable impact of miscalibrated trust is overreliance. Past work looks at these issues, and they come ito play here
%  In response to errors in Machine Learning models, prior work stresses the importance of creating calibrated trust. Calibrated trust aligns the human's belief in the model's capabilities with the model's capabilities~\cite{bansal2021does,zhang2020effect,tomsett2020rapid}. Trust is multifaceted and can include not only trust in the AI system itself, but also an innate propensity to trust~\cite{zhang2020effect,kunkel2019trust,yu2019trust,pop2015individual}, cultural differences~\cite{kunkel2019trust,yu2019trust,pop2015individual}, as well as social and organizational contexts~\cite{pop2015individual,jacobs2021designing}. Although it is not possible to quantify and measure trust directly, one often studied measurable impact of poorly calibrated trust is overreliance: a phenomenon in which people accept an AI's incorrect prediction ~\cite{buccinca2021trust,bussone2015role,vasconcelos2023explanations,yin2019understanding}. 
%  \mgm{This is feeling not as relevant to the explanations section now that I look at it -- considering just getting rid of it for now?}

% % Why is this a potential issue that needs to be designed for. Danger to make things worse if not calibrated
% Given the possibility of errors in LLM outputs and the varying trust levels of analysts, future systems should design for calibrated trust to minimize the incorporation of faulty suggestions. Our provided suggestions often included explanations, although it is important to note that the effectiveness of explanations in reducing overreliance and calibrating trust is an open field of research~\cite{bansal2021does,buccinca2021trust,eiband2019impact,vasconcelos2023explanations}. 
% % Design should go for calibrated trust. many prior works on how to do this. Some things to consider in analysis are X, y, and z
% Several analysts responded positively to these explanations, as detailed in Section~\ref{sec:results_what_qualities}. There are also numerous other design options beyond explanation for calibrating trust. Analysts can be encouraged to engage critically with AI suggestions through cognitive forcing functions~\cite{buccinca2021trust}. Displaying a measure of the models' confidence in its suggestions could encourage calibrated trust, although the effects of showing confidence scores vary across prior works~\cite{lai2019human,yu2019trust,zhang2020effect, pop2015individual}. Finally, hard-coded sanity checks on LLM outputs, such as extracting p-scores and comparing them directly to the user's definition of significance, could calibrate trust by reducing the amount of incorrect information returned by the assistant.
% \mgm{Seems like most of this should also be removed? Or cognitive forcing functions can be mentioned with some of the critical engagement stuff, and we want to get rid of confidence scores stuff. I moved up some stuff about how explanations are still an open field of research}

% \mgm{I removed stuff from the final paragraph to go up to explanation section though. Except the following sentence that is more engagement i think}
% For example, instead of using previously studied cognitive forcing functions~\cite{buccinca2021trust}, a study could compare the impact of an assistant giving multiple diverging paths forward with an assistant consistently pushing towards an incorrect analysis path.

% The goal is for people to critixally engage with their own analysis process
% We do that through suggerstions
% But, danger of overcorrecting (not a great word -- sounds like now they're thinking too critically), which we saw sometimes, where you go on autopilot with suggestoins
% LLMs can have errors, that autopilot could be dangerous
% Need to reduce the amount of overreliance, which we encourage to do throug critical engagement
% That is hard, but there are some suggestions from prior work


% Get rid of confidence scores

% Ways to make people critically engaged
% Force them to write out an outline before starting
    % have to think through planning process on your own before assistant tells you the answer
    % The assistant throughout the process suggestsion deviations and ways of doing the plan better
    % Ken look sinto prior work
% (maybe) purposefully put in bad information and suggestions so people trust it less??
% Lower the barrier to understanding how decisions affect future options? Or make explanations/content easier to engage with?
% Can't copy-paste code
% Give multiple options so people have to choose & tradeoffs of each
% extra step to access code? make analysis planning ver obvious
% visualie analysis spce and highlight parts that are missing

\subsubsection{Assistants should adopt multiple explanation methods for increased understanding and trust.}
\label{sec:discussion_design_implications_explanation}
Analysts highly valued suggestion explanations, as they helped them better understand and trust the assistant's suggestions (Sec.~\ref{sec:results_what_qualities}). 
% In our study, code, code comments, and natural language suggestion rationales all contributed to explaining suggestions. 
Explanations provided both rationale for why an analysis decision should be considered and definitions of potentially unfamiliar concepts. 
Future assistants should incorporate multiple forms of explanations, that are sensitive to  analysts' backgrounds and preferences. To avoid introducing excessive cognitive load~\cite{vasconcelos2023explanations}, assistants could allow analysts to select their preferred types of explanation. 
Alternative explanation mediums, like visualizations or animations~\cite{Pu2021DatamationsAE, Xiong2022VisualizingTS}, could better contextualize suggestions.
% other potential methods to present suggestion explanations. For example, visualizations or animations of the data during and after data transformations could help analysts understand the assistant's code actions~\cite{Pu2021DatamationsAE, Xiong2022VisualizingTS}. 
% Recent work~\cite{Dibia2023LIDAAT, Lin2022TeachingMT, Liu2023GEvalNE} has demonstrated that LLMs, like GPT-4, can assess the quality of their output, approaching human-level judgment for tasks such as summarization and visualization.
% which might be useful for constructining explanations.
% \tim{that's a pretty strong claim? I didn't look at these papers but I imagine they couldn't always do that. otherwise they wouldn't need people anymore :) I think we should probably make this softer of more nuanced.}
As LLMs continue to improve, assistants could also provide model-generated critiques of their own suggestions~\cite{Dibia2023LIDAAT, Lin2022TeachingMT, Liu2023GEvalNE}.
% as an initial pass at explaining the strengths and limitations of an approach. 
% Nevertheless, 
Identifying explanation best practices remains an open area of research~\cite{bansal2021does,buccinca2021trust,eiband2019impact,vasconcelos2023explanations}. 
% Future work could explore the effects of different explanation types in the context of a data analysis task. 
Unlike many other tasks however, there are often multiple reasonable paths in data analysis~\cite{Liu2019PathsEP} without an objectively ``correct'' answer or other measures besides accuracy---making evaluation of explanations especially troublesome.
% ---such as alternative paths considered, analysis quality (though this is difficult to evaluate), or analysts' perceptions and actions---could help assess different explanation designs. 
% Although this lack of an objective ``correct'' answer deviates from prior work, it may also open to the door to interesting new analyses.  
% Furthermore, future studies can still measure the impact of explanation design on analyst perceptions and actions. 
% For example, a study could present incorrect suggestions and measure if analysts notice the errors under different explanation conditions.
% Future work could also apply similar methods to judge the effectiveness of the assistant intervention through the quality of the final analysis outputs, or by creating experimental conditions in which the incoming dataset has flaws and seeing if analysts perform measures to address those flaws.

% \tim{I don't like when limitations is the very last part of the paper. so much good work to end on a concentrated note of all the potential issues. I think I'd either prefer a very short conclusion back or having some kind of other last subsection here.}

\subsection{Limitations and Future Work}
\label{sec:discussion_limitations}
This work has several limitations, relating to our participants, our study design, and our analysis of the results. 

% \am{unhappy with this paragraph}
First, we selected analysts who self-identified as having a high proficiency in statistical analysis. As we wanted to understand the mechanisms surrounding planning assistance, we determined that analysts with sufficient programming and statistical knowledge would be more engaged with analysis planning and our assistant's suggestions; we found that even they were often unaware of the decisions and rationales our assistant offered. 
% As such analysts are often the ones performing analyses that influence real-world decisions, understanding planning assistance with this audience is paramount. 
Analysts with less statistical and programming expertise may have different experiences and preferences when working with an analysis assistant. Future work should explore how this style of assistance can be support for novice data analysts.
In addition, we focused on people willing to participate and perform data analysis with an AI assistant, which may positively bias our results.
% This may affect analysts' willingness to work with an assistant and eagerness to probe the assistant's capabilities. 

Next, to facilitate a lab study of reasonable duration, we chose to conduct a same-day, in-person study of two hours. 
% If analysts had more time with the assistant, say weeks, they may have calibrated their expectations for the behaviors of the assistant and developed a better sense of when to rely or not to rely on it. Likewise, analysts may have developed a better sense of the assistant's timing and goals, as well as overcome any potential novelty effects latent to our one-shot design.
If analysts had more time with the assistant, say weeks, they may have calibrated their expectations for the behaviors of the assistant, developed a better sense of the assistant's timing and goals, and overcome any potential novelty effects latent to our one-shot design.
In future work we intend to explore these issues by developing a tool that supports this style of longitudinal usage.
% , which can be realistic in certain scenarios,
Similarly, while our lab-based \woz study design afforded us substantial control over the assistant, it may not have presented the same stakes as a real-world one. 
% Outside the lab, conclusions from analyses may impact critical decisions, and analysts may be more careful because of this. 
% Similarly, the time pressure may have pushed analysts towards favoring execution assistance. 
As a result, participants may have been more willing to accept planning and execution assistance. We tried to mitigate this effect by priming analysts to consider the robustness of their analyses via our introductory material. 
% , and, contrastingly, may have placed assistant suggestions under greater scrutiny




% —when provided with planning assistance—
Finally, our study concentrated on analyst preferences, leaving evaluation of the resulting quality of analyses unaddressed. Determining analysis correctness is inherently challenging \cite{Silberzahn2018ManyAO, Breznau2022ObservingMR, Schweinsberg2021SameDD, Dutilh2018TheQO, BotvinikNezer2019VariabilityIT, Bastiaansen2019TimeTG, Menkveld2021NonStandardE}, with there often being 
% given that real-world analytical questions can yield a range of defensible analysis approaches \cite{Silberzahn2018ManyAO, Breznau2022ObservingMR, Schweinsberg2021SameDD, Dutilh2018TheQO, BotvinikNezer2019VariabilityIT, Bastiaansen2019TimeTG, Menkveld2021NonStandardE}. 
% Often, there is 
no single ``correct'' answer, but rather multiple defensible interpretations. However, extensive literature on multiverse analysis \cite{Steegen2016IncreasingTT, Simonsohn2015SpecificationCD, Liu2020BobaAA} notes the importance of considering alternative approaches. This helps analysts appreciate uncertainties surrounding their decisions and enhances analysis robustness. 
This work takes a step toward this larger goal by showing how planning assistance can guide analysts toward assessing multiple analytical perspectives. 
% Future research could examine the influence of planning assistance on analysis ``correctness.''

% or beginners in a more educational setting. 
% \tim{the educational part is interesting but came out of nowhere for me.}

% Finally, while overarching principles were in place as to when and what suggestions we raised, there is room for personal bias regarding what the wizard determined to be relevant and important. However, as our study is largely exploratory, there was no easy way to get around it without a rubric so rigorous it would assume the answer to what we were exploring. \tim{is this last sentence commonly put in woz papers? otherwise perhaps just say: as this was a necessarily exploratory study, the wizard was not bound to a strict protocol and it is possible that wizard actions reflected biases despite best attempts to mitigate them. --- are we worried about any particular bias? paragraph is important but feels very generic. what's a concrete example that would be problematic?}


% \subsection{Future work}
% \label{sec:discussion_future}

% \tim{this section feels overlapping with 8.3 design implications. I suggest to not call it future work and consolidate it into design implications. for example, calibrating trust seems to fit well there too. what do you think?}

% \xhdr{Designing for shared analysis goals and background}
% Given the importance of shared analysis goals and background between the analyst and the assistant (Sec. \ref{sec:discussion_commonground}), it is important to design mechanisms in the system to enable this union. That being said, there are open questions surrounding how this could best be achieved. Analysts could communicate this early on with the assistant and update this throughout the interaction. It is an open question on how to design this interaction such that there is not too much responsibility placed on the analyst to determine the level of assistance they require. Meanwhile, the assistant could infer analysts' goals based on the content of the analysis. \textit{LIDA}, \cite{Dibia2023LIDAAT} for example, uses LLMs to generate visualization goals based on a dataset. More broadly, recent work \cite{Park2023GenerativeAI} in the context of simulating human behavior in AI agents leverages ChatGPT to store experiences in memory, and dynamically retrieve the relevant background to inform agent behavior. Data analysis assistants can utilize a similar framework to store the background and actions of analysts and use the appropriate information to determine the adequate level of planning assistance at different moments in the analysis. However, this is no easy task. This was partially what the wizard was trying to do in our study and was difficult even with additional inputs from analysts' screens and audio. Future work could explore the extent to which LLMs can support this and what sorts of behaviors are characteristic of analysts engaging in analysis execution and  planning. 


% \xhdr{Designing for calibrated trust} 


%%%%%%%%%%
% Subsection: What
%     - Different levels of planning help
%     - Challenges with building a fully automated system and the stochastic nature/hallucinations that comes with LLMs

% Subsection: Helpfulness
%     - Varying analyst needs
%         - speed vs accuracy etc
%     - Changing assistant's goal:
%         - Effect on output conclusion of analysis
%             - Could take datasets /analysis goals that are hard in different ways and see if it’s able to catch

% Subsection: Common ground
%     - Impacting analyst perception of common ground
%         - Overreliance / trust  (& effect of wording on this perception)
%     - Impacting assistant perception of common ground:
%         - changing explicitness / methods of defining common ground (Subsection: initiative)
%     - Changing use of common ground
%         - More rigorous study of when different things are useful (Subsection: When)?











%%%%%%%% NOTES
% - Change so a small future work seciton at the bottom of each discussion section?

==> 9-conclusion.tex <==
\section{Conclusion}
This paper explores the potential of AI-based data analysis assistants that incorporate execution \textit{and} planning assistance. To understand the space of helpful suggestion content, we perform a \litreview review and a behavior-driven study to establish a categorization of suggestion content. To explore the essential components of a helpful suggestion, we design and conduct a \woz study that is inspired by but not limited by the capabilities of existing LLM-based assistants. This work contributes the first user study involving analysts working on a real dataset and task to better understand how to design and incorporate planning assistance into analysts' workflows. In addition, we provide an open-source implementation of an assistant interface building on prior work. From our study, we find that analysts found many categories of planning assistance helpful, highlighting the potential of incorporating planning assistance. However, in order to achieve this, it is crucial to comprehend and address the contextual factors that influence analysts' willingness to consider planning suggestions. We synthesize these findings to highlight design implications for future AI-based analysis assistants. Among these are aligning the analysis and the assistant on shared analysis goals and adding measures to reduce overreliance and promote trust 
% \tim{what could we say here to be  more specific about engagement? promote trust but not overreliance? etc?}
in this new analyst-assistant paradigm. 

% we will stick with design implications

% ...\ken{TODO: add what we contribute and how we have findings}


% \tim{is there some way to have the mega author lists abbreviated in the references?}

==> main-design-motivation.tex <==
\section{Design Motivation}
\label{sec:designMotivation}
Based on the formative study study in \autoref{formative}, we identify three design goals to support analysts in the multiverse debugging workflow (\autoref{fig:debug_workflow}). The goals correspond to addressing the three challenges identified in \autoref{subsec:workflow_model_exploratory}. 

\begin{enumerate}
    \item \textit{DG 1 - Reduce the time between executing universes and encountering errors.}
    After compiling a multiverse specification, a tool should enable analysts to quickly observe errors before committing to running the full multiverse. This is in the spirit of unit testing in which different components of the multiverse is rapidly tested before running the entire system. Quickly identifying errors before executing an entire multiverse may reduce time spent authoring (buggy) multiverse analyses.
    
    \item \textit{DG 2 - Give an overview of errors and how they relate to specific
    decision options.} Running thousands of universes can lead to thousands of individual error logs. In addition, errors may arise due to a combination of decision options, which the analyst did not test when writing the multiverse specification. Therefore, diagnosing the severity and frequency of an error helps to identify which parts of the code may need to be updated (including adding or removing dependencies between decision options in the multiverse specification). 
    % \tim{review previous sentence for accuracy}
    % is necessary to update code, which may impose or remove new dependencies between decision options. 
    To identify common bugs and distinguish among
    different kinds of bugs, summarizing the frequency of errors and connecting
    them to specific decisions and decision options are likely to help
    analysts.
    \item \textit{DG 3 - Support the abstraction and propagation of single universe error fixes to a multiverse specification} The context of a
    multiverse analysis adds new complexity to fixing errors. Analysts may elect to debug errors in a specific universe as opposed to the higher-level multiverse specification. This enables analysts to take advantage of already familiar and idiosyncratic ways of debugging specific universe errors. In the analysts process of debugging a single universe, they can leverage an entire ecosystem of single script debugging tools that they may already be familiar with. Therefore, making the process of propagating changes to individual universes to the higher-level multiverse specification easier, empowers the single universe debugging workflow. 
    
\end{enumerate}

==> old/8-discussion-future-work_v1.tex <==
\section{Discussion}
\label{sec:discussion}

In this work, we set out to understand the design of AI-powered analysis assistants that provide execution \textit{and} planning assistance. As planning assistance is under-explored and underdeveloped in existing systems, we placed special attention on this form of assistance. To first understand the scope of suggestion content, we performed a \litreview review and a behavioral-driven analysis of crowd-sourced analyses (Sec. \ref{sec:suggestions}) and defined categories of relevant suggestions (Table \ref{tab:suggestions}). Next, we designed (Sec. \ref{sec:woz_design}) and conducted (Sec. \ref{sec:labstudy}) a \woz study to understand what suggestions are helpful to analysts and how these suggestions impact analysts' workflows.

Here, we discuss the implications of our study findings for creating helpful assistants. In Section~\ref{sec:discussion_helpful} we examine various ways of defining the goals of raising suggestions, and how that may impact design. We then explain in Section~\ref{sec:discussion_commonground} why establishing common ground is critical to achieving these defined goals. Section~\ref{sec:discussion_initiative} discusses the dimensions along which this common ground can be established, and Section~\ref{sec:discussion_when} discusses the importance of updating this common ground over time. Finally, by establishing common ground as the crux for making helpful suggestions, we  present design guidelines based on our current findings in Section~\ref{sec:discussion_design} and avenues for future research in Section~\ref{sec:discussion_future}.

\subsection{What makes a suggestion helpful?}
\label{sec:discussion_helpful}

To define what sorts of suggestions may be helpful, we created a categorization of suggestion content as shown in Table~\ref{tab:suggestions}. In our subsequent \woz study, we found both execution and planning suggestions were considered helpful (Sec. \ref{sec:results_what_assistance}). However, while execution assistance was almost always considered beneficial, analysts' reception of planning assistance was more varied. We noticed the same raised planning content (e.g., interpreting the outputs of a linear model) was received differently depending on contextual factors, which we outlined in Section~\ref{sec:results} through a who-what-where-when-why-how framework. 

% \mgm{is the following fair? Def need to reword} We posit that the impact of contextual factors on the perceived helpfulness of planning suggestions is for several reasons. First, most people when trying to achieve a specific function, would agree on some level of execution as long as it processes inputs into an output correctly. However, an analysis plan can be much more varied and personalized based on higher-level goals. Even with the same data set and question, there are different approaches and goals for rigor at different parts of the analysis process. Furthermore, the stakes are higher, as it is more intrusive on the analyst's workflow to have them consider multiple possible paths, which increases the negative impacts when suggestions are not helpful. 

There are several factors that contribute to the nuanced difference in preferences. For analysis execution, analysts have a direct goal: write code to help execute the current analysis task. With existing systems, this can be achieved by continuing analysts' current code context. However, analysis planning can be much more varied and personalized depending on the analysts' background (Sec. \ref{sec:results_who}), something that may not be obviously clear based on analysts' immediate notebook contents. Even with the same data set and question, we noticed analysts naturally consider different approaches, with different levels of rigidity to these approaches, and at different points analysis process (Sec. \ref{sec:results_who_analysisplan}). Furthermore, the stakes are higher when providing a planning suggestion. Planning assistance is more intrusive on the analyst's workflow as they must consider multiple possible analysis decisions, rationales behind these decisions, and where the suggestion fits into their overall analysis plan. This increases the negative impacts when suggestions are not helpful. 

We also found analysts had different perspectives on what planning assistance would be helpful. These perceptions varied across analysts, and within analysts over time. This ranged from treating planning assistance as help for precise analysis steps, to guidance for overall workflow planning (Sec. \ref{sec:results_what_assistance}), to distractions on the side while analysts only consider their own plan. 

% also -- multiple levels of planning goals -- th overall gaol and the current steps

In our study, because we were motivated to assist analysts in making more informed inferences, the assistant provided suggestions that aimed to help analysts consider alternative but reasonable approaches. 
% we considered suggestions to be helpful if they impacted analysts to consider new workflows that the analysts considered to be ``helpful.''
However, based on our observations of analysts' reasons to use our assistant (Sec. \ref{sec:results_why}), there can be other goals that assistants can have. Beyond promoting analysts to consider alternative decisions, data analysis assistants could prioritize helping analysts flesh out their analysis plan. Alternatively, assistants could only provide execution assistance in speeding up analysts' analysis plans. Or, the assistant could serve in a teaching role. 

Different assistant goals may lead to different definitions of what it means to be helpful as the assistant, and this may be in tension with analysts' perspectives of usefulness. For example, if the assistant's goal is to broaden the analysts' understanding of the decision space, then it might prefer offering planning assistance over execution assistance despite analysts' universal affinity towards execution assistance. Therefore, to surface helpful suggestions, ideally, the assistant will strike a balance between understanding and acting upon the analyst's view of what is helpful and the assistant's objective of its ideal impact on an analyst's workflow.

%%%%%%%%%%%%%%%%%%%%
% We defined a lot of helpful suggestions via literature review. Included both execution (previously done) and planning (relatively new) in our study. Found overall in our study that most people found planning and execution helpful. 


% We did the goal of being open to new workflows, focused on the content they put into the jupyter notebook. However, because of the variety in analysis perspective,  This happened even wiht a defined AI designer perspective, and that could change depending on the context. 


% We define this ``helpfulness'' very loosely on purpose, because it may vary. 

% Varies along analysts perspective
% - sometimes want lazy assistance
% - sometimes wants to open new workflows
% - sometimes wants speed
% - sometimes a combination
% - level of abstraction they're looking for
% - sometimes changes along analysts (they discussed wanting toggles and stuff)
% - What is the end goal? even with same data set (and sometimes same question too), could be different approaches or levels of rigor or where they feel lost.


% Also varies along AI designer's perspective. In our study, we focused on getting anlaysts to consider new workflows
% - Is it to help along with current analysis path with small misses?
% - Is it to just help the analyst on whatever they want to do?
% - Is it to challenge the analyst and get towards some specific goal? 
% - is it to update analysts beliefs only or also their actions?


% To surface helpful suggestions, ideally, assistant will find a balance between understanding and acting upon analyst's view of what is helpful and it's objective of how much to challenge with vs smoothly support the analyst's workflow.


\subsection{The importance of common ground}
\label{sec:discussion_commonground}

To create this alignment \mgm{(loaded word but maybe it works?)} necessary for helpful suggestions, it is critical to establish common ground

Common ground is \mgm{TODO: definition}. In past HAI work it is described by \mgm{TODO}. Ours is different because \mgm{TODO: planning much more higher level so requires common ground, a lot more context, etc.}\ken{not sure if different or just follow and adapt for data analysis scenario. Will have to see what the works say}.

Through our study, we found that analysts often considered suggestions to be unhelpful was a misalignment between the mentality of the analyst and the context in which the suggestion was raised \mgm{(is this fair? reword to be more specific)}\ken{maybe: the analysts' current focus (i.e., analysis execution or a specific level of analysis planning), their background, and the content and timing of the assistance (Fig. \ref{fig:results}G and H vs. D and E)}. 
Throughout the analysis process, an ideal assistant would completely understand the analyst's background, overall goals, and current plan (Fig.~\ref{fig:results}G and H) and reconcile that with the assistant's own goals (Fig.~\ref{fig:results}D). The analyst should also understand the assistant's goals in addition to the assistant's capabilities. This common understanding is the basis from which helpful assistance can be provided and perceived. 

\subsection{Creating common ground between analyst and agent}
\label{sec:discussion_initiative}
\
The analyst and assistant need to establish common ground in the beginning about the analyst's background, needs and goals. They then should continue creating common ground about the analyst's updating plan throughout the analysis process. Unfortunately, a perfect level of common understanding is unrealistic, as the methods of communication are just the assistant's suggestions, the notebook contents, and the agent's initiative. In our study, as described in Section~\ref{sec:results_how}, the analyst's initiative to interact with the agent is just the content they type into the notebook, and we briefed them on this method of interaction in the beginning of the study. Throughout the study, users continued to try different ways of interacting and typing commands to see the impacts of their actions. In follow interviews, users were especially interested in how to expand this ability to establish their own initiative (e.g. \mgm{TODO: direct query, specifying when to get results, wishes for less initiative and more initiative of the agent,}). Methods for creating this common ground on the ever-changing and variable task of data analysis is an interesting path for future work that we discuss in more detail in Section~\ref{sec:discussion_future}.

Furthermore, at the moment our assistant does not explicitly request any information from the user (e.g. their goal, statistical background, etc). Our assistant also does not provide any intro specifically to build up basics first so person has understanding of what the tool can do. More explicit definition of these aspects may be helpful in establishing common ground. 


\subsection{Updating common ground over time}
\label{sec:discussion_when}

An incredibly important factor was the time the suggestion was raised in relation to the workflow, as described in Section~\ref{sec:results_when}. The users' needs are different in the beginning, middle, and end of the analysis process \mgm{TODO: cite?}, and often go in iterative refinement loops. If the suggestion raised is too different from the analyst's perspective of their current needs, they will ignore, get distracted, or put a pin in it for later. If the suggestion is completely in line with their current practices, execution help may help it become faster, but the assistant's helpfulness for planning is limited. 

The time at which suggestions are raised seems critically important from our user study, but this phenomenon can be much more rigorously studied. We discuss these potential avenues for future work in Section~\ref{sec:discussion_future.} \mgm{Right now not very in detail in the future work section. I think either flesh out more details, or bring up future work here so doesn't need to stand alone as much}

%%% Not sure if to include or not:
% Additionally, what the assistant surfaces in the beginning impacts the analyst's perspective of the assistant over time. 
%  possibly include here how it relates to how llms like to just do sequencing and stuff?

\subsection{Takeaways for designers}
\label{sec:discussion_design}

For designers looking to create assistants that can help with both planning and execution, we have created a set of recommended design guidelines. These are based on our literature review and user study, however, we expect them to be further defined by future work. 

\subsubsection{Design guidelines}
\label{sec:discussion_design_guidelines}
\mgm{TODO: I'm not sure what goes here. You can't control who it is or how it will be recieved, but can control what you ask of the person/the initiative you have, the content you raise, the methods by which you raise it, and when you raise it}
\mgm{TODO: how guidelines we've found are different from other HAI ones}
- Include organization of suggestions here

\subsubsection{Steps to a functional system}
\label{sec:discussion_design_system}
\mgm{TODO: anticipated road blocs}
\mgm{TODO: steps for building an actual system}



\subsection{Future work}
\label{sec:discussion_future}

There are promising future directions for better understanding what types of suggestions these assistants can provide, how to make the suggestions helpful, and how to establish the common ground necessary to make the suggestions helpful.

\subsubsection{Suggestion content}
We provide a variety of levels of planning abstraction and execution help with our suggestions, using content types defined by a literature review. However, future work could compare different levels of planning abstraction in a more rigorous way to define these levels and see their effect. 

We conduct a \woz study in order to focus on ideal design rather than the limitations of current LLM capabilities. We encourage future work to explore the challenges of building a fully (or more) automated system that accounts for hallucinations and the stochastic nature of LLMs. \mgm{TODO: need to cite?}

\subsubsection{Helpfulness of suggestions}
We establish the goal of an assistant that helps the analyst think of alternative plans, and we do not provide specific incentives to the analyst. However, future work can vary analyst needs and incentives (e.g. speed vs robustness of analysis), as well as their background (e.g. level of statistical knowledge). Future work can also change the assistant's definition of what is helpful. For example, our study did not consider the analyst's final answer, but future work could measure utility by if the final output is correct, or if throughout the process analysts are able to avoid common pitfalls when given a difficult dataset or analysis.

\subsubsection{Common ground}
We see multiple avenues of future work for better understanding the impact and establishment of common ground in the analysis domain. First, there are ways of incorporating prior work on overreliance, trust, and wording into understanding how the system design affects the analyst's perception of common ground. Future work can also change the methods of communication between the assistant and the analyst to impact how the assistant's perception of common ground is created and defined. Finally, future work can more specifically study the impact of when different kinds of content are raised on their utility. 

\subsection{Limitations}

%%%%%%%%%%
% Subsection: What
%     - Different levels of planning help
%     - Challenges with building a fully automated system and the stochastic nature/hallucinations that comes with LLMs

% Subsection: Helpfulness
%     - Varying analyst needs
%         - speed vs accuracy etc
%     - Changing assistant's goal:
%         - Effect on output conclusion of analysis
%             - Could take datasets /analysis goals that are hard in different ways and see if it’s able to catch

% Subsection: Common ground
%     - Impacting analyst perception of common ground
%         - Overreliance / trust  (& effect of wording on this perception)
%     - Impacting assistant perception of common ground:
%         - changing explicitness / methods of defining common ground (Subsection: initiative)
%     - Changing use of common ground
%         - More rigorous study of when different things are useful (Subsection: When)?











%%%%%%%% NOTES
% - Change so a small future work seciton at the bottom of each discussion section?

==> old/8-discussion-future-work_v2.tex <==
\tableResults

\section{Discussion}
\label{sec:discussion}
In this work, we set out to understand how to incorporate planning assistance into AI-powered analysis assistants. To first understand the scope of suggestion content, we performed a \litreview review and a behavioral-driven analysis of crowd-sourced analyses (Sec. \ref{sec:suggestions}) to define categories of relevant suggestions (Table \ref{tab:suggestions}). Next, we designed (Sec. \ref{sec:woz_design}) and conducted (Sec. \ref{sec:labstudy}) a \woz study to understand the circumstances in which suggestions are helpful. Here, we discuss the implications of our study findings for creating helpful assistants summarized in (Table~\ref{tab:design_implications}).
% First, we examine various ways of defining the goals of raising suggestions, and how that may impact the design of the assistant (Sec. \ref{sec:discussion_helpful}). We then explain why establishing common ground is critical to achieving these defined goals (Sec~\ref{sec:discussion_commonground}). Using the framework of common ground and integrating our observations from our study, we share design implications for building a data analysis assistant (Sec~\ref{sec:discussion_design_guidelines}). We conclude our discussion by reviewing study limitations (Sec.~\ref{sec:discussion_limitations}) and discussing avenues for future research (Sec~\ref{sec:discussion_future}).

\subsection{What Makes a Suggestion Helpful?}
\label{sec:discussion_helpful}

% To define what categories of suggestions content may be helpful, we created a categorization of suggestion content as shown in Table~\ref{tab:suggestions}. In our subsequent \woz study, we found both execution and planning suggestions were considered helpful (Sec. \ref{sec:results_what_assistance}). We provided analysts a thumbs up and down button (Fig. \ref{fig:interface}F) such that they can apply their own definition of helpfulness towards each suggestion. However, while execution assistance was almost always considered beneficial, analysts' reception of planning assistance was more varied.

% Contextual factors which we described in Section~\ref{sec:results}, were often referenced as reasons for why planning suggestions were preferred.

In our study, we noticed the same planning suggestion content (e.g., interpreting the outputs of a linear model) was received differently depending on contextual factors (Sec.~\ref{sec:results}).
% , which we described in Section~\ref{sec:results} through a who-what-where-when-why-how framework. 

% \mgm{is the following fair? Def need to reword} We posit that the impact of contextual factors on the perceived helpfulness of planning suggestions is for several reasons. First, most people when trying to achieve a specific function, would agree on some level of execution as long as it processes inputs into an output correctly. However, an analysis plan can be much more varied and personalized based on higher-level goals. Even with the same data set and question, there are different approaches and goals for rigor at different parts of the analysis process. Furthermore, the stakes are higher, as it is more intrusive on the analyst's workflow to have them consider multiple possible paths, which increases the negative impacts when suggestions are not helpful. 

% There are several factors that contribute to the nuanced difference in preferences. For analysis execution, analysts have a direct goal: write code to help execute the current analysis step. With existing systems, this can be achieved by continuing analysts' current code context. However, 

As opposed to analysis execution, in which the focus is to write code to execute the current analysis step, analysis planning can be much more varied and personalized depending on the analyst's background (Sec. \ref{sec:results_who}) and analysis progress (Sec.~\ref{sec:results_when}). Analysts naturally considered different approaches, with different levels of rigidity to these approaches, and at different points in the analysis process (Sec. \ref{sec:results_who_analysisplan}). Within analysis planning, there are also different levels of abstraction. For example, analysts may make broader planning decisions about the choice of the statistical model, or after choosing the statistical model, make fine-grained choices of model regularization parameters. 

% Furthermore, the stakes are higher when providing a planning suggestion. Planning assistance is more intrusive on the analyst's workflow as they must consider multiple possible analysis decisions, rationales behind these decisions, and where the suggestion fits into their overall analysis plan. This increases the negative impacts when suggestions are not helpful. 


% \tim{I noticed that we didn't discuss planning on different levels of abstraction, e.g. do I want to use a Lasso model vs other model. and I should check a few different regularization parameter values. Was that important?}
% \tim{I visualize this as a triangle with execution at the very bottom and  multiple planning  layers on top. Interestingly, execution takes lots of time and that's what execution assistance tools focus on. that's important  but it focuses on reducing time, not necessarily improving the analysis. that takes planning considerations. without that, the execution  may even focus on  misguided directions and be wasteful/misleading even if accelerated by execution assistance.  ---- what do you think of this higher level picture? }

As a result, we found analysts had different perspectives on what planning assistance would be helpful. These perceptions varied across analysts and within analysts over time. This ranged from treating planning assistance as help for precise analysis steps to guidance for overall workflow planning (Sec. \ref{sec:results_what_assistance}), to distractions on the side while analysts only consider their own plan. Moreover, despite mainly providing suggestions that aimed to help analysts consider alternative but reasonable approaches, analysts liked execution assistance (Sec. \ref{sec:results_why}). This follows the preferences found in prior works that studied code execution assistants \cite{Vaswani2017AttentionIA, Liang2023UnderstandingTU, Ross2023ThePA}.

% also -- multiple levels of planning goals -- th overall gaol and the current steps

% In our study, because we were motivated to assist analysts in making more informed inferences, the assistant provided suggestions that aimed to help analysts consider alternative but reasonable approaches. 
% we considered suggestions to be helpful if they impacted analysts to consider new workflows that the analysts considered to be ``helpful.''
% However, based on our observations of analysts' reasons to use our assistant (Sec. \ref{sec:results_why}), analysts widely favored execution assistance. 

Unsurprisingly, analysis execution takes lots of time and this is what execution assistance tools focus on. For planning assistance, the stakes are understandably higher. Planning assistance is more intrusive on the analyst's workflow as analysts must consider multiple possible analysis decisions, rationales behind these decisions, and where the suggestion fits into their overall analysis plan. This increases the negative impacts when suggestions are not helpful. However, while execution assistance is valuable for reducing time, it does not necessarily improve the analysis. Without taking proper planning considerations, execution assistance may focus on misguided directions and be wasteful or misleading. 

% Beyond recommending analysts consider alternative decisions, data analysis assistants could prioritize helping analysts flesh out their analysis plan. Alternatively, assistants could only provide execution assistance in speeding up analysts' analysis plans. Or, the assistant could serve in a teaching role. 

Different goals between the assistant and analysts may lead to different definitions of what is considered helpful.  While analysts' goals are primary, assistant goals, even those in potential tension with analysts, might be important. Providing planning assistance aims towards higher quality and more robust data analysis. Only serving analysts on execution assistance may not lead to such outcomes. Therefore, striking a balance between understanding analysts' perspectives of helpfulness and the assistant's impact on the workflow is crucial for providing truly valuable suggestions.

% Therefore, to surface helpful suggestions, ideally, the assistant will strike a balance between understanding and acting upon the analyst's view of what is helpful and the assistant's objective of its impact on the analyst's workflow.

% For example, if the assistant's goal is to broaden the analysts' understanding of the analysis decision space, then it might prefer offering planning assistance over execution assistance despite analysts' affinity towards execution assistance. Therefore, to surface helpful suggestions, ideally, the assistant will strike a balance between understanding and acting upon the analyst's view of what is helpful and the assistant's objective of its impact on the analyst's workflow.

% \tim{in the paragraphs above we should say more clearly that analyst and assistant have goals. While analysts goals are primary, assistant goals, even those in potential tension with analysts, might be important. I see our planning assistance towards higher quality / more robust data analysis as such a goal. of course these need to be reconciled but the point is that an assistant  only serving the analyst what they want on their initiative may not lead to important outcomes that we are after. }

%%%%%%%%%%%%%%%%%%%%
% We defined a lot of helpful suggestions via literature review. Included both execution (previously done) and planning (relatively new) in our study. Found overall in our study that most people found planning and execution helpful. 


% We did the goal of being open to new workflows, focused on the content they put into the jupyter notebook. However, because of the variety in analysis perspective,  This happened even wiht a defined AI designer perspective, and that could change depending on the context. 


% We define this ``helpfulness'' very loosely on purpose, because it may vary. 

% Varies along analysts perspective
% - sometimes want lazy assistance
% - sometimes wants to open new workflows
% - sometimes wants speed
% - sometimes a combination
% - level of abstraction they're looking for
% - sometimes changes along analysts (they discussed wanting toggles and stuff)
% - What is the end goal? even with same data set (and sometimes same question too), could be different approaches or levels of rigor or where they feel lost.


% Also varies along AI designer's perspective. In our study, we focused on getting anlaysts to consider new workflows
% - Is it to help along with current analysis path with small misses?
% - Is it to just help the analyst on whatever they want to do?
% - Is it to challenge the analyst and get towards some specific goal? 
% - is it to update analysts beliefs only or also their actions?


% To surface helpful suggestions, ideally, assistant will find a balance between understanding and acting upon analyst's view of what is helpful and it's objective of how much to challenge with vs smoothly support the analyst's workflow.


\subsection{The Importance of Common Ground}
\label{sec:discussion_commonground}

To create the alignment necessary for helpful suggestions, it is critical to establish common ground. Common ground is the shared understanding between two participants in a dialogue or interaction. In psychology, “two people’s common ground is, in effect, the sum of their mutual, common, or joint knowledge, beliefs, and suppositions”~\cite{clark1996using}. With people, this common ground is established through many means, including a contextual understanding of the setting of interaction, shared cultural knowledge, shared experiences, and social and transactional dialogue~\cite{clark2019makes}. 

Computer science research also notes the importance of establishing common ground through dialogue between an agent and a person. For example, when communicating with a robot, prior work has emphasized having a shared understanding of the world and communicating internal representations from the robot to the user~\cite{chai2014collaborative,chai2016collaborative}. In conversational models, common ground is a crucial component of effective communication and personalization to the context and person of that interaction~\cite{clark2019makes,kopp2021revisiting}. 

 We find that common ground between the analyst and the assistant is also important for AI-powered planning and execution assistance. In this application, common ground refers to understanding the analyst's and the assistant's analysis goals, the assistant's capabilities, the analyst's analysis process, and the analyst's domain, statistical, and AI backgrounds. In our study, we observed analysts often found suggestions unhelpful when the content and timing of the suggestion did not align with the analyst's background and current focus. Throughout the analysis process, an ideal assistant would completely understand the analyst's background, overall goals, and current plan (Fig.~\ref{fig:results}G and H) and reconcile that with the assistant's own goals (Fig.~\ref{fig:results}D). On the other hand, the analyst should also understand the assistant's goals in addition to the assistant's capabilities. 

To summarize, the assistant's perception of the analyst (Fig.~\ref{fig:results}C) should be matched with the analyst's goals (Fig.~\ref{fig:results}G) while considering the assistant's own goals (Fig.~\ref{fig:results}D). Likewise, the analyst's perception of the assistant (Fig.~\ref{fig:results}F) should match the analyst's goals for the analysis (Fig.~\ref{fig:results}G) while also considering the assistant's goals (Fig.~\ref{fig:results}D). This common understanding is the basis from which helpful assistance can be provided and perceived. 

% \tim{or vice versa?}

% \subsection{Creating common ground between analyst and agent}
% \label{sec:discussion_initiative}
% \
% The analyst and assistant need to establish common ground in the beginning about the analyst's background, needs and goals. They then should continue creating common ground about the analyst's updating plan throughout the analysis process. Unfortunately, a perfect level of common understanding is unrealistic, as the methods of communication are just the assistant's suggestions, the notebook contents, and the agent's initiative. In our study, as described in Section~\ref{sec:results_how}, the analyst's initiative to interact with the agent is just the content they type into the notebook, and we briefed them on this method of interaction in the beginning of the study. Throughout the study, users continued to try different ways of interacting and typing commands to see the impacts of their actions. In follow interviews, users were especially interested in how to expand this ability to establish their own initiative (e.g. \mgm{TODO: direct query, specifying when to get results, wishes for less initiative and more initiative of the agent,}). Methods for creating this common ground on the ever-changing and variable task of data analysis is an interesting path for future work that we discuss in more detail in Section~\ref{sec:discussion_future}.

% Furthermore, at the moment our assistant does not explicitly request any information from the user (e.g. their goal, statistical background, etc). Our assistant also does not provide any intro specifically to build up basics first so person has understanding of what the tool can do. More explicit definition of these aspects may be helpful in establishing common ground. 


% \subsection{Updating common ground over time}
% \label{sec:discussion_when}

% An incredibly important factor was the time the suggestion was raised in relation to the workflow, as described in Section~\ref{sec:results_when}. The users' needs are different in the beginning, middle, and end of the analysis process \mgm{TODO: cite?}, and often go in iterative refinement loops. If the suggestion raised is too different from the analyst's perspective of their current needs, they will ignore, get distracted, or put a pin in it for later. If the suggestion is completely in line with their current practices, execution help may help it become faster, but the assistant's helpfulness for planning is limited. 

% The time at which suggestions are raised seems critically important from our user study, but this phenomenon can be much more rigorously studied. We discuss these potential avenues for future work in Section~\ref{sec:discussion_future.} \mgm{Right now not very in detail in the future work section. I think either flesh out more details, or bring up future work here so doesn't need to stand alone as much}

%%% Not sure if to include or not:
% Additionally, what the assistant surfaces in the beginning impacts the analyst's perspective of the assistant over time. 
%  possibly include here how it relates to how llms like to just do sequencing and stuff? 

\subsection{Design Implications}
\label{sec:discussion_design_guidelines}
In this section, we synthesize our observations and the discussion on common ground. We highlight seven design implications that add to existing Human-AI Interaction guidelines \cite{Amershi2019GuidelinesFH} for the application of designing a data analysis assistant.

\subsubsection{Assistants should communicate with the analyst to align on analysis goals}
% The old  Creating common ground between analyst and agent could probably fit in here.
\label{sec:discussion_design_implications_match_goals}


% In this paragraph talk about how it should be on the agent to establish it? Or maybe in the parapgrah on how to establish

During the analysis portion of our study, the wizard was sometimes unaligned with the analyst's goals (Sec.~\ref{sec:results_when}). Likewise, analysts spent time figuring out the assistant's goals (Sec.~\ref{sec:results_who_curiosity}).
% \tim{it stands out to me that this is the "opposite direction"} 
% A few curious analysts typed comments seeking suggestions from the assistant and were curious about the assistant's resulting suggestions to understand the assistant (Sec.~\ref{sec:results_who_curiosity}).
% For example, participants noted if the assistant gave information similar to queries they had typed in comment boxes [A3, A8, A10]~\mgm{include A-X descriptions here if it's included in results section?}, and noted when the assistant did not respond to other kinds of artifacts in the notebook, such as error messages [A5, A13]. \ken{i usually just refer to results section but we can see what others think. Also I think this discussion was more about capabilities then goals.}
% Moreover, analysts in our study wanted more agency (e.g. directly prompting, choosing from a list of options, and specifying when they wanted to receive inputs) to direct the assistant toward their goals (Sec.~\ref{sec:results_how}).

Therefore, the analyst and the assistant need to establish shared goals at the beginning of the analysis, and this understanding should evolve over time. Although prior work on conversational agents has found users wanted the system to only adapt and personalize to them ~\cite{clark2019makes}, we argue it is still important to communicate and reconcile shared goals between the analyst and the assistant. In the context of data analysis, blindly following the analyst's execution preferences may perpetuate poor analysis decisions and practices leading to misguided inferences. Thus, it is necessary to communicate clearly the goals of planning assistance to the analyst. After, the analyst and the assistant can work towards coordinating their collaboration. Understanding the best ways to establish, integrate, and uphold shared goals over time is an important area for future exploration.


% \tim{this is great, just make this a bit more clear above or argue for why it should only be in one section?}


\subsubsection{Assistants should provide suggestion content suited to the analyst's background}
\label{sec:discussion_design_implications_match_bg}

% different people had different prior knowledge, preffered one staistical approach over the other, had different levels of understanding, coding expertise etc. 
As another facet of encouraging common ground, the assistant should match suggestion content to the analyst's background. Analysts differ in their statistical, domain, and coding backgrounds even amongst those who self-reported as proficient in statistical analysis. We observed that these differences between analysts impacted their analysis plan as well as their reactions to suggestions. The same suggestion could be considered helpful by some participants, while others considered it to be too elementary and distracting, too separated from their expertise such that testing its validity was prohibitively difficult, or too different from their usual analysis or coding practices to be useful (Sec. \ref{sec:results_who_expertise}). 

 % Prior work on conversational agents found many users thought the system should take on the burden of establishing common ground to personalize outputs~\cite{clark2019makes}\mgm{This seems to be an interesting point but I'm not quite sure where to put it.}. 
In our study, the assistant does not explicitly request any information from the analyst. A more explicit definition of the analyst's background knowledge, such as through analyst initiative (Fig. \ref{fig:results}A), may be helpful in establishing common ground. 

For instance, analysts may configure their backgrounds by providing a short bio or filled template containing their educational background, self-rating of their coding expertise, typical workflows, and preferences for analysis methods and software packages. This can then be used as relevant context to customize LLM-based assistant suggestions \cite{Andreas2022LanguageMA, Kirk2023PersonalisationWB}. 


% different levels of explanation for different audiences
\subsubsection{Assistants should match the analyst's preferred level of planning assistance abstraction.}
\label{sec:discussion_design_implications_match_abstraction}

As discussed in Section \ref{sec:discussion_commonground}, there are multiple perspectives of helpful planning assistance. This can range from guiding analysts in choosing hyper-parameters to providing a comprehensive plan with multiple analysis steps.
% \tim{I must have missed this?!}
% What analysts find helpful at the moment depends on their background and goals and their current planning process. 
Future assistants should account for analysts' preferences regarding different levels of planning assistance and how these preferences may change throughout the analysis process. This could be communicated explicitly by the analyst (analyst initiative) via the user interface. For instance, analysts may want to iteratively refine their intent for assistance such as in \textit{Wrex}, a non-LLM-based notebook extension that generates code based on programming by example \cite{Drosos2020WrexAU}. The assistant could also provide the analyst dials for offering assistance such as an "execution" mode that focuses on code execution and a "exploration" mode for planning suggestions.
% ikewise, there could be a "exploration" mode for when the analyst needs more consideration of planning focused suggestions while coordinating these with their current analysis. 

% \ken{any works similar to this with different modes for abstraction to cite} \tim{maybe check in w Jeff directly}. 
The assistant can also learn analysts' preferences by observing their behavior across multiple analyses. At a finer scale, as analysts' needs may not always be the same between analyses, the assistant should also learn analysts' goals and behavior for the current analysis. More broadly, recent work \cite{Park2023GenerativeAI} in the context of simulating human behavior in AI agents leverages ChatGPT to store experiences in memory, and dynamically retrieve the relevant background to inform agent behavior. Data analysis assistants can utilize a similar framework to store the background and actions of analysts and use the appropriate information to determine the adequate level of planning assistance at different moments in the analysis. Future research can explore how LLMs can support this and identify characteristic behaviors of analysts engaged in analysis execution and planning.
% However, this is no easy task. This was partially what the wizard was trying to do in our study and was difficult even with additional inputs from analysts' screens and audio. Future work could explore the extent to which LLMs can support this and what sorts of behaviors are characteristic of analysts engaging in analysis execution and planning

Likewise, the level of abstraction also relates closely to the scope of the analysis code that the assistance affects. An analytical decision could be one parameter, line, function, code block, or even multiple chunks of code \cite{Liu2020BobaAA}. Once a suggestion impacts large parts of the analyst's analysis, it requires more willingness from the analyst to consider and adopt the suggestion. Thus, future assistants should consider the scope of analysis a suggestion influences.

\subsubsection{Assistants should time suggestions based on the analyst's openness to considering alternative approaches.}
\label{sec:discussion_design_implications_timing}

In our study, analysts expressed liking certain suggestions but felt they were not well-timed based on their current analysis process (Sec. \ref{sec:results_when}). When analysts are focused on executing a specific analysis decision or plan, they may prefer execution assistance rather than planning suggestions. Conversely, when analysts are considering their next steps, they may be more open to guidance for analysis planning. Therefore, assistants should recognize when analysts are open to planning assistance. Analysts can explicitly communicate their preferences to the assistant or use a "remind me later" response for suggestions. Additionally, organizing and tagging suggestions can help analysts easily find and revisit helpful suggestions, even if the timing was not ideal. (Sec.~\ref{sec:results_where}). 

Meanwhile, the assistant can also learn proper timing through analysts' behaviors. For instance, simple sensors could be used to model and predict human interruptibility \cite{Fogarty2005PredictingHI}. The assistant could also follow a utility model for mixed-initiative AI intervention by considering the expected utility of different actions\cite{Horvitz1999PrinciplesOM}. We note that this may be challenging if analysts only want to fixate on a rigid analysis plan, highlighting the importance of establishing shared goals between the analyst and the assistant (Sec. \ref{sec:discussion_design_implications_match_goals}). While many analysts may prefer planning assistance, there may be tension in considering planning assistance for others.
% \tim{the last sentence speaks to the question: Is there ever a good time to engage the analyst on planning assistance. It sounds  like while this is the case for many, it isn't for some and that's an inherent tension. perhaps clarify that slightly here.}

\subsubsection{Assistants should provide multiple ways to request content at different abstraction levels.}
\label{sec:discussion_design_implications_initiative}

Analysts preferred to have their own initiative in requesting suggestions (Sec.~\ref{sec:results_how}) and had different preferences for levels of planning assistance (Sec.~\ref{sec:results_what_assistance}). Therefore, there is an open question as to how analysts can request assistance, and at what level of abstraction. 

There is flexibility around the input mechanism and initiative. For example, analysts can write comments, select text, trigger suggestions via a hotkey, request proactive suggestions in a side panel, etc. Each of these can carry implicit context regarding the level of feedback analysts desire \cite{McNutt2023OnTD}. Ambient and textual interfaces (i.e., assistant follows the cursor and can be invoked via an action) suggest localized context and help. For example, a common workflow with execution assistants such as Github Copilot is for the programmer to write comments that detail what the lines of code should be to complete the task \cite{Vaithilingam2022ExpectationVE}. Meanwhile, a side-panel interface with controls outside the immediate notebook suggests global context and help. 

While existing systems usually offer one form of invocation, LLM-powered analysis assistants should allow and interleave multiple forms of invocation and context for different granularity of assistance. It is also important to clarify the context for the LLM in each form of interaction. For example, a hotkey trigger at the line level may indicate a focus on execution assistance using only the current cell. On the other hand, analysts can specify broader suggestions when requesting feedback in the side panel and choose the LLM context by selecting relevant cells. 

Interactive visualizations can also be employed to show and allow analysts to select analysis decisions and alternative choices \cite{Liu2019PathsEP, Liu2020BobaAA}. These visualizations (e.g., Fig~\ref{fig:teaser}), tied to the analysis code, allow analysts to review their steps and select areas where additional assistance is needed.

\subsubsection{Assistants should provide relevant forms of suggestion explanation.}
\label{sec:discussion_design_implications_explanation}
Analysts highly valued suggestion explanations to better understand and trust the assistant's suggestions (Sec.~\ref{sec:results_what_qualities}). In our study, code, code comments, and natural language suggestion rationales all contributed to explaining suggestions. Future assistants should incorporate multiple forms of explanations, considering analysts' backgrounds and preferences. To avoid verbosity, assistants could allow analysts to select their preferred forms of explanation. Moreover, there are other potential methods to present suggestion explanations. For example, visualizations or animations of the data during and after data transformations can help analysts understand the code actions of the assistant \cite{Pu2021DatamationsAE, Xiong2022VisualizingTS}. 





\subsubsection{Assistants should design for calibrated trust.}
\label{sec:discussion_design_implications_trust}

\ken{TODO relate this to observation in results section \ref{sec:results_who_curiosity}} 
\ken{from tim:  We should discuss this later if we haven't yet. danger to make things worse, especially if the assistant is not worthy of the trust put in it. see \ref{sec:results_why}}
Large Language Models are adaptable, but they often have erroneous outputs~\cite{Amershi2019GuidelinesFH,bender2021dangers}. In our study, one analyst [A4] caught an error in a ChatGPT-generated result analysis suggestion that suggested a result was significant at a p-value of $.15$. In response to errors in Machine Learning models, prior work stresses the importance of creating calibrated trust: or aligning the human's willingness to accept the model's response as accurate with the model's capabilities~\cite{bansal2021does,zhang2020effect,tomsett2020rapid}. A related goal is reducing overreliance, a phenomenon when people take an AI's prediction or advice when it is low quality or incorrect~\cite{buccinca2021trust,bussone2015role,vasconcelos2023explanations}.

Future work on AI data analysis assistants could study the impacts of assistant design on calibrating trust and overreliance on suggestions. 

For example, a study could present some incorrect suggestions and measure if analysts notice the errors. This methodology is similar to past overreliance studies, but past works often study overreliance on predictions that can be objectively considered incorrect~\cite{vasconcelos2023explanations}. In data analysis suggestions, some errors are objectively incorrect (e.g. saying a result is significant when it is not and suggesting a statistical model with incorrect assumptions), but there are other judgments that may be more difficult to make (e.g. overstating the importance of a step, suggesting data manipulations that are valid but may change distributions etc). Due to the nature of the data analysis task, work in this area could provide a new dimension to overreliance work. ~\mgm{I am trying to argue why this is also interesting for overreliance work as well, but I'm not too happy with the current examples for judgments that are more difficult to make, Can anyone else think of examples? Or might this be overstating the importance of this difference?. If we think this is a point worth arguing I will add more citations.} \ken{this is indeed very interesting! Analysts often can't even come to a consensus themselves on what is right or wrong unlike existing work on overreliance which has one correct answer.}
\tim{I agree it's interesting but had a similar impression. If the "not obviously right or wrong" is the key addition, that could be viewed as a limitation and something that's really hard to evaluate. could consider explicitly embracing that and arguing why you still think it's important.}

\tim{the paragraph above seems to only study overreliance but you don't talk about how to design and calibrate trust (what the title suggests and what seems  like a great design implication). What do we know from overreliance literature to deal with this in terms  of potential solutions. E.g., assistant could alert analystss about potential mistakes. assistants could avoid relying on LLMs for regurtitating numbers/analysis results but actually execute code to ensure correctness?...}

Using similar methods, future work also can judge the effectiveness of the assistant intervention through the quality of the final analysis outputs, or by creating experimental conditions in which the incoming dataset has flaws and seeing if people perform those accountability measures to address those flaws.

\subsection{Limitations}
\label{sec:discussion_limitations}
There are several limitations involved with our \woz study approach. First, the study was focused on people willing to participate in the study and perform data analysis with an AI assistant. This may affect analysts to be more willing to work with the assistant and exploratory in probing the assistant's capabilities. 

Next, to facilitate a lab study of reasonable duration, we chose to conduct a same-day in-person study of two hours. This time pressure, which is also realistic in certain scenarios, may have pushed analysts towards favoring execution assistance. Likewise, although we chose a \woz study to enable greater control over the assistant and its suggestions, the lab setting may not have the same stakes as a real-world setting. Outside the lab, conclusions from analyses may impact critical decisions and analysts may be more careful because of that. As a result, they can both be more willing to accept planning assistance and place assistant suggestions under greater scrutiny. Nevertheless, we tried to mitigate this effect by priming analysts to give increased consideration to the robustness of their analysis decisions in our task and introductory material. 

We also selected analysts who self-identified as having high proficiency in statistical analysis. As we were motivated by understanding the mechanisms surrounding planning assistance, we determined analysts with sufficient programming and statistical knowledge would be more engaged with analysis planning and our assistant's suggestions. Analysts with less statistical and programming expertise may have different experiences and preferences when working with an analysis assistant. Nevertheless, even the experienced analysts in our study were often unaware of the decisions and rationales pointed out by our assistant. As even trained analysts can form divergent analysis conclusions and are often the ones performing analyses that influence critical real-world decisions, understanding how planning assistance with this audience is paramount. Future work could explore how execution and planning assistance may be incorporated for novice data analysts.
% or beginners in a more educational setting. 
% \tim{the educational part is interesting but came out of nowhere for me.}

% Finally, while overarching principles were in place as to when and what suggestions we raised, there is room for personal bias regarding what the wizard determined to be relevant and important. However, as our study is largely exploratory, there was no easy way to get around it without a rubric so rigorous it would assume the answer to what we were exploring. \tim{is this last sentence commonly put in woz papers? otherwise perhaps just say: as this was a necessarily exploratory study, the wizard was not bound to a strict protocol and it is possible that wizard actions reflected biases despite best attempts to mitigate them. --- are we worried about any particular bias? paragraph is important but feels very generic. what's a concrete example that would be problematic?}


% \subsection{Future work}
% \label{sec:discussion_future}

% \tim{this section feels overlapping with 8.3 design implications. I suggest to not call it future work and consolidate it into design implications. for example, calibrating trust seems to fit well there too. what do you think?}

% \xhdr{Designing for shared analysis goals and background}
% Given the importance of shared analysis goals and background between the analyst and the assistant (Sec. \ref{sec:discussion_commonground}), it is important to design mechanisms in the system to enable this union. That being said, there are open questions surrounding how this could best be achieved. Analysts could communicate this early on with the assistant and update this throughout the interaction. It is an open question on how to design this interaction such that there is not too much responsibility placed on the analyst to determine the level of assistance they require. Meanwhile, the assistant could infer analysts' goals based on the content of the analysis. \textit{LIDA}, \cite{Dibia2023LIDAAT} for example, uses LLMs to generate visualization goals based on a dataset. More broadly, recent work \cite{Park2023GenerativeAI} in the context of simulating human behavior in AI agents leverages ChatGPT to store experiences in memory, and dynamically retrieve the relevant background to inform agent behavior. Data analysis assistants can utilize a similar framework to store the background and actions of analysts and use the appropriate information to determine the adequate level of planning assistance at different moments in the analysis. However, this is no easy task. This was partially what the wizard was trying to do in our study and was difficult even with additional inputs from analysts' screens and audio. Future work could explore the extent to which LLMs can support this and what sorts of behaviors are characteristic of analysts engaging in analysis execution and  planning. 


% \xhdr{Designing for calibrated trust} 


%%%%%%%%%%
% Subsection: What
%     - Different levels of planning help
%     - Challenges with building a fully automated system and the stochastic nature/hallucinations that comes with LLMs

% Subsection: Helpfulness
%     - Varying analyst needs
%         - speed vs accuracy etc
%     - Changing assistant's goal:
%         - Effect on output conclusion of analysis
%             - Could take datasets /analysis goals that are hard in different ways and see if it’s able to catch

% Subsection: Common ground
%     - Impacting analyst perception of common ground
%         - Overreliance / trust  (& effect of wording on this perception)
%     - Impacting assistant perception of common ground:
%         - changing explicitness / methods of defining common ground (Subsection: initiative)
%     - Changing use of common ground
%         - More rigorous study of when different things are useful (Subsection: When)?











%%%%%%%% NOTES
% - Change so a small future work seciton at the bottom of each discussion section?
